Interpolation can hurt robust generalization even when there is no noise

Numerous recent works show that overparameterization implicitly reduces variance for min-norm interpolators and max-margin classifiers. These findings suggest that ridge regularization has vanishing benefits in high dimensions. We challenge this narrative by showing that, even in the absence of noise, avoiding interpolation through ridge regularization can significantly improve generalization. We prove this phenomenon for the robust risk of both linear regression and classification and hence provide the first theoretical result on robust overfitting.

==> Neurips_submission_version/conclusion.tex <==
\vspace{-0.1in}
\section{Conclusions}

% Highly overparameterized models enjoy inductive biases that make them generalize
% well even for noisy data and in the absence of explicit regularization. In this
% work we offer a different perspective and argue that interpolation can indeed be
% suboptimal when the goal is robustness to adversarial attacks or distribution
% shifts. We show that ridge regularization .....
% Moreover, our work provides both a rigorous analysis and insights about robust
% overfitting, showing that it also occurs in noiseless and linear settings.

We show that overparameterized linear models can overfit with respect
to the robust risk even when there is no noise in the training
dataset. Our results put into perspective the modern narrative that
interpolating overparameterized models yield good performance without
explicit regularization and motivate the use of ridge regularization
and early stopping for improved robust generalization. Perhaps
surprisingly, we further observe that ridge regularization enhances
the bias of logistic regression trained with adversarial
$\ell_{\infty}$ attacks towards sparser solutions. Thus, ridge
regularization can have a positive effect on generalization for
high-dimensional linear models going beyond variance reduction.  While
our theoretical results hold for the ridge penalty, we experimentally observe
the same behavior for early stopping gradient descent.
While our theoretical results apply for ridge
regularization, we also observe the same behavior for early stopping. A formal
proof could reveal important insights to better understand the phenomenon and  we
leave this as future work. Furthermore, it would be interesting to study
whether our observations also transfer to random feature and kernel regression.

%% A formal proof of this phenomenon would be insightful and motivates
%% interesting future work. Furthermore, it could prove useful
%% to investigate whether our observations also transfer to 
%% random feature and kernel regression.

%% %% could reveal important insights to better understand the
%% %% phenomenon. We motivate this as a as future work. Furthermore, it
%% %% would be interesting to study how our observations transfer to
%% %% non-linear feature models.
%% =======
%% We show that overparameterized linear models can overfit with respect to the
%% robust risk even when there is no noise in the training dataset. Our results put
%% into perspective the modern narrative that interpolating overparameterized
%% models yield good performance without explicit regularization and motivate the
%% use of ridge regularization and early stopping when the aim is to achieve robust
%% generalization.  Perhaps surprisingly, we observe that ridge regularization
%% enhances the bias of logistic regression trained with adversarial
%% $\ell_{\infty}$ attacks towards sparser solutions. Thus, ridge regularization
%% can have a positive effect on generalization for high-dimensional linear models
%% going beyond variance reduction.  While our theoretical results apply for ridge
%% regularization, we also observe the same behavior for early stopping. A formal
%% proof could reveal important insights to better understand the phenomenon and  we
%% leave this as future work. Furthermore, it would be interesting to study
%% how our observations transfer to non-linear feature models. 
%% >>>>>>> 82fc5f8d7891fa848f89a46df3c8ee696600b9b6



==> Neurips_submission_version/intro.tex <==
\section{Introduction}

Classical machine learning theory and practice suggest caution when fitting a
model to data: exactly fitting the training data, without regularization, can
result in high variance, and thus, sub-optimal prediction performance. This rule
of thumb seemingly does not apply to large, overparameterized models: Large
neural networks, for example, have excellent generalization performance on
\iid{} sales despite their ability to interpolate the training
set~\cite{Zhang16}. 

Empirical evidence suggests that interpolating the training data can even help
neural networks to generalize better as the model size grows~\cite{Nakkiran20},
and theoretical work for linear models \cite{Dobriban15, Mei19, Bartlett20,
Muthukumar20, Muthukumar20a} and kernel methods \cite{Liang20a, Ghorbani19} has
shown that increasing the dimensionality of the data decreases the variance. 


These findings promote the perspective that there is no need for regularization
for modern, high-dimensional models. However, these prior works focus
exclusively on the impact of interpolation on the \emph{standard} test risk that
assumes \iid{} training and test data.

This measure of performance, however, may not reflect the accuracy of model
deployed in the real world, where robustness to distribution shifts, adversarial
attacks, or fairness metrics such as the worst-group risk play an increasingly
important role.
 %to distribution shifts and other notions of robustness.  In order to evaluate
%and enhance reliability, alternative performance metrics have recently gained
%popularity, such as distributionally and adversarially robust risks, or
%fairness metrics including the worst-group risk. 

%The robust notions of risk are governed by two terms that feature prominently in the statistical literature: the first is due to noise in the data (\emph{variance}), and the second persists even in the noiseless case (\emph{bias}).


%Classical wisdom \cite{Hastie01} suggests to use regularization in order to reduce variance, at the cost of an increased bias that prevents models from achieving vanishing training loss (which we refer to as \emph{interpolating}).
% to prevent an estimator to achieve vanishing training loss (we say it
% \emph{interpolates}) and hence fit noise. % RH: rewritten because potentially
% misleading, because not clear whether the estimator literally fits noise when
% it is regularized

% With the emergence of heavily overparameterized models that generalize well
% despite interpolating the data (i.e.\ achieving vanishing training loss),
% significant attention has been directed to understanding interpolation in the
% overparameterized regime. In particular, increasing width in neural networks
% also seems to remove the need to avoid interpolation.\fy{cite DDD} \rh{I don't
% get the last sentence-increasing width makes the network more linear; how does
% that remove the need for interpolation?}. The theory community has since
% presented multiple results to explain this phenomenon for linear, kernel and
% RF regression models: in particular they find that increasing dimensionality
% \rh{do you mean model size? If yes, let's better use model size.} decreases
% variance \fy{cite everybody} \fy{also kernels doesn't quite fit here}.
% Therefore, the dominant narrative/conclusion in the current literature on
% overparameterized models is that there is no need for regularization in high
% dimensions.

% However, those findings presume that the data is noisy; for example, DDD shows
% the double descent phenomenon only after adding artificial label \rh{We have
% to be careful here; Mei and Montanari establish double descent ``The
% generalization error of random features regression'' for the noise-less case.
% Here, the missfit of the models (data geneated linearly, estimator is random
% feature model) ``noise'' has an effect just like noise. Can we say ``those
% findings presume that the data is noisy or that there is a model missfit'', or
% is this not accurate any more?} %However there are a few shortcomings that
% this conclusion does not explain: For one, is the data really noisy? .
% CIFAR10 can achieve 99.7\% on the latest models .  

In fact, mounting empirical evidence challenges the narrative that there is no
need for regularization for modern, high-dimensional models, and suggests that
regularization actually improves \emph{robust test risks}, for instance in the
context of adversarial perturbations \cite{Rice20} or for worst-group
generalization \cite{Sagawa20a, Sagawa20b}, even in the highly overparameterized
regime! This phenomenon persists even after we perform data sanitization
procedures to drastically reduce the noise in the training data, as illustrated
by our experiments in Figure~\ref{fig:teaser_plot_nn} (we provide details on the
experimental setup in Section~\ref{sec:appendix_experiments} of the Appendix).

% These experimental findings suggest that robust notions of performance still
% require regularization even for overparameterized models. The goal of this
% paper is to understand the causes of this phenomenon and investigate the
% following question theoretically: 
% 
% \begin{center} 
% 
% %   \emph{If the data is noiseless/In the highly overparameterized regime where
%   %   variance is low, when is it still beneficial to avoid perfectly fitting
%   %   the training data/minimizing the training loss?}
%   \emph{In the highly overparameterized regime in which variance is low, why is
%   it still beneficial to avoid perfectly fitting the training data?}
% 
% \end{center}
% 
% \rh{This formulation of a question is too vague, can we formulated it
% differently? Also, the question should contain some reference to robustness,
% because that is central. Perhaps this question: ``Is there a provable robustness
% benefit of regularizing interpolating models in the noiseless regime?''. If we
% can't find a good formulation here, we can also work without posing a concrete
% question.}
%``....'' Here we need a more concrete question that we actually answer, than
%the one emphasized below.  }

%These experimental findings indicate that the current perspective on
%the benefits of interpolation in high dimensions may be incomplete,
%and that one may arrive at a different conclusion if robustness is
%considered for evaluation \fy{imprecise sentence in part due to
%  passive voice. which different conclusion?}. In this paper we aim to
%fill this gap and study the following question:
%


\fy{not sure I'd use ``interpolate'' here}
% Further, it seems that when measuring the adversarially robust risk or
% worst-group generalization, early stopping before the training loss vanishes in
% fact improves generalization (\emph{robust overfitting}), even for very wide
% overparameterized models! \fy{cite rice, pangwei} Also, even after proposed
% noise sanitization procedures on very simple images,~\ref{fig:teaser}, we still
% observe robust overfitting.

%% Generalization performance measure using risk / test metric.
%% Risks that
%%  we care about: natural/standard + robust 
%% distributional robustness
%% adversarial robustness (related)
%% Image experiments also find robust overfitting but only give explanation for noisy and argue noiseless 
%% Generalization / excess risk depends on a term that is nonzero only when there’s noise (we say variance…?) and another term that is driven by optimization procedure, averaged over training data (we call bias)

These experimental findings suggest that robust notions of performance still
require regularization even for overparameterized models. When the training data
does not contradict the ground truth, for example for noiseless observations or
for adversarial training with consistent perturbations \cite{Raghunathan20},
then a natural intuition is that leveraging all signals perfectly should help to
achieve best generalization.
% contains samples of the ground truth  \fy{I want to include consistent
% adversarial perturbations here} without noise, a natural intuition is that
% leveraging all signals perfectly should help to achieve best generalization.
%% Even though when working with noiseless data a natural reflex is to
%% use all the signal in the training set and interpolate to achieve the
%% best generalization, there exist examples \fy{of what?} that indicate
%% otherwise.
For instance, it is well-known that when the ground truth has a low-dimensional
structure matched by the implicit bias of the estimator, we can hope to achieve
good generalization even with relatively little data, as is the case for the
lasso estimator \cite{Tibshirani96}. However, in the case of a structural
mismatch, interpolation may not suffice to find a satisfactory overparameterized
estimator.

In particular, our main contribution is that we show theoretically that
achieving zero training loss does not lead to an optimal adversarially robust
risk for linear regression and classification, even in noiseless settings.
Moreover, we prove that $\ell_2$ regularization or early stopping can
significantly improve performance even for robust estimators trained with
adversarial training, a phenomenon previously observed empirically for neural
networks and referred to as robust overfitting \cite{Rice20}.

The next section introduces notation used throughout the paper and makes a
connection between adversarial and distributional robustness for linear models.
In Section~\ref{sec:linreg} we give precise asymptotics for the robust risk of
the ridge estimator and the minimum norm interpolator in the context of linear
regression. Then, in Section~\ref{sec:logreg} we show that adversarial training
for logistic regression can benefit from ridge regularization and provide
insights explaining this phenomenon.

% When the amount of noise in the data is insignificant, a natural reflex is to
% use all the signal in the training set and interpolate to achieve the best
% generalization. 

% A natural reflex is to say that even though in the overparameterized regime we
% are given little information about the function, we should use as much true data
% as possible, and deliberately avoiding interpolation would not help
% generalization. It is well known that in the case when the implicit bias of the
% interpolator matches a ground truth that has low-dimensional structure, we can
% hope to achieve good generalization even with relatively little data \fy{lasso
% etc.} However in the case of a structural mismatch, this might not be the case.
% For example, a recent paper shows for linear regression, how adding a new
% noiseless data point data can decrease prediction accuracy when the test
% distribution favors certain directions.  \fy{could cite our tradeoff paper - it
% is the only work in this direction that I know but its very ehm toy ...  don't
% have to cite, also makes the sentence harder}
% 
% In this work, we prove for linear regression and classification, that perfectly
% fitting all available noiseless samples is often undesirable in many scenarios,
% in particular for the robust risk. In Section bla we do bla.




%% Motivated by the observation that large deep neural networks \fy{cite
%%   Chiyuan,openai} \rh{perhaps zhang UnderstandingDeepLearning 2016} perform well, in recent years increasing attention has been
%% devoted in the field of learning theory to study when
%% estimators that achieve perfect train accuracy still generalize well.
%% %% interpolation \fy{maybe zero empirical risk sth...? unclear for classification}
%% %% with overparameterized models
%% %% still yields estimators with good
%% %% generalization properties \fy{a bit long}.
%% These papers show that overparameterization acts as implicit regularization as it reduces the variance in the high-dimensional regime when
%% $d,n\to\infty$ \fy{not sure if good to bring up here}. For certain distributions, it is even possible to
%% reach consistency \fy{cite benign, vidya, ghorbani etc.}. This
%% phenomenon is often manifested in a double descent shaped risk curve, where the risk as a function of the amount of overparameterization first decreases, then increases, and finally decreases again.
%% This is observed for a variety of machine learning models, including linear and logistic regression, random features and kernel
%% regression. \fy{citestuff}
%% %\rh{Perhaps better to not mention double descent so prominently here, because this is not central to the storyline (unless I'm missing something)}


%% %A common story and conclusion of these papers is to just interpolate without the need to regularize as the overparameterization ratio increases.  
%% This development suggests that training to interpolation without regularization is sufficient to obtain a well-performing model. 
%% However these conclusions were based on studying the
%% standard population risk only. Modern machine learning practice
%% often requires models to also exhibit certain degrees of reliability
%% and fairness such as robust against distribution shifts,
%% adversarial perturbations, and the ability to achieve good worst-group performances
%% \fy{citestuff}. Lately, there has been rising empirical evidence that
%% common methods to tackle these \emph{robust risks} in fact
%% \emph{benefit from regularization that prevent interpolation} even in
%% the overparameterized regime. This phenomenon, referred to as
%% \emph{robust overfitting} in some contexts, has been observed for
%% $\ell_\infty$ robustness and worst-group generalization for images.
%% \fy{cite pangwei and rice}. This raises the question:

%% \begin{center}

%% When does regularization regain its merits when measuring robust generalization?

%% \end{center}

%% Some works following the observations of \rh{cite pangwei and rice again} conjectured explanations based on experimental
%% evidence.  In particular they argue that robust overfitting is caused
%% by noisy or ambiguous samples in the training data
%% \cite{Amartya20,Dong21} and suggest filtering methods that can eradicate/mitigate
%% the phenomenon.
%% %That is, the robust risk and adversarial
%% %training amplify the variance due to noise and hence benefit more from
%% %regularization.
%% %reminiscent of similar geometric arguments  made in
%% %earlier work \fy{Gilmerblowup, goldstein stuff?}.
%% \fy{is it that we contradict the tautology paper with mnist 1,3
%%   or is it just that we show for pruned and unpruned, gap doesn't change?}
%% %% However recent results suggest that CIFAR-10 \fy{is not really that noisy},
%% %% and furthermore
%% However, as shown in Figure~\ref{fig:teaser}, simple experiments using the proposed variance
%% reduction methods \fy{is that true} suggest that robust overfitting persists even on MNIST
%% with a simple RELU MLP when the bootstrap estimated variance is below \fy{bla}.
%% \fy{explain gap in one sentence}

%% It is hard to rigorously verify or falsify that datasets such as CIFAR-10 are indeed noisy,
%% even though small bootstrap estimated variances \fy{steinhardt} and $99.7\%$
%% test performance with the latest architecture \fy{cite} suggest that label noise is indeed neglible.
%% To challenge this hypothesis, Figure~\ref{fig:teaser} shows that even after
%% noise reduction with a final variance of ..., robust accuracy persists
%% the overfitting gap of a
%% neural network trained on a pruned binary classification task where only classes
%% 1 and 3 from the MNIST data set were considered. We can still observe robust
%% overfitting in this sanitized setting, where the noise has been reduced
%% significantly. Perhaps surprisingly, even overparameterized models with
%% remarkably low variance still exhibit robust overfitting and benefit from
%% early-stopping regularization. This observation raises the following question:

%% \begin{center}

%%   \emph{Are there situations when preventing interpolation can actually be
%%   beneficial for overparameterized models?}

%% \end{center}


\begin{figure*}
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_nn.pdf}
    \caption{Neural network}
    \label{fig:teaser_plot_nn}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_linreg.pdf}
    \caption{Linear regression}
    \label{fig:teaser_plot_linreg}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_logreg.pdf}
    \caption{Linear classification}
    \label{fig:teaser_plot_logreg}
  \end{subfigure}

  \caption{ In this plot we show the gap between the standard and
    distributionally robust risk of the best regularized and final estimator for
    a (a) two-layer neural network with varying width, trained on (binary
    $1$-$3$) MNIST after using suggested variance reduction methods (see
    Appendix~\ref{sec:appendix_experiments}, regularized using early stopping .
    (b) linear regression on noiseless observations (c) distributionally robust
    training on logistic regression. The robust risk benefits significantly from
    regularization. For logistic regression, the standard risk also overfits
    however to a lesser extent than the robust risk.
    %% Performance gap between unregularized and optimally regularized estimators
    %% in simple noiseless interpolating settings.
    %% Subfigure \ref{fig:teaser_plot_nn} shows the performance of a two-layer neural networks with varying width, trained on (binary $1$-$3$) MNIST and evaluated with respect to $\ell_{\infty}$-perturbations.
    %% To reduce variance, we discard all training samples which a separately trained estimator cannot easily fit. We refer to
    %% \suppmat~\ref{sec:appendix_experiments} for the details.
    %% \ref{fig:teaser_plot_linreg} is linear regression standard training on noiseless synthetic data
    %% evaluated wrt $\ell_2$ perturbations.
    %% \ref{fig:teaser_plot_logreg} is logistic regression adversarial training on noiseless synthetic data
    %% trained and evaluated wrt $\ell_\infty$ perturbations. 
    %% The experiments shows that--even with the suggested variance reduction technique--the robust risk overfits (i.e., there is a non-zero gap between optimally regularized and the non-regularized estimate). 
%    \rh{Can we have a sentence summarizing the main conclusion from the
    %    experiment here, like: ``Even with the suggested variance reduction
    %    method, the robust overfitting phenomena persists.} a) The gap between
    %    optimal early stopped and final standard and robust risk with respect
    %    to $\ell_{\infty}$ perturbations for a single
%     hidden layer neural network with varying width on the binary $1$-$3$
    %     MNIST.  To reduce the variance, we additionally prune the samples
    %     which are not fitted by a separately trained estimator after early
    %     stopping.\ b) The estimated variance of the original and pruned data
    %     set. We refer to \suppmat~\ref{sec:appendix_experiments} for the
    %     details.
%   To reduce potential noise in the training set and fitting procedure, we
    %   discard all training samples which are not correctly classified within
    %   the first 100 epochs of training Nevertheless, we still observe
    %   significant robust overfitting in \ref{fig:teaser_overfitting}.  In
    %   order to quantify the amount of noise at hand,
%   we estimate model variances on the test set for each number of hidden units.
    %   \ref{fig:teaser_variances} shows the estimated variance averaged all
    %   test samples with bars indicating one empirical standard deviation.
    %   While the estimated variance for the full training set is already low,
    %   our pruning procedure further reduces it.
%   Artificial low-noise setting which exhibits significant robust overfitting.
    %   We fit a single hidden layer neural network with varying width on two
    %   MNIST classes.  To reduce potential noise in the training set and
    %   fitting procedure, we discard all training samples which are not
    %   correctly classified within the first 100 epochs of training
%   Nevertheless, we still observe significant robust overfitting in
    %   \ref{fig:teaser_overfitting}.  In order to quantify the amount of noise
    %   at hand, we estimate model variances on the test set for each number of
    %   hidden units.  \ref{fig:teaser_variances} shows the estimated variance
    %   averaged all test samples with bars indicating one empirical standard
    %   deviation.  While the estimated variance for the full training set is
    %   already low, our pruning procedure further reduces it.
  }

  \label{fig:teaser}
\end{figure*}
% 

%% Indeed, in this paper we show that robust overfitting occurs for
%% linear models \emph{even in the noiseless setting} in the heavily
%% overparameterized regime, illustrated in Figure~\ref{fig:teaser}.  We
%% prove robust overfitting of interpolating estimators for linear and
%% logistic regression in the high-dimensional regime.  In particular, we
%% show that in the overparameterized regime, i.e., for large overparameterization ratios $d/n \to \gamma$ and $d,n\to\infty$ regularization significantly improves generalization on the robust risk even though it does not benefit standard generalization. 
%% With this
%% work we'd like to provide a clear \fy{other word} counterpoint to an
%% increasing line of work that focuses on the diminished relevance of
%% regularization in the overparameterized regime.

%% %studies benefitsof overparameterization.

%% In section we do bla.

%% In this paper we answer this question in the positive and show that evaluating
%% adversarial robustness is one such setting where regularization does more than
%% only reduce variance.  Our main \textbf{contribution} is that we show that, for
%% both linear regression and logistic regression, the consistent robust risk
%% benefits from ridge regularization or early stopping even on noiseless
%% observations. Furthermore, this form of overfitting occurs only in the
%% overparameterized regime where the standard error benefits from the implicit
%% regularization that is characteristic for interpolating models. However, our
%% results demonstrate that interpolation can be harmful even when the standard
%% error does not suffer from overfitting.  Thus, we argue that regularization
%% plays a fundamentally different role for the consistent robust risk and acts not
%% just on the variance, but also as a form of bias reduction. To the best of our
%% knowledge, we are the first to study theoretically the impact of early stopping
%% and ridge regularization on the consistent robust risk for overparameterized
%% models. 

%% The double descent phenomenon, which has recently gained popularity in the
%% machine learning community, points to the beneficial effects of
%% overparameterization.  The effect of implicit regularization due to
%% overparameterizating has been first explicitly pointed out by \citet{Zhang17}
%% for deep neural networks where it is shown that these models achieve good
%% generalization performance although interpolating the train data. Surprisingly,
%% these observations put into perspective the classical wisdom on the
%% bias-variance trade-off which tells us us that the bias decreases and variance
%% increases with model complexity [TODO cite textbook]. Since then, a modern line
%% of statistical and machine learning research has emerged studying this effect
%% more carefully. In particular, the paper \cite{Nakkiran20,Yang20} observe that
%% the variance of deep neural networks decreases again after the interpolation
%% threshold when further increasing the model complexity, and hence achieve a
%% similar effect to regularization. 

%% Multiple papers from the statistical side underline this observation by proving
%% that such a behavior also occurs for classical regression and classification
%% algorithms including linear, logistic and random feature regression
%% \cite{Belkin19,Nakkiran20,Hastie19,Mei19,Deng20,Chinot21}. In fact, it has even
%% been shown that for certain spiked covariance data models both logistic and
%% linear regression can be asymptotically consistent in high dimensional regimes
%% albeit interpolating noisy train data \cite{Bartlett20,Muthukumar20}. In
%% summary, these papers suggest that the effect of implicit regularization in
%% overparameterized regimes makes explicit variance reduction techniques like
%% early stopping or ridge regularization redundant. 

%% All of these works have focused on the effect of overparameterization on the
%% prediction error of estimators. However, in many practical applications we are
%% interested in other criteria for evaluation as well, such as ensuring fair
%% predictors [TODO cite], or models that generalize well under covariate shift
%% [TODO cite]. Another example of a desirable property of prediction models, known
%% as \emph{adversarial robustness}, is that they are invariant to small (in
%% $\ell_p$ norm) additive perturbations of the input data \cite{Szegedy14}.
%% % For instance, in the case of image data sets these perturbations are often
%% % imperceptible to a human and, thus, do not change the semantics or the label
%% % of the inputs.
%% In order to avoid an ill-defined problem, it is crucial that the notion of
%% robustness that we use is not at odds with the other goal, which is to recover
%% the ground truth function and to achieve a low prediction error. To ensure that
%% we do not have interfering objectives, we only consider consistent perturbations
%% for evaluating the models, namely perturbations that do not change the value of
%% the ground truth function [TODO cite]. For linear models, consistent adversarial
%% robustness has even more profound consequences: perfect $\ell_p$ robustness
%% against consistent perturbations implies automatically robustness to
%% distribution shifts along any direction perpendicular to the linear ground
%% truth. This invariance to changes along directions that are independent of the
%% ground truth is of great importance in practice, in particular in situations
%% where fairness is important or when we do not wish to make predictions that rely
%% on spurious features.

% On top of achieving a low prediction accuracy on unseen test samples, in
% practical applications we often require the models to be robustness against
% perturbations in the input data.  \textit{say somehting here, but i really
% dont know the literature. This must be good, for instance we could mention
% fairness or distribution shifts? But motivate well why we do want a low robust
% risk BEYOND image data sets! Also motivate consistent perturbations}

% Modern machine learning models have to be vulnerable to imperceptible
% perturbations of the inputs \cite{Szegedy14}. This worrisome behavior has
% garnered a lot of attention in recent years and it spurred several lines of
% work that try to propose ways to defend against such adversarial attacks. Even
% though many of the suggested defences have been breached by carefully designed
% attacks \cite{Tramer20}, there are two approaches that stand out. Firstly,
% adversarial training \cite{Goodfellow15} has consistently been reliable even
% in the face of these newly discovered attacks. Secondly, a number of works
% have proposed certified defences \cite{Salman19, Balunovic19} which come with
% appealing robustness guarantees.

%% One popular approach to improve the robustness of a model to adversarial
%% $\ell_p$-perturbations is to use adversarial training (AT) where we minimize the
%% empirical risk with perturbed input train samples. This method has successfully
%% been applied to various models including deep neural networks
%% \cite{Goodfellow15} but also linear and logistic regression
%% \cite{Javanmard20a,Javanmard20b}. In a recent paper \cite{Rice20} the authors
%% uncover an interesting phenomenon: When minimizing the adversarial training loss
%% using an iterative algorithm (e.g.\ stochastic gradient descent), the
%% optimization path passes through a more robust solution first, before it
%% converges to a less robust one. Hence, an early-stopped model has better robust
%% accuracy, as measured on a hold out test set, than a model trained to
%% convergence. What makes this phenomenon surprising is that the authors observe
%% it for highly overparameterized deep neural networks where the natural test
%% error does not suffer from overfitting despite interpolating the train samples. 

%  A natural approach is to try and understand robust overfitting through the
%  lens of regular overfitting of the standard accuracy.  For a long time, the
%  classical statistics literature has pointed at noise as the major culprit for
%  overfitting.  More recently, a new story line has started to emerge:
%  overparameterization alone can mitigate overfitting by reducing the variance,
%  a phenomenon that is often referred to as `double descent`. One important
%  conclusion stressed by this line of work is that regularization is redundant
%  in the highly overparameterized regime.



% Our contributions are as follows:
% \begin{itemize}[leftmargin=*]
% 
%   \item for linear regression, we show that the consistent $\ell_2$ robust risk
%     benefits from ridge regularization or early stopping even on completely
%     noiseless observations. Furthermore, the described effect is only observed
%     in the overparameterized regime where the standard error benefits from the
%     implicit regularization described in \cite{Hastie19}.
% 
%   \item for classification, we study the consistent $\ell_{\infty}$ robust risk
%     for logistic regression and show that the adversarially trained estimator
%     suffers from overfitting of both the standard and robust risk, even in the
%     noiseless case. \at{TODO need to fit the next two sentences with the rest of
%     the story} Finally, we show that when adding label noise we need a higher
%     degree of overparameterization $d/n$ to interpolate the train data.
%     Surprisingly, this leads to the observation that the unregularized estimator
%     trained with noise achieves a lower final robust and standard risk compared
%     to the one trained without label noise.

%   \item for classification, we study the consistent $\ell_{\infty}$ robust
%     for logistic regression. Since standard training achieves only very poor robust risk, we focus on the adversarially trained estimator and show that this suffers from overfitting of both the standard and robust risk, even in the
%     noiseless case.
% \end{itemize}

% As a first contribution, we show that the consistent $\ell_2$-adversarial robust
% risk of linear regression benefits form ridge regularization or equivalently
% early stopping even on completely noiseless observations.  In this case, the
% variance of the standard risk is zero and hence suffers from explicit
% regularization. Our results demonstrate that interpolation can be harmful even
% when the standard error does not suffer from overfitting. Thus, we can conclude
% that regularization plays a fundamental different role for the consistent robust
% risk and Furthermore, the described effect is only observed in the
% overparameterized regime where the standard error benefits form the effect of
% implicit regularization as describe in the paper \cite{Hastie19}. 

% As a second contribution this paper studies the consistent
% $\ell_{\infty}$-adversarial robust risk for logistic regression on a
% discriminative sparse linear data model. While the standard trained estimator
% achieves very poor robust population accuracy close to $0$, the adversarially
% trained estimator trained with inconsistent adversarial $\ell_{\infty}$ attacks
% achieves a significantly better standard and robust test accuracy albeit still
% being able to interpolate the train samples. Surprisingly, however, we show that
% even in the noiseless case the estimator suffers from overfitting of both the
% standard and robust risk. While inconsistent attacks may induce some noise
% during training even for noiseless data, we also show that the we observe
% overfitting of the risks when training with consistent adversarial attacks
% assuming that we have full knowledge of the ground truth during training.
% Finally, we show that when adding label noise we need a higher degree of
% overparameterization $d/n$ to interpolate the train data. Surprisingly, this
% leads to the effect that the unregularized estimator trained with noise achieves
% a lower final robust and standard risk compared to the one trained without label
% noise. 

% Both examples demonstrate how interpolation suffers from overfitting in the
% overparameterized regime even for noiseless train data. As a result, this paper
% puts into perspective the modern story line on the implicit regularization due
% to overparameterization by highlighting that additional robustness constrains
% still require additional explicit regularization to prevent the model from
% interpolation. 





% This puts the modern story line on regularization into perspecti observes a
% vanishing In particular, we show that the robust risk suffers from overfitting
% even on noiseless which questions the 
% 
% 






% « In the paper \cite{Amatya20} the authors show that the robust accuracy is
% much more sensitive to noise in the train data than the standard accuracy.
% Although the experiments in the paper \cite{Rice20} are conducted on the
% original \textit{CIFAR-10} \cite{Krizhevsky09} dataset without any additional
% label noise, the authors from the paper \cite{Amatya20} highlight that these
% there are still misslabeled/wrong samples contained in the dataset. Therefore,
% the authors suggest that the overfitting of the robust risk may be explained
% due to a higher sensitivity to noise fitted by the estimator. A similar
% conclusion is suggested by the paper \cite{Dong21}, where the authors observe
% that the robust risk does not overfit when removing problematic samples which
% are not fit by a early stopped estimator form the data. 


% Yet this phenomenon not yet well understood and existing attempts to explain
% the phenomenon have predominantly linked it to noise respectively problematic
% samples in the train data. In the paper \cite{Amatya20} the authors show that
% the robust accuracy is much more sensitive to noise in the train data than the
% standard accuracy.  Although the experiments in the paper \cite{Rice20} are
% conducted on the original \textit{CIFAR-10} \cite{Krizhevsky09} dataset
% without any additional label noise, the authors from the paper \cite{Amatya20}
% highlight that these there are still misslabeled/wrong samples contained in
% the dataset. Therefore, the authors suggest that the overfitting of the robust
% risk may be explained due to a higher sensitivity to noise fitted by the
% estimator. A similar conclusion is suggested by the paper \cite{Dong21}, where
% the authors observe that the robust risk does not overfit when removing
% problematic samples which are not fit by a early stopped estimator form the
% data. 
% 
% While noisy/problematic samples in the train data certainly have an effect on
% the robust accuarcy, we observe in Figure~\ref{fig:teaser} that the robust
% accuracy overfits even on binary 1-3-MNIST with additional pruning of unfitted
% samples by a early stopped neural network. In this paper we aim to better
% understand 



% ttempt to explain the overfitting of the robust accuarcy due to an
% oversensitivity to noise in the train data.  samples. While noise in the train
% data clearly has an impact on robust overfitting (see Figure \ref{fig:asdf}),
% this paper shows that robust overfitting also occurs   noiseless settings
% where the natural accuracy does not benefit from regularization at all. Hence,
% this paper challenges the role of regularization: In the classical
% understanding we have that in the well specified setting, regularization leads
% to a bias-variance tradeoff, meaning that we increase bias but decrease
% variance. In particualr, this suggests that if you have no noise,
% regularization does not improve performance.  More specifically, this paper is
% the first one theoretically studying overfitting of the robust loss. Unlike
% existing literature we \kd{continue to write soon }


% 
% Mission of the paper: Hence we seek to complete the picture by proving the
% conjecture for lin reg The conjecture: in settings: ST, AT, noiseless … … when
% evaluating the robust error, early stopping is needed for a much wider range
% of d/n and p/n ratios, compared to testing using the std error Our
% contributions: We prove … … this conjecture is true in the settings above for
% linear models (lin reg).  in particular our claim is that …. causes it. (proof
% intuition) We also show experimentally that indeed RO happens in these
% settings and second the intuition carries through to images. 






% \kd{A bit a repetition from the intro}
% Robust overfitting is the intriguing phenomenon that has been observed by
% \cite{Rice20} on neural networks trained with adversarial training: early
% stopping regularization has a significant effect in reducing the robust test
% error, while, in contrast, the standard test error is always non-increasing as a
% function of time. \kd{Rice does this as well, need to write more here} In this
% section we provide empirical evidence that robust overfitting occurs even in a
% noiseless setting, raising questions about the nature of the phenomenon.

% \kd{this is already contained in the intro: A natural approach is to try and
% understand robust overfitting through the lens of regular overfitting of the
% standard accuracy. For a long time, the classical statistics literature has
% pointed at noise as the major culprit for overfitting.  More recently, a new
% story line has started to emerge: overparameterization alone can mitigate
% overfitting by reducing the variance, a phenomenon that is often referred to
% as `double descent`. One important conclusion stressed by this line of work is
% that regularization is redundant in the highly overparameterized regime.
% 
% Robust overfitting is indeed exacerbated by noise. Adding artificial label
% noise to the training data makes robust overfitting much more pronounced, as
% we show in Appendix TODO for overparameterized fully-connected neural
% networks. However, going in the opposite direction and \textit{reducing} the
% amount of noise of the prediction problem to a minimum reveals a surprising
% situation. In a noiseless setting where the variance vanishes, it seems like a
% sensible hypothesis is that regularization has no effect on the test robust
% error.  }

% \citet{Rice20} showed that the robust loss overfits when training
% overparameterized deep neural networks on CIFAR \cite{Krizhevsky09} without
% adding any additional label noise. However, as highlighted by \citet{Sanyal21}
% the original data set itself cointains noisy samples. Hence, we cannot
% conclude from the presented experiments that robust overfitting occurs even in
% the absence of noise. 

% , the following experiments indicate that, for overparameterized models, the
% role of regularization is not lpimited to just reducing the variance.




% The observation that regularization is beneficial even in a noiseless setting
% raises the following question:
% 
% \begin{center}
% 
%   \textit{Can regularization reduce the bias of overparameterized models \\
%   with respect to certain evaluation metrics?}
% 
% \end{center}
% 
% In particular, is it the case that certain traditional regularization
% techniques are better suited at priming estimators for robust evaluation? In
% the sequel we analyze lineapr and logistic regression in the context of
% adversarial robustness and prove that, in high dimensions, early stopping and
% ridge regularization lead to more robust predictors.


==> Neurips_submission_version/lin_reg.tex <==
\section{Regularization for linear regression}
\label{sec:linreg}

In this section we prove that preventing interpolation on noiseless
samples via ridge regularization~\eqref{eq:ridgeloss} with $\lambda
>0$ improves the robust risk relative to an un-regularized,
interpolating predictor.  We further provide an explanation for why
regularization is beneficial for the robust risk when it is not
beneficial for improving the standard risk.
%% , which we argue is due to how the two risks penalize
%% differently the terms that appear in their decomposition.
% an overparameterized least-squares estimator provably exhibits robust
% overfitting, i.e., there is a gap between the $\ell_2$-regularized robust risk
% and the robust risk, even when there is no such gap for the standard risk. We
% then explain this by decomposing the robust risk into two terms, and
% demonstrating that regularization achieves a better trade-off between those
% two terms.

\subsection{Problem setting}
\label{sec:linregsetting}

We consider an observation model with covariates $x \in
\R^d$ drawn from a standard normal distribution with zero mean, i.e., $x \sim
\Normal(0,I_d)$, and with the target variable $y \in \R$ defined as
a noisy observation of a linear function  $y = \langle \thetatrue, x \rangle + \xi $ with $\xi \sim \Normal(0, \ynoisestd^2)$.
% \begin{equation*}
% y = \langle \thetatrue, x \rangle + \xi,
% \quad \text{with} \quad \xi \sim \Normal(0, \ynoisestd^2).
% \end{equation*}
Here, $\thetatrue$ denotes the ground truth vector which we set to
have unit $\ell_2$-norm.  As mentioned before, we focus on the
noiseless case of $\sigma=0$ since overfitting is not expected for
that case and include $\sigma>0$ only for
completeness.
%% linear predictor is determined by a fixed, unit
%% $\ell_2$-norm vector $\thetatrue$, and $\xi$ is additive Gaussian noise.
%Our results hold for general $\sigma^2 \ge 0$, even for the noiseless setting with$\sigma^2 = 0$, as we stress later in the section. \rh{too early to remark this because context is missing-reserve for later}
We illustrate the phenomenon of robust overfitting
for consistent $\ell_2$ perturbations sets~\eqref{eq:AR}.
% \fy{in some sense also a standard choice in the linreg literature right? can we refer to lit here?}.
%% aim to learn a linear model that achieves small adversarially
%% robust risk against consistent $\ell_2$ perturbations
%% (as defined in~\eqref{eq:AR} with $p=2$).
By Lemma~\ref{lem:dro} in the appendix, this is equivalent to
minimizing the distributionally robust risk for $\ell_2$-bounded mean
shifts.  Due to rotation invariance of the problem our results hold
for sparse and dense vectors alike.  We expect robust overfitting also
for $\ell_\infty$ perturbations and different choices of $\empriskrob$
and $\thetatrue$ but leave a detailed discussion for future work.
% \fy{we expect RO also for: linf AT on dense vectors with AT. linf
%   sparse vectors and ST} \fy{maybe add some exps?}
%with distributional neighborhood definedin~\eqref{eq:DR}.
%% \fy{no
%%   real motivation} Equivalently, our goal can be viewed as searching
%% for a distributionally robust estimator, using Equation~\eqref{eq:DR}
%% for evaluation, where we choose $\probspace$ to be the space of all
%% normal distributions $\Normal(\mu,\Sigma)$ with $\langle \mu,
%% \thetastar\rangle = 0$ and $\probmet(\probx,\probrobx) =
%% \|\mu(\probx)-\mu(\probrobx)\|_2$. \fy{a bit too many symbols for what
%%   it is}
%% %% against small mean shifts
%% %% i.e. $X\sim \Normal(\mu,\inputcov)$ with $\|\mu\|_2\leq \eps$.
%% A formal proof of this equivalence can be found in Lemma~\ref{lem:dro} in the
%% appendix. \fy{write Lemma!}

\subsection{Interpolating and regularized estimator}
We study the ridge penalized loss for
regression~\eqref{eq:ridgeloss} that corresponds to $\epstrain = 0$
and choosing $\losstrain$ as the squared loss which yields
\begin{equation}
  \label{eq:linregridge}
\thetalambda = \arg\min_{\theta} \frac{1}{n} \sum_{i=0}^n (y_i - \langle \theta,
x_i \rangle)^2 + \lambda \|\theta\|_2^2.
\end{equation}
% that we obtain by choosing the square loss
% $\losstrain(u,v)=\frac{1}{2}(u-v)^2$ and $\epstrain =0$ in
% Equation~\eqref{eq:ridge}.  and reads
%% trained by minimizing the
%% standard risk, i.e.\ $\epstrain = 0$, which, for the square loss, takes the
%% following form
For $\lambda > 0$, we obtain a regularized predictor $\thetalambda$. In
addition, we also consider the minimum norm interpolator, namely the
unregularized estimator that corresponds to $\lambda \to 0$ and can be written
as follows:
\begin{equation} \label{eq:minnorm} \thetaminnorm =
\arg\min_{\theta} \|\theta\|_2 ~~\mathrm{such~that}~~ \langle \theta, x_i\rangle
= \y_i ~~\mathrm{for~all}~ i.
\end{equation}
The minimum norm interpolator is the solution of gradient descent whereas
ridge regression with $\lambda > 0$ corresponds to early stopping path \cite{Ali19,Ali20}.

The attentive reader might wonder why we choose $\epstrain=0$, corresponding to standard training although we study the robust risk. For this we need to note that consistent adversarial training with $\epstrain >0$ simply recovers the ground truth as it reveals full information during training. On the other hand, adversarial training with inconsistent perturbations has a similar effect to $\ell_2$ regularization and in particular prevents the estimator from interpolating (see more detailed discussion in~\ref{sec:linreg_inconsistent}).


%
%
% leads to a penalty on the $\ell_2$-norm of the projection of $\theta$ onto the ground truth vector $\thetatrue$, and is minimized by the ground truth in the noiseless case - in contrast, we are interested in settings where the structural bias and hence the interpolator is imperfect and study whether regularization can help in that case.
% Inconsistent perturbations, i.e. entire $\ell_2$ balls, on the other hand
% introduce noise to the training loss that is not the focus of our exposition
% (see more detailed discussion in~\ref{sec:linreg_inconsistent}).
% \fy{honestly still think having $\sigma>0$ makes it really harder to argue here}.


% The attentive reader might wonder why we choose $\epstrain=0$, corresponding to standard training although we study the robust risk. For this we need to note that consistent adversarial training with $\epstrain >0$ leads to a penalty on the $\ell_2$-norm of the projection of $\theta$ onto the ground truth vector $\thetatrue$, and is minimized by the ground truth in the noiseless case - in contrast, we are interested in settings where the structural bias and hence the interpolator is imperfect and study whether regularization can help in that case.
% Inconsistent perturbations, i.e. entire $\ell_2$ balls, on the other hand
% introduce noise to the training loss that is not the focus of our exposition
% (see more detailed discussion in~\ref{sec:linreg_inconsistent}).
% \fy{honestly still think having $\sigma>0$ makes it really harder to argue here}.
%% minimizing the loss
%% does not yield perfect estimator and study whether regularization improves them.
%% This particular interpolating
%% estimator has been heavily studied in the overparameterized literature \fy{cite}
%% as it corresponds to the solution obtained by running gradient descent on the
%% least-squares loss, and thus models the implicit bias of gradient descent.
%% \fy{in case the reader wonders about why not AT}: We focus on the standard
%% training as it is implementable in practice without prior knowledge about
%% $\thetastar$, as opposed to adversarial training with consistent perturbations.
%% \at{maybe mention inconsistent perturbations}



\subsection{Main result and experiments}

% ne maybe unexpected observation has been pointed out in \cite{Hastie19} The
% simplicity of the model allows This allows a very rigorous theoretical
% understanding of the behavior of the model.

The following theorem provides a precise asymptotic description of the
consistent $\ell_2$ robust risk for the ridge regression estimate
in~\eqref{eq:linregridge} as $d/n\to\gamma$ and $d,n\to\infty$. The proof uses
techniques from \cite{Hastie19,Knowles16} and can be found in \suppmat~\ref{sec:prooflinregthm}.

\begin{figure*}
  \centering
  \includegraphics[width=5.5in]{figures/linreg_standard_training_legend.pdf}
  \begin{subfigure}[b]{2.7in}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/fig_eps_diff.pdf}
    \caption{Noisy observations}
    \label{fig:lra}
  \end{subfigure}
  \begin{subfigure}[b]{2.7in}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/fig_eps_diff_noiseless.pdf}
    \caption{Noiseless observations}
    \label{fig:lrb}
  \end{subfigure}
  \caption{ We plot the asymptotic theoretical predictions for $d,n\to\infty$ (curves)
    and experimental results with finite $d,n$ (markers) for the
    robust (yellow, $\epstest=0.4$) and standard (blue) risk of the
    min-norm solution (solid, \emph{interpolating}) and the ridge
    regression estimate with the optimal $\lambda$ (dashed,
    \emph{regularized}) for noisy data with $\sigma^2 = 0.2$ (left)
    and noiseless data (right). For the experiments we use
    $n=1000$ and the model described in
    Section~\ref{sec:linregsetting}.  We observe that the gap between
    the robust risk of the interpolating and optimally regularized
    estimator remains even when $\sigma^2 = 0$.
    \vspace{-0.2in}
    }
  %%   The for the asymptotic robust risk of the standard linear ridge
  %%   regression algorithm ($\epstrain = 0$) as a function of $\gamma
  %%   = d/n$ for isotropic Gaussian features with (a) additional
  %%   $\sigma^2= 0.2$-normal distributed noise and (b) noiseless
  %%   observations.  The risk is plotted for different choices of
  %%   test attack strengths $\epstest$. Dashed lines show the
  %%   unregularized risk ($\lambda = 0$) and solid lines the risk for
  %%   the optimal regularization parameter $\optridgeparam$.  We
  %%   verify our predictions empirically using $n = 1000$ training
  %%   samples and mark the risks of estimators trained with and
  %%   without optimal regularization using crosses and diamons
  %%   respectively.
  \label{fig:main_thm_lr}
\end{figure*}



\begin{theorem}
\label{thm:main_thm_lr}

%% For any $\lambda \geq0$ the risk of the standard estimator $\thetahat$
%% minimizing the mean squared loss from Equation \eqref{eq:SE} and
%% \eqref{eq:minnorm} with additional ridge regularization $\lambda \geq 0$
Assume isotropic Gaussian covariates, i.e., $\prob_X = \Normal(0, \idmat_d))$. Then, for $d,n \to \infty$ with $d/n \to \gamma$ and for any $\lambda\geq 0$, the robust risk of the
estimators $\thetalambda$ defined in
Equations~\ref{eq:linregridge},~\ref{eq:minnorm} converges
\begin{align}
 \AR(\thetalambda) \: \overset{\text{a.s.}}{\longrightarrow} \:\Biasinfty + \Varinfty +  \epstest^2  \Pperpinfty + \sqrt{\frac{8 \epstest^2}{\pi} \Pperpinfty ( \Biasinfty + \Varinfty)} ,
\end{align}
where  $ {\Pperpinfty= \Biasinfty + \Varinfty -\lambda^2 (m(-\lambda))^2}$ and  ${\Biasinfty = \lambda^2 m'(-\lambda)}$, ${\Varinfty = \sigma^2 \gamma (m(-\lambda) - \lambda m'(-\lambda))}$ are the
asymptotic bias and variance with ${\SR(\thetalambda)\: \overset{\text{a.s.}}{\longrightarrow}\: \Biasinfty + \Varinfty}$ as shown in Corollary 5 of \cite{Hastie19}. The function $m(z)$ is given by $m(z) = \frac{1 - \gamma - z - \sqrt{(1-\gamma
-z)^2 - 4 \gamma z }}{2\gamma z}$ and $m'$ is the derivative of $m$. Finally,
% \begin{align*}
%  \Pperpinfty &= \Biasinfty + \Varinfty - 2 \lambda m(-\lambda) +1 - (1-  \lambda m(-\lambda))^2.
% \end{align*}
% \begin{align*}
%  \Pperpinfty &= \Biasinfty + \Varinfty -\lambda^2 (m(-\lambda))^2.
% \end{align*}
\end{theorem}


% \begin{theorem}
% \label{thm:main_thm_lr}
%
% %% For any $\lambda \geq0$ the risk of the standard estimator $\thetahat$
% %% minimizing the mean squared loss from Equation \eqref{eq:SE} and
% %% \eqref{eq:minnorm} with additional ridge regularization $\lambda \geq 0$
% Assueme isotropic Gaussian covariates (i.e. $\prob_X = \Normal(0, \idmat_d))$ and $d,n \to \infty$ with $d/n \to \gamma$ and for any $\lambda\geq 0$, the robust and standard risk of the
% estimators $\thetalambda$ defined in
% Equations~\ref{eq:linregridge},~\ref{eq:minnorm} converge to
% \begin{align}
%  \SR(\thetalambda)\: \overset{\text{a.s.}}{\longrightarrow}\: \Biasinfty + \Varinfty ~~\textrm{and} ~~
%  \AR(\thetalambda) \: \overset{\text{a.s.}}{\longrightarrow} \:\Biasinfty + \Varinfty + 2\sqrt{\frac{2}{\pi}} \epstest \Pperpinfty \sqrt{\Biasinfty + \Varinfty} + \epstest^2  \Pperpinfty^2,
% \end{align}
% where $\Biasinfty$ and $\Varinfty$ denote the usual bias and variance \fy{rephrase} and
% \begin{align*}
%  \Biasinfty &= \lambda^2 m'(-\lambda),~~
%  \Varinfty = \sigma^2 \gamma (m(-\lambda) - \lambda m'(-\lambda)) ~~\mathrm{and}\\
%  \Pperpinfty^2 &= \Biasinfty + \Varinfty - 2 \lambda m(-\lambda) +1 - (1-  \lambda m(-\lambda))^2.
% \end{align*}
% The function $m(z)$ is given by $m(z) = \frac{1 - \gamma - z - \sqrt{(1-\gamma
% -z)^2 - 4 \gamma z }}{2\gamma z}$ and $m'$ is the derivative of $m$.
% \end{theorem}



Using the precise asymptotics derived in this theorem, we plot
the asymptotic standard and robust risk of the ridge estimate
with the optimal $\lambda$ parameter and the min-norm interpolator in Figure~\ref{fig:main_thm_lr}.\footnote{Here we choose $\lambda$
using the population risk oracle, in practice one would resort to standard tools such as cross-validation techniques \cite{Patil21}}
%% The main message of this theorem is captured by the curves in
%% Figure~\ref{fig:main_thm_lr} that show the theoretical predictions for the
%% standard and robust population risks ($\SR$ and $\AR$, respectively) as
%% functions of the $d/n$ ratio\footnote{For standard risk, similar curves have
%%   been presented in \cite{Hastie19}}.
%% We highlight a number of surprising observations that follow from
%% Theorem~\ref{thm:main_thm_lr}.
Firstly, Figure~\ref{fig:lra} reveals
that ridge regularization reduces the robust risk even for $d>n$
well beyond the interpolation threshold where
previous works show that variance is negligible.
%regularization has no effect on the standard risk.
Moreover, Figure~\ref{fig:lrb} shows that the beneficial effect of ridge regularization persists even for noiseless data, that is when $\Varinfty = 0$.
This supports our statement that regularization not only helps reduce
variance,
% \fy{ superfluous cause we have the noiseless case, also don't wanna stress }
%% as we see for instance close to the interpolation threshold
%% when the data is noisy,
but also reduces the part of the robust risk that is unaffected by noise in the overparameterized regime.
%% but it also endows estimators with the right
%% structure that is required to achieve a low robust risk,
%% thus acting
%% as a form of bias reduction in the overparameterized
%% regime.
Furthermore, we show that experiments (depicted by the markers in
Figure~\ref{fig:main_thm_lr}) run with finite $d$ and $n$ closely
match the predictions in Theorem~\ref{thm:main_thm_lr} for $d, n \to
\infty$ and $d/n \to \gamma$. This indicates that the asymptotic
regime that we adopt in this paper indeed characterizes the
high-dimensional non-asymptotic regime well.
% \fy{here or where?}
Finally, even though Theorem \ref{thm:main_thm_lr} assumes isotropic Gaussian covariates
$\inputcov=I_d$, we can extend the result to more general covariance matricies following the same argument as in \cite{Hastie19} based on random matrix theory \cite{Knowles16}.

% we expect the behavior to persist for arbitrary
% diagonal $\inputcov$ with effective dimensionality asymptotically
% proportional to the sample size, i.e. $\trace(\inputcov)/n \to\gamma$.
% We leave the analysis of the more general case to future work.


% Finally, even though we prove RO for the special case of
% $\inputcov=I_d$ we expect the behavior to persist for arbitrary
% diagonal $\inputcov$ with effective dimensionality asymptotically
% proportional to the sample size, i.e. $\trace(\inputcov)/n \to\gamma$.
% We leave the analysis of the more general case to future work.


% In order to understand the consequences of the theorem, we refer to the
% theoretical predictions plotted in Figure \ref{fig:lra} that show both the
% asymptotic standard and robust risk in Theorem \ref{thm:main_thm_lr} for
% different over-sampling ratios $\gamma$ and ridge-regularization parameter
% $\lambda$.  \fy{On the left hand side is noise standard double descent curve as
% in Hastie. Regularization helps! Right hand side - persists even without noise!}
% Note that as $\gamma$ increases beyond the interpolation threshold at $d = n$,
% the effect of regularization for the robust risk does not vanish as opposed to
% the standard risk.

% First note that both risks behave similar in the underparametirzed regime
% where $\gamma \leq 1$ and diverge at $\gamma =1$.  surprisingly we observe
% that the effect of regularization does not vanish for the robust risk when
% increasing $\gamma$. We can make the same observation also in Figure
% \ref{fig:lrb} where the curves are shown for noiseless observations. In this
% case the standard risk never benefits form regularization while we can clearly
% see that regularization helps the robust risk in the overparametrized regime.


\begin{figure*}
  \centering
  \includegraphics[width=5.5in]{figures/linreg_theory_legend.pdf}
  \begin{subfigure}[b]{3.15in}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/linreg_increasing_fit.pdf}
    \caption{Robust risk as $\lambda$ increases}
    \label{fig:linreg_increasing_fit}
  \end{subfigure}
  \begin{subfigure}[b]{2.25in}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/linreg_gammacurves.pdf}
    \caption{Orthogonal and parallel parameter error}
    \label{fig:tradeofflinreg}
  \end{subfigure}
  \caption{
    %% \at{I would swap a and b; it feels more natural to introduce the
    %% tradeoff between the two terms first and then talk about lambda opt}
    %% \ma{This is the old caption only for \ref{fig:tradeofflinreg}.  Needs to be
    %%   updated.}
    Theoretical curves for the robust risk with $\epstest=0.4$ (a) and decomposed terms (b) as $\lambda$ increases (arrow direction), for different choices of the overparamterization ratio $d/n\to\gamma$. We see in (b) that for large $\gamma >1$, as $\lambda$ increases, the orthogonal error $\|\Proj_\perp \thetalambda\|_2$ decreases whereas the parallel error $\|\thetatrue - \Proj_\parallel \thetalambda\|_2$ increases. For $\eps>0$, the best $\lambda$ is chosen at a large $\lambda$ that prevents interpolation.\vspace{-0.1in}
  }

  %%   Relation between the key quantities of the robust risk for
  %%   standard ridge regression estimators in the noiseless case.  Each dashed
  %%   line corresponds to the trajectory of the risk terms for a fixed $\gamma$ as
  %%   the ridge parameter $\lambda$ increases.  The slide lines correspond to the
  %%   $\lambda$ which minimize the robust risk for fixed test attack strengths
  %%   $\epstest$ as a function of $\gamma$.  The arrows denote the direction of
  %%   increase for both types of trajectories.  \rh{As the curve show, ...
  %% conclusion/take-away here} }

  \label{fig:linreg_noiseless_theory}
\end{figure*}

\subsection{Intuitive explanations and discussion}

We now shed light on the phenomena revealed by
Theorem~\ref{thm:main_thm_lr} and Figure~\ref{fig:main_thm_lr}.
In particular we discuss why regularization can
reduce the robust risk even in a noiseless setting
and why the effect is not noticeable for the standard risk.

% We now give insights explaining why the robust error overfits even in the
% noiseless case.  As shown in Figure~\ref{fig:lrb}, in this setting, the standard
% risk does not benefit from regularization, while we can clearly see that it
% improves the robust risk.
% This phenomenon is exclusively an issue in overparameterized regimes for
% noiseless observations, as illustrated in Figure~\ref{fig:lrb}. In this case
% the standard risk never benefits from regularization while we can clearly see
% that regularization helps the robust risk.

For this purpose, we examine the robust risk as a function of
$\lambda$, depicted in Figure~\ref{fig:linreg_increasing_fit} for
different overparameterization ratios $\gamma>1$ and $\epsilon=0.4$.
In order to understand the overfitting phenomenon, we decompose the
ridge estimate $\thetalambda$ into its projection
$\Pi_{\parallel}$ on the ground-truth direction $\thetatrue$ and its
projection $\Pi_\perp$ onto its orthogonal complement,
i.e., $\thetalambda = \Pi_\parallel \thetalambda + \Pi_\perp
\thetalambda$.
%% onto to the direction ground truth $\thetatrue$
%% Let $\Pi_{\parallel}$ be the orthonormal projection onto the ground truth
%% $\thetanull$, and let $\Pi_{\perp}$ be the projection on its orthogonal
%% complement. Basic algebra yields that we can decompose the estimator
%% $\thetalambda$ into orthogonal components $\thetalambda = \Pi_\parallel
%% \thetalambda + \Pi_\perp \thetalambda$, and,
%% As a straight-forward extension of
%% Lemma 3.1 in \cite{Javanmard20a} \fy{sorry isn't that kinda obvious and not worth mentioning javanmard?},
For the noiseless setup ($\sigma^2=0$), the closed-form expression of the consistent robust risk involves the parallel error $\|\thetanull - \Pi_{\parallel} \thetalambda\|_2^2$ and the orthogonal error $\|\Pi_{\perp} \thetalambda\|_2^2$ as follows:
%% \rh{We can have $\epstest=\epsilon$ throughout, right? Let's please do that if possible, and note that this is important below where the RHS uses $\epstest$ but the LHS uses $\epsilon$.
%% }
\begin{align}
  \label{eq:ARnoiseless}
% \SR(\thetalambda) &=  \|\thetanull - \Pi_{\parallel} \thetalambda\|_2^2 + \|\Pi_{\perp} \thetalambda\|_2^2 \\
  \AR(\thetalambda) &=  \|\thetanull - \Pi_{\parallel} \thetalambda\|_2^2  + (1+\epstest^2) \|\Pi_{\perp} \thetalambda\|_2^2 + \sqrt{\frac{8 \epstest^2 }{\pi} \|\Pi_{\perp} \thetalambda\|_2^2 (\|\thetanull - \Pi_{\parallel} \thetalambda\|_2^2 + \|\Pi_{\perp} \thetalambda\|_2^2 )}
\end{align}

The proof can be found in \suppmat{}~\ref{sec:linrobrisk}.
% \fy{TODO ???- write
% Lemma}
As $\lambda$ increases, Figure~\ref{fig:tradeofflinreg} shows that the parallel error increases faster than the orthogonal error decreases.
% \fy{some
% detail how we drew Figure}
When the perturbation strength $\epstest$ is large
enough, we see in expression~\eqref{eq:ARnoiseless} that the orthogonal error is
weighted more heavily. Hence, for the robust risk, some nonzero $\lambda$ that
\emph{prevents interpolation} yields the best trade-off. On the other hand the
standard risk with $\epstrain =0 $ weighs both errors equally, resulting in an
optimum at $\lambda = 0$.

% \fy{discussion on linf - The phenomenon also happens for linf and it's future work to prove it}
%% \paragraph{Implicit bias} \fy{wondering whether we should put that in some
%% discussion section cause its easier to start with logreg and then link to
%% linreg} We emphasize that the \emph{robust overfitting} phenomenon occurs for
%% all unit-norm ground truth vectors $\thetatrue$ as long as the data is
%% effectively high-dimensional, that is $\frac{\trace(\inputcov)}{n}\to \gamma >
%% 1$. In the case of a sparse ground truth, $\ell_2$-based inductive biases do not
%% lead to consistent solutions for large $\gamma$ and hence, we cannot recover the
%% $d$-dimensional $\thetatrue$ from only $ n < d$ samples. However, experiments
%% show that interpolation is not harmful, provided that we induce the right
%% implicit bias, e.g.\ by taking the minimum $\ell_1$ norm interpolator for a
%% sparse ground truth (see Appendix~\ref{sec:linregl1}). In conclusion, in the
%% overparameterized regime, overfitting may occur for the robust risk when the
%% implicit bias of the interpolator does not match the structure of the ground
%% truth.



%% on how generic the phenomenon of
%% \emph{robust overfitting} is. First of all, we observe robust overfitting for all
%% unit-norm ground truths vectors $\thetatrue$, independent of their sparsity.
%% %\fy{discuss how generic this observation is wrt different GT $\ell_p$ etc.}
%% \fy{need experiment for this}


%% The minimum norm solution $\thetaminnorm$ is a projection of
%% $\thetastar$ onto the column space of the design matrix $X^\top =
%% [x_1, ..., x_n] \in \R^{n \times d}$. Since in the overparameterized
%% regime the column space is at most $n$-dimensional, i.e.\ $rank(X) \le
%% n < d$, the two orthogonal components $\Pi_\parallel \thetaminnorm$
%% and $\Pi_\perp \thetaminnorm$ are nonzero.  Ridge regularization
%% prevents interpolation by shrinking the norm of the estimator
%% $\thetalambda$, for $\lambda > 0$. Hence, as $\lambda$ increases, the
%% error in the orthogonal subspace $\|\Pi_\perp\thetalambda\|_2$
%% shrinks, the error $\|\thetatrue - \Pi_\parallel\thetalambda\|_2$ in
%% the direction of $\thetatrue$ increases.




%% We illustrate the resulting trade-off between the two terms
%% $\|\thetanull - \Pi_{\parallel} \thetalambda\|_2^2$ and $\|\Pi_{\perp}
%% \thetalambda\|_2^2$ in Figure~\ref{fig:tradeofflinreg} where the arrow
%% indicates increasing $\lambda$ and the solid lines correspond
%% to different choices of the overparameterization ratio $\gamma$.
%% %% % \fy{we don't talk about this}
%% For the standard risk, the error reduction for high $\lambda$ via $\|\Pi_\perp\thetalambda\|_2$
%% is balanced out by the error gain  $\|\thetatrue -
%% \Pi_\parallel\thetalambda\|_2$  and hence the
%% the optimal standard risk is achieved for $\lambda = 0$.
%% %and hence the interpolating minimum norm solution dominates the ridge
%% %estimate $\thetalambda$ for any $\lambda > 0$.  Because consistent
%% %adversarial attacks are only caused by the orthogonal projection
%% %$\Pi_{\perp} \thetahat$,
%% The robust risk~\eqref{eq:ARnoiseless} however weighs the term
%% $\|\Pi_{\perp} \thetahat\|_2^2$ more heavily. Consequently, a higher
%% ridge penalty $\lambda>0$ that \emph{prevents} interpolation
%% optmizes the trade-off for the robust risk. Furthermore,
%% the optimal penalty increases with the overparameterization ratio $\gamma$ (see
%% Figure~\ref{fig:lambdaopt}).




%% At a fundamental level,
%% different evaluation metrics require estimators with a certain
%% structure (in this case, the optimal robust risk requires low
%% $\|\Pi_{\perp} \thetahat\|_2^2$ norm) and interpolation alone cannot
%% always find the best solution, even when it is not impaired by noise
%% in the observations. Therefore, in the overparameterized regime,
%% explicit regularization serves as a means to select predictors with
%% the appropriate implicit bias demanded by the task at hand.
% The robust risk in equation \eqref{eq:ARnoiseless} however, weights the term
% $\|\Pi_{\perp} \thetahat\|_2^2$ more heavily and hence achieves the optimal
% trade-off for a nonzero ridge penalty that \emph{prevents} interpolation.




%%%%%%%%%%%%%%%%%% OLD STUFF %%%%%%%%%%%%%%%%%%%%%
%% \paragraph{Standard estimator} For a given loss function ${\lossf: \YY \times
%% \YY \to \RR}$ the standard estimator is a minimizer of the unregularized
%% empirical risk $\Lossfemp$, that is

%% \begin{equation}
%% \label{eq:SE}
%% \thetahat \in \arg\min_{\theta} \Lossfemp(\theta) \define \arg\min_{\theta} \frac{1}{n} \sum_{i=1}^n \lossf(\yhattheta(x_i), \y_i).
%% \end{equation}

%% We refer to optimizing this problem as standard training.  In the following, we
%% consider the squared loss $\lossf(\yhat,y) = (\yhat-y)^2$ for regression and the
%% logistic loss $\lossf(\yhat,y) = \log(1+\exp(-\y\yhat))$ for classification.

%% The solution in Equation \eqref{eq:SE} may be non-unique if there exists a
%% sequence of estimators $\thetahat$ achieving vanishing empirical risk $\Lossfemp
%% \to 0$.  In this case, we define the standard estimator to be the min norm
%% interpolator for regression and the max margin interpolator for classification:

%% \begin{align}
%%   \label{eq:minnorm}
%%   &\mathrm{min~norm~interpolator}~ &\thetahat
%%   \define \arg\min_{\theta} \|\theta\|_2 ~~\mathrm{such~that}~~
%%   \yhattheta(x_i) = \y_i ~~\mathrm{for~all}~ i\\
%%   \label{eq:maxmargin}
%%   &\mathrm{max~margin~interpolator}~ &\thetahat
%%   \define \arg\min_{\theta} \|\theta\|_2  ~~\mathrm{such~that}~~
%%   ~\y_i \yhattheta(x_i) \geq 1 ~~\mathrm{for~all}~ i
%% \end{align}

%% These solutions have a special relevance as they correspond to the solution
%% obtained when running gradient descent on the loss form Equation \eqref{eq:SE}.
%% The proof for the min norm interpolator follows from a standard argument as
%% discussed in  the paper \cite{Hastie19} and the proof for the max margin
%% interpolator can be found in the paper \cite{Ji19}.  We remark that in
%% classification the sole quantity of interest is the signum of the predictions
%% $\sgn(\thetahat^\top x)$.  Hence, while the max margin interpolator in Equation
%% \eqref{eq:maxmargin} fails to attain zero empirical risk on a training set, we
%% can arbitrarily rescale the estimator without changing its predictions such that
%% the empirical risk vanishes.


==> Neurips_submission_version/log_reg.tex <==
\vspace{-0.1in}
\section{Regularization for logistic regression}
\label{sec:logreg}

In this section, we show that the max-margin solution
(corresponding to $\lambda \to 0$ in $\empriskrob$~\eqref{eq:AR}
for the logistic loss with $\ell_{\infty}$-attacks)
yields worse generalization than when choosing $\lambda >0$.
%% non-interpolating solution obtained
%% via a nonzero $\ell_2$  enalty.  We show this for logistic regression by
We derive precise asymptotic predictions
that show a systematic benefit
for the standard and robust risk
under $\ell_2$ regularization
when $d, n \to \infty$ and $d/n \to \gamma$.
%% and show that they are
%% matched by experiments for finite $d$ and $n$. W
We explain this phenomenon by arguing that unexpectedly, for the $\ell_\infty$ robust
logistic loss, a large $\ell_2$ penalty in fact enhances the
%to the (adversarial) logistic loss enhances the
bias of the estimator towards approximately sparse solutions.  As a
consequence, for a sparse ground truth, both the robust and standard
risk benefit from a non-zero regularization parameter.

%% Furthermore, we provide intuitive explanations on the role of regularization for the problem that we study.
%% \rh{Instead of ``intuitive explanation'', better summarize in a sentence what the explanation is.}


\begin{figure*}
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=2.6in]{figures/logreg_theory_combined.pdf}
    \caption{Fixed $n,d$ vs asymptotic predicitons}
    \label{fig:logreg_theory_combined}
  \end{subfigure}
  \begin{subfigure}[b]{0.48\textwidth}
      \centering
      \includegraphics[width=2.6in]{figures/logreg_explanation_standard_and_robust_risk.pdf}
      \caption{Risks of $\thetaepslambda$}
      \label{fig:logreg_explanation_standard_and_robust_risk}
  \end{subfigure}
  \caption{
      (a) The markers show the robust and standard risks for empirical training
      using $n = 1000$ and $\epstrain = 0.05$ when interpolating ($\lambda =0$) and regularizing ($\lambda = 1$).
      Additionally, the lines display the corresponding asymptotic theoretical predictions
      from Theorem \ref{theo:logreg}.
      (b) The training losses, robust risks and standard risks of empirical simulations
      with $\eps =1$ and $n =1000$, plottet with respect to increasing $1/\lambda$.
      Both figures demonstrate that regularization improves the robust and standard risk.
      See \ref{sec:appendix_experiments} for experimental details.\vspace{-0.2in}
  }
  \label{fig:logreg_theory}
\end{figure*}


\subsection{Problem setting}

We consider a discriminative data-generating model for classification
with isotropic Gaussian features $x\sim \Normal(0,I_d)$. Since the
focus of this paper is on interpolation with noiseless data,
we observe deterministic ground truth labels $\sgn \langle \thetatrue,\x \rangle$ for all covariates $x\in\R^d$ and fixed vector $\thetatrue$ in this section.
% %observations conditioned on $x_i$,
% given by $\langle \thetatrue,\x \rangle$ where $\thetatrue$ is the
% ground truth.
We refer to \suppmat{}~\ref{sec:logregnoise}, \ref{sec:logregtheory} for results
under observation noise.

We illustrate the phenomenon of robust overfitting for consistent
$\ell_\infty$ perturbation sets $\pertset{\infty}(\eps)$,
%(i.e., we choose $p=\infty$ in the robustrisk~\eqref{eq:AR}),
a standard choice in the experimental and
theoretical classification literature
\cite{Goodfellow15,Javanmard20b,Rice20,Sanyal21}.
%% For image classification, where adversarial robustness was first brought to
%% attention, a popular choice of attack motivated by security arguments are
%% imperceptible (and hence consistent) $\ell_\infty$ perturbations~\cite{Goodfellow15}. We adopt this
%% choice of adversarial attack for the evaluation metric in our analysis, that is
%% we choose $p=\infty$ in the adversarial risk defined in Equation~\eqref{eq:AR}.
Similar to linear regression, the adversarially robust risk computed
with such perturbation sets can be shown to upper bound the
distributionally robust risk with respect to mean shifts (see
\suppmat{}~\ref{sec:dro}) so that adversarial robustness implies
distributional robustness.

%% in~\eqref{eq:DR} when
%% $\probspace$ includes all \fy{actually might not need normal, just
%%   same covariance etc.} normal distributions $\Normal(\mu,\inputcov)$
%% with mean $\langle \mu, \thetastar \rangle=0$ and
%% $\rho(\probx,\probrobx)=\|\mu(\probx)-\mu(\probrobx)\|_\infty$ (see
%% Lemma~\ref{lem:dro}).
We consider the scenario where the ground truth has inherent
low-dimensional structure in the form of sparsity $\thetastar =
(1,0,\dots,0)^\top$. As we discuss later in this section, $\linf$
robustness and sparsity via its convex surrogate, the $\lone$
norm, are related objectives. Nonetheless,
we show that the inductive bias of the $\ell_\infty$ robust logistic loss with $\lambda \to 0$
(that is the robust max-margin solution)
is imperfect and that alternatively choosing a non-zero $\ell_2$ penalty
surprisingly promotes better sparsity and generalization.
%% the structural bias via
%% adversarial training is imperfect and we show that by preventing the estimator to converge to the max margin solution, $\ell_2$~regularization improves robust and standard generalization.

%% In the overparameterized regime, even if noiseless data is available, it is only
%% possible to recover the ground truth if it satisfies certain structural
%% assumptions. One popular example of such structure %that has been studied extensively
%% is sparsity, and hence, we assume the ground truth to be $\thetastar =
%% (1,0,\dots,0)^\top$. As we discuss later in this section, $\linf$ robustness and
%% sparsity via its convex surrogate, i.e.\ the $\lone$ norm, are related
%% objectives, which further motivates this choice of perturbations.
%% \fy{it seems about backwards, the motivation}

% \fy{maybe some discussion about That goes sth like:} In overparameterized
% regime, we can only try to recover, even in the noiseless case, if we encourage
% some structure. One of the most studied structural assumptions is sparsity and
% min $\ell_1$ norm, which is also what makes $\ell_\infty$ perturbations
% reasonable. Hence we assume a sparse ground truth $\thetastar =
% (1,0,\dots,0)^\top$.  \fy{just weird that we don't have the discussion in
% linreg}

\subsection{Interpolating and regularized estimators}

For training, we consider
the common $\ell_2$-regularized robust logistic regression estimate
that corresponds to Equation~\eqref{eq:ridgeloss} by choosing $\losstrain$ to be the logistic loss:
%$\losstrain(u,v) = \log(1+\exp(-uv))$. With a slight abuse of notation, we write $\losstrain(u) = \log(1+\exp(-u))$ so that
%the
%% for training standard regularized logistic regression
%% where in equation~\eqref{eq:ridge}, we choose $\lossf(u,v) = \log(1+\exp(-uv))$
%% and a slightly different perturbation set than for evaluation that is $\pertset(\epsilon)=\{\delta\in \R^d: \|\delta\|_\infty \leq \epsilon\}$,
%% \rh{Please justify as discussed in the call}
%minimizer of the empirical loss that corresponds to~\eqref{eq:ridge} takes the
%following form: \at{we should have $p$ as a subscript of $\pertset$}
\begin{equation}
  \label{eq:logridge}
  \thetaepslambda \define \arg\min_\theta \frac{1}{n}\sum_{i=1}^n \max_{\delta \in \pertset{\infty}(\epstrain)}\log(1 + e^{-\langle \theta, x_i+\delta\rangle y_i}) + \lambda \|\theta\|_2^2.
\end{equation}
%with $\lossf(u) = \log(1+\exp(-u))$.
% corresponding to (consistent)
% $\ell_\infty$-adversarial training.
As $\lambda\to 0$, we obtain the max-margin estimator~\cite{Rosset04}
on consistent perturbation sets of the training data
\begin{equation}
  \label{eq:maxmarginAE}
  \thetaeps \define \arg\min_{\theta} \|\theta\|_2
  ~~\mathrm{such~that}~~ \y_i \langle \theta, x_i\rangle - \epstrain \|\Proj_\perp \theta\|_1  \geq 1
   ~~\mathrm{for~all}~ i,
\end{equation}
where $\Proj_\perp$ is the projection onto the orthogonal complement of $\thetatrue$.
Similar to linear regression, this estimator is of particular interest since it
corresponds to the gradient descent solution of the
unregularized loss with $\lambda =0$ (see for example \cite{Ji19,Soudry18}, \cite{Javanmard20b}).


We recall that we focus on noiseless training to disentangle the effect of
noise from finite-sample effects. This also motivates why we
not only evaluate with consistent attacks but also train with
consistent adversarial perturbation sets: by definition,
for points close to the true decision boundary (which are likely in our data model),
$\ell_p$ perturbed points parallel to $\thetatrue$ cross
the true decision boundary. Hence, the ground truth does not achieve
$100\%$ robust accuracy on the training dataset.
Nonetheless, we also include a discussion on inconsistent adversarial
training in \suppmat{}~\ref{sec:inconsistent} for completeness
and show that it behaves similarly to training with consistent perturbation sets.
%
% Recall that we focus on noiseless training to disentangle the effect of
% noise and the finite-sample effects. This also motivates why we
% not only evaluate with consistent attacks but also train with
% consistent adversarial perturbation sets: by definition,
% for points close to the true decision boundary (likely in high dimensions),
% $\ell_p$ perturbed points parallel to $\thetatrue$ might cross
% the true decision boundary and a different ground truth label.
% Nonetheless we also include a discussion in
% Section~\ref{sec:inconsistent} on inconsistent adversarial
% training for completeness and show that it behaves similarly to
% consistent perturbation sets.

%% Recall that we limit ourselves to consistent perturbations
%% noiseless training loss to also exclude any noise emerging from the
%% training procedure. In practice, consistent adversarial training is
%% infeasible (because we don't know the ground truth) and instead
%% inconsistent attacks are a popular choice. Although inconsistent
%% attacks inject additional noise during training, we show in
%% Section~\ref{sec:inconsistent} that the effect of this is very mild
%% and is not mitigating robust overfitting.

%% Recall that we would like to investigate
%% interpolation \fy{redefine} on observations that consist of correct and consistent ground truth signals. This is the reason why we choose to study consistent perturbations
%% that are orthogonal to the ground truth $\thetatrue$ and hence result in the same
%% ground truth label as the unperturbed input. In practice, consistent
%% adversarial training is infeasible and instead inconsistent attacks are a popular choice. Although these attacks inject some additional noise during training, we show in Section~\ref{sec:inconsistent} that the effect is only very mild and in particular not mitigating robust overfitting.
% \fy{also have theory}, that robust overfitting also occurs in that case.
%

%% we consider consistent perturbations $\pertset{\infty}(\epsilon)$ that
%% provides correct ground truth signals, i.e. additive perturbations
%% that are orthogonal to the ground truth $\thetatrue$ and hence result in the same
%% ground truth label as the unperturbed input.
%If interpolating the consistent signals hurts generalization

%% In the low-sample regime,
%% standard training with $\epstrain=0$ yields solutions with an
%% extremely high robust risk even for optimal regularization \rh{would
%%   be good to have a citation or reference to an experiment here, or we
%%   can just not have this sentence, if the sentence is only to motivate
%%   robust training}. Therefore,
%% We perform adversarial training with
%% the usual choice $\epstrain=\epstest$ in order to obtain a more robust
%% estimator.

% In Section~\ref{sec:logreg_discussion}
% we argue that, if the ground truth is sparse, then adversarial training with
% $\linf$ perturbations benefits even the
% standard risk. When $\epstrain$ is sufficiently small (see
% Proposition~\ref{prop:gammastar}), the $\epstrain$-max-margin estimator
% \begin{equation}
%   \label{eq:maxmarginAE}
%   \thetaeps \define \arg\min_{\theta} \|\theta\|_2
%   ~~\mathrm{such~that}~~ \y_i \langle \theta, x_i\rangle - \epstrain \|\Proj_\perp \theta\|_1  \geq 1
%    ~~\mathrm{for~all}~ i
% \end{equation}
% exists and, as $\lambda\to 0$, the $\ell_2$-regularized robust logistic regression estimate $\thetaepslambda$
% converge to $\thetaeps$.
% Similar to linear regression, this estimator corresponds to the gradient descent solution of the
% unregularized loss (i.e.\ with $\lambda =0$) (see e.g. \cite{Ji19,Soudry18}, \cite{Javanmard20b})
% and is therefore of
% particular interest.
%  \fy{not entirely proven}.

%% \rh{The paragraph below is very unclear. ``Consistent perturbations'' needs to be defined or it needs to be recalled what they are. Also ``showing X is more surprising'' and ``should imply'' is too vague to be appropriate language for a paper. Either we can say something concrete here, or not.}
%% \fy{this is similar to a current footnote earlier} Note that training with
%% consistent perturbations is not feasible, since it requires knowledge of the
%% ground truth linear predictor. However, showing robust overfitting for
%% consistent perturbations is more surprising and should imply overfitting for
%% inconsistent perturbations (see Section~\ref{sec:inconsistent} for a more
%% detailed discussion).

%% Analogous to the literature,
%% we sometimes refer to $\thetaepslambda$ and $\thetaeps$ for $\epstrain >0$ as
%% the estimator obtained via \emph{adversarial training}.
%% \fy{something about
%%   $\epsilon=0$ not achieving good solutions, even true for standard
%%   risk?}



%% \footnote{Note that these are inconsistent perturbations since during training
%% we do not have access to the feasible set of $\pertset(\epsilon)$ unless we
%% know the direction of the ground truth $\thetatrue$.}

%% In what follows we choose $\epstrain>0$ to be
%% such that an adversarially interpolating estimator exists that achieves
%% vanishing loss for $\lambda=0$.
%% \begin{equation}
%%   \label{eq:adv_interpolate}
%%   y_i \max_{\delta \in \pertset(\epsilon)} \langle \thetaepslambda,x_i+\delta \rangle \geq 1 \:\: \text{for all }i.
%% \end{equation}
%% .




\subsection{Main results and experiments}
We now present an informal statement describing the asymptotic standard
and robust risk for linear classification with the logistic loss as
$d,n\to\infty$. We refer to
\suppmat{}~\ref{sec:logregtheory} for the precise statement and the proof.
The latter is inspired by the works \cite{Javanmard20b,Salehi19} and
uses the Convex Gaussian Minimax
Theorem~(CGMT)~\cite{Gordon88,Thrampoulidis15}.


\begin{theorem}[Informal]
  \label{theo:logreg}
Assume that $\eps = \epsnull/\sqrt{d}$ for some constant $\epsnull$ independent of $n,d$ and
$\thetastar = (1,0,\cdots,0)$.
Then, the robust and standard risks of the ridge regularized estimator
$\thetaepslambda$ with $\lambda \geq 0$ converge in probability as $d,n \to \infty$, $d/n \to \gamma$
 \begin{align*}
 \SR(\thetaepslambda) &\to \frac{1}{\pi}\arccos\left(\frac{\nupar^\star}{\nu^\star}\right) ~~\mathrm{,}~~
  \AR(\thetaepslambda) \to \frac{1}{\pi}\arccos\left(\frac{\nupar^\star}{\nu^\star}\right) +  \frac{1}{2} \erf\left(\frac{\epsnull \delta^\star}{\sqrt{2} \nu^\star}\right) + I\left(\frac{\epsnull \delta^\star}{\nu^\star}, \frac{\nupar^\star}{\nu^\star}\right)
\end{align*}
with $\erf$ the error function,
\begin{equation*}
 I(t,u) \define \int_{0}^{t} \frac{1}{\sqrt{2\pi}} \exp\left(-\frac{x^2}{2}\right)\erf\left(\frac{x u}{\sqrt{2(1- u^2)}}\right)dx
\end{equation*}
% \begin{align}
%  \|\Piper \thetaepslambda \|_2 \to \nuper^\star, ~~~~
%  \| \Pipar \thetaepslambda \|_2 \to  \nupar^\star, ~~~~ \mathrm{and}~~~~
%  \|\Piper \thetaepslambda \|_1 \to \delta^\star,
% \end{align}
and where $\nu^\star = \sqrt{(\nuper^\star)^2 + (\nupar^\star)^2}$, and $\nuper^\star,\nupar^\star,\delta^\star$ are the unique solution of a scalar optimization problem specified in Appendix~\ref{sec:logregtheory} that depends on $\thetatrue, \gamma, \epsnull$ and $\lambda$.
%Let $\gamma^\star$ be the asymptotic
%interpolation threshold from Proposition \ref{prop:gammastar} and
%$(\nuper^\star,\nupar^\star,\delta^\star)$ be given by the unique solution of
%one of the following scalar optimization problems:
%\begin{enumerate}
% \item The problem in Equation \eqref{eq:nonseperable} if $\lambda > 0$ or $\gamma < \gamma^\star$
% \item The problem in Equation \eqref{eq:seperable} if $\lambda = 0$ and $\gamma > \gamma^\star$
%\end{enumerate}
\end{theorem}


We illustrate the consequences of this theorem in
Figure~\ref{fig:logreg_theory_combined} where we plot the standard and
robust risk obtained by the asymptotic theoretical predictions for
$d,n\to\infty$ and simulations for $n=1000$ and $\eps = 0.1$.
%% the robust risk
%% $\AR$ of $\thetaepslambda$ for $c = \sqrt{1000} \sqrt{\gamma} 0.01$
%% (corresponding to $\epsilon=0.1$ if $n=1000$)
The theoretical curves are obtained by solving the scalar optimization
problem specified in Appendix~\ref{sec:logregtheory};
the empirical setup is described in Appendix~\ref{sec:appendix_experiments}.
%% In addition, we show the empirical
%% predictions for $n =1000$ and $\epstrain=0.1$
%\kd{michael can you add  a sentence here how you get it. I.e. using the optimizer bla}.
%of the different optimization problems that can be constructed for each value of $d/n$.
%\footnote{We refer the reader to Section~\ref{sec:logregopt} for details on the procedure used to solve the optimization problems.}
We observe that the precise asymptotics indeed predict benefits of
regularization for adversarial logistic regression.
This trend is further supported by our simulation results closely following
the theoretical curves.
%% and empirical curves that the
%% regularized estimator $\thetaepslambda$ achieves a significantly
%% better population risk than the interpolating estimator $\thetaeps$.
Even though the standard risk also benefits from regularization in
our setting, the gains for the robust risk are more significant and
increase with the overparameterization ratio.

Finally, in Figure
\ref{fig:logreg_explanation_standard_and_robust_risk} we observe for a
fixed overparameterization ratio $d/n$ how optimizing the average
adversarial logistic loss beyond $100\%$ training accuracy
substantially hurts generalization.
%% That is, for high-dimensional
%% noiseless and consistent $\ell_\infty$ adversarial perturbations with
%% a sparse ground truth, the max-margin solution is not desirable and
%% hence,
In particular, this challenges the common belief
that training overparameterized classifiers
even beyond the point of achieving $100\%$ training accuracy
improves generalization.
%% underlines this observation by empirically showing that for a fixed
%% $\gamma$, both the robust and standard risk increase when decreasing
%% $\lambda$. \kd{not sure what to say about the train loss here}.
%% \subsection{Early stopping.}
%In this section, we focused on explicit $\ell_2$-regularization
Even though the theory and simulations in this section are for
varying $\lambda$, we show in \suppmat{}~\ref{sec:gdlogreg}
that the same trends as for $1/\lambda\to \infty$
can be observed epoch-wise when training with gradient descent
as the epochs $t\to \infty$ .
%% : When initializing at zero, there are two phases where
%% we first obtain a sparse solution matching the ground truth well. When
%% training for longer, the estimator then approaches the max margin
%% solution and suffers form the same issues as when decreasing
%% $\lambda$.
We leave the proof for the benefits of early stopping as interesting future
work.
%% Yet, the connections
%% between early stopping and $\ell_2$ regularization are not yet well understood
%% compared to linear regression and that is interesting future work.



\begin{figure}[tbp]
  \centering
      \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=1.8in]{figures/logreg_explanation_robust_margin_decay.pdf}
        \caption{Robust margin decay of $\thetaepslambda$}
        \label{fig:logreg_explanation_robust_margin_decay}
    \end{subfigure}
      \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=1.8in]{figures/logreg_explanation_margins.pdf}
        \caption{Robust margin of $\thetaepslambda$}
        \label{fig:logreg_explanation_margins}
      \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=1.8in]{figures/logreg_explanation_sparsity.pdf}
        \caption{Sparsity of $\thetaepslambda$}
        \label{fig:logreg_explanation_sparsity}
    \end{subfigure}
    \caption{
      (a) The ordered sample-wise penalized margin $\langle x_i, \theta\rangle - \epsilon\|\Piper\theta\|_1$ of the normalized estimator $\thetahat/\|\thetahat\|_2$ when interpolating and regularizing with $\lambda =5$.  For larger $\lambda$, the minimum margin is decreases while the average margin (horizontal lines) decreases. This trendis also observed in (b) where the minimum penalized margin (robust margin) and the average penalized margin as in (a) are plotted with respect to $1/\lambda$. The horizontal line is the corresponding average penalized margin of $\thetatrue$. (c) The $\ell_1$ norm of the normalized estimator increasing with $1/\lambda$. See \ref{sec:appendix_experiments} for experimental details. \vspace{-0.2in}
%     rescaled minimum margin and approximate sparsity. We use $n=10^3$ and $d/n=8$ and vertical line marks the point at which
%       $\thetalambda$ achieves standard interpolation i.e. $y_i \langle \theta,x_i\rangle >0$. We see that for a large enough $\lambda$ we achieve small risk and a sparse solution.
    }
    \label{fig:logreg_explanation}
\end{figure}


\subsection{Why regularization improves regularization}
\label{sec:logreg_discussion}

While Theorem~\ref{theo:logreg} specifies the precise asymptotic
behavior of the standard and robust risks and predicts the benefits
of regularization for generalization, it is hard to extract
intuitive insights directly from the proof.
Instead, in this section we provide intuition
for why a non-zero ridge penalty induces a sparser $\thetaepslambda$
than the $\ell_1$ penalized max-margin solution $\thetaeps$ and use
simulations to support our claims.

%than the unregularized robust logistic loss.
%% the result does not provide
%% insights on why regularization is beneficial.  In order to gain
%% intuition for this, we next show that, perhaps unexpectedly, the ridge
%% penalty induces a bias towards a sparse solution which in turn yields
%% an estimate $\thetaepslambda$ that better aligns with the sparse
%% ground-truth $\thetatrue$ than the unregularized estimate.

As shown in \suppmat{}~\ref{sec:logregtheory}, the unregularized and
consistent adversarial robust loss $\empriskrob$ with $\ell_\infty$
perturbations can be written as $\empriskrobunreg(\theta) =
\frac{1}{n}\sum_{i=1}^n \log (1 + e^{-y_i \langle \theta,x_i \rangle +
  \epsilon \|\Proj_\perp \theta\|_1})$.
%  with ${\lossf(u) =    \log(1+\exp(-u))}$ as before.
Hence, adversarial training with
$\linf$ perturbations penalize solutions with large $\ell_1$-norm,
which in turn is well known to encourage sparse solutions (see
\cite{Tibshirani96} and references therein). However, in contrast to
an explicit additive $\ell_1$ penalty, the $\ell_1$ term appears
inside the loss function. As illustrated in Figure
\ref{fig:logreg_explanation_sparsity}, this leads to the effect that
additionally regularizing with an $\ell_2$ penalty leads to a
smaller normalized $\ell_1$ norm and hence a sparser solution.


To gain intuition for this phenomenon, we consider two cases: large
$\lambda$ inducing small $\|\thetahat\|_2$ and small $\lambda$
inducing large $\|\thetahat\|_2$ solutions. As we argue below and
illustrate in Figure~\ref{fig:logreg_explanation_robust_margin_decay},
the former corresponds to large-average margin solutions whereas the
latter approaches a large-min margin solution for small enough
$\lambda$. Since the ground truth $\thetatrue$ is sparse and has a
small min-margin and large-average margin (horizontal dotted line in
Figure~\ref{fig:logreg_explanation_margins}) itself, the large-average
margin solution is likely to align better with the ground truth. Hence, we expect it to be sparse and have a low standard and robust risk. The improved sparsity is indeed observed in
Figure~\ref{fig:logreg_explanation_sparsity} and the corresponding
standard risk decrease is plotted in
Figure~\ref{fig:logreg_explanation_standard_and_robust_risk}.
%% large average-margin solution is sparser than the large max-margin
%% solution and by the standard risk plotted in
%% Figure~\ref{fig:logreg_explanation_standard_and_robust_risk} also
%% aligns better with the ground truth.
%% As we observe in Figure~\ref{fig:logreg_explanation_margins},
%% the ground truth indeed has large average margin (horizontal dotted line) and
%% corresponds well
%% to the regularized solution with large $\lambda$ that also has large
%% average margin. As $\lambda$ decreases, we approach the max margin
%% solution which has larger min-margin but smaller average margin.
%% For completeness, the distribution of the (ordered) margins for large
%% (red) and small (blue) $\lambda$ together with their average margins
%% (horizontal lines) is plotted in
%% Figure~\ref{fig:logreg_explanation_robust_margin_decay}. We can

We now reason why large $\|\thetahat\|_2$ leads to the max-min margin
solution. Due to the logistic loss, most training points have large
values $y_i\langle \thetahat, x_i\rangle$ for large $\|\thetahat\|_2$
and do not contribute to the loss. In contrast, small
$\|\thetahat\|_2$ lead to a large average-margin solution since
\emph{all training points} contribute to the loss, most easily seen
via the Taylor series expansion $\empriskrobunreg(\theta)\approx -
\frac{1}{n}\sum_{i=1}^n \y_i \langle x_i, \theta\rangle + \epstrain \|
\Pi_{\perp} \theta\|_1$.
%% \fy{could ditch what follows, quiet vague
%%   anyway} Finally, trading off the $\ell_1$ norm of $\thetahat$ with
%% the margins of all values naturally dominates trading off only with a
%% few points.

%% note that when the norm
%% $\|\thetahat\|_2$ is small (i.e., for large $\lambda$), all training
%% points will have non-zero contribution to the loss. Hence, the
%% $\ell_1$ penalty is traded off with the margin $y_i\langle
%% \theta,x_i\rangle$ of all points equally, most easily seen via the
%% Taylor series expansion ${\empriskrob(\theta)\approx -
%%   \frac{1}{n}\sum_{i=1}^n \y_i \langle x_i, \theta\rangle + \epstrain
%%   \| \Pi_{\perp} \theta\|_1}$.

%% However when the norm of the solution, $\|\thetahat\|_2$, is large
%% (i.e. for small $\lambda$), in the overparameterized regime, the
%% estimator $\thetahat$ maximizes the penalized margin, that is $ \min_i
%% y_i \langle \theta,x_i\rangle - \|\Piper \theta\|_1$. Figure
%% \ref{fig:logreg_explanation_robust_margin_decay} shows the tradeoff
%% between the normalized margin and averaged sample wise margin. Yet,
%% since for high $n$ we can always find samples $x_i$ arbitrarily close
%% to the decision boundary, the penalized margin of the ground truth is
%% approximately zero, which also explains the bad performance for large
%% $\lambda$ shown in Figure \ref{fig:logreg_explanation_margins}. On the
%% other hand, as illustrate in Figure
%% \ref{fig:logreg_explanation_margins}, the ground truth has a large
%% averaged penalized margin aligning well with the one of the estimator
%% for small $\lambda$.


==> Neurips_submission_version/new_intro2.tex <==
\section{Introduction}


Conventional statistical wisdom suggests that optimizing the data fit
by minimizing a loss $\Loss(\theta)$ with respect to parameters
$\theta$ should be exercised with care: if a global minimizer achieves
zero or near-zero training loss (i.e. it \emph{interpolates}), we run
the risk of overfitting (i.e.\ high variance) and thus sub-optimal
prediction performance.  \emph{Regularization} is commonly used to
reduce the effect of noise and to obtain an estimator with better
generalization.  Specifically, it induces worse data fit by limiting
model complexity, for example via an explicit penalty term
$R(\theta)$, which in turn imposes certain structural properties on
the minimizer of the penalized loss $\Loss(\theta) + \lambda
R(\theta)$.  This classical rationale, however, does not apply to
overparameterized models:
%% neural networks with large widths yield the same generalization performance
%% when $\Loss(\theta)$ vanishes as compared to 
Large neural networks, for example, have good generalization performance on
\iid{} samples when $\Loss(\theta)$ vanishes and label
noise is present~\cite{Nakkiran20}.

Since interpolators are not unique in the overparameterized regime, it
is crucial to study the \emph{implicit bias} of specific
interpolating estimators. A large body of recent work analyzes the
properties of the solution found via gradient descent at convergence
for common choices of $\Loss(\theta)$ (see
e.g.~\cite{Rosset04,Chizat18,Chizat20,Gunasekar18,Ji18,Ji19,Soudry18}).
\fy{i think we're not citing enough} For example, for linear and
logistic regression, it is well-known that gradient descent converges
to the minimum-$\ell_2$-norm and maximum-$\ell_2$-margin
solutions~\cite{Gunasekar18, Ji19,Lyu20,Soudry18}, respectively,
%These estimators also
that also correspond to the minimizers of the loss
$\Loss(\theta) + \lambda \|\theta\|^2_2$ in the limit of $\lambda\to
0$ \cite{Rosset04}.

How well do these specific interpolators generalize?
A plethora of recent papers explicitly study generalization properties
on min-norm interpolators
\cite{Dobriban15,Ghorbani19,Hastie19, Bartlett20,Mei19, Muthukumar20,
  Muthukumar20a} and max-margin solutions
\cite{Deng20,Muthukumar20,Salehi19} and show that the
variance decreases as overparameterization ratio increases.
Motivated by the double descent phenomenon \cite{Belkin18c},
most of them focus on settings where the optimal
regularization parameter $\lambdaopt \leq 0$ \cite{Kobak20, Wu20,
  Richards21}, implying that it is redundant or even
detrimental to explicitly regularize with $\lambda >0$.

The narrative that regularization is obsolete for large
overparameterized models %to achieve good performance
is drawn from theoretical and experimental findings that analyze the \emph{standard}
test risk. Since this measure of performance assumes identically
distributed training and test data however, it does not reflect the
\emph{robust risk} of models when the test data has a shifted
distribution, is attacked by adversaries, or primarily contains
samples from minority groups.
In fact, mounting empirical evidence suggests that regularization is indeed
helpful for robust generalization, even when it \emph{does not} benefit the
standard risk \cite{Rice20,Sagawa20a,Sagawa20b}.
This phenomenon is sometimes referred to as \emph{robust overfitting}.
% \fy{careful now it seems like definition of robust overfitting is s.t. not
% having standard overfitting}

In the presence of noise, the following intuition holds true:
since the robust risk amplifies estimation errors, its variance is larger
and hence regularization-- e.g. via early stopping-- can be beneficial for generalization \cite{Sanyal21}.
%% increases in the presence of noise, meaning that
%% %% one can argue that in the noisy case, the resulting parameter error
%% %% is amplified and hence
%% additional variance reduction techniques
%% like early stopping can help \cite{Sanyal21}.
%% The reason why robust risk can behave differently than standard risk
%% is that robust risk amplifies parameter errors. Now of course
%% interpolating noise increases parameter error and robust risk would
%% amplify that (Amartya style argument).
However, we observe that even when estimating entirely noiseless signals,
robust overfitting persists!
% \fy{that include adversarially robust losses $\Loss(\theta)$ (aka adv. training) thatlead to fitting imperceptible or consistent perturbation sets around original inputs (see Section~\ref{sec:setting} for clear motivation} In
In particular, we observe that for truly high-dimensional feature models,
the robust risk of minimum $\ell_2$ norm/max-margin interpolators
(i.e.\ $\lambda \to 0$) suffers from overfitting when compared to
explicit ridge regularization with $\lambda >0$ that prevents
interpolation. In Figure~\ref{fig:teaser} we provide three examples
including neural networks on sanitized image data linear models (see
Section~\ref{sec:appendix_experiments} for experimental details).


%% However, the implicit bias of gradient descent or equivalently,
%% $\ell_2$ penalty is unlikely to match the structure of the ground
%% truth.  As a consequence, even when there is no noise, $\lambda \to 0$
%% yields a estimator with high standard and robust risk. In such a case \fy{restate?}, can
%% increasing $\lambda >0$ actually improve generalization?
% In fact it is highly unlikely.
%% When the final solution of gradient descent equivalently or
%% $\lambda \to 0$ incurs a large error and we have noiseless signals,
%% would avoiding interpolation using early stopping help or $\lambda >
%% 0$ ?

To date, prior work does not predict nor explain our
observations. Further, they contradict a possible intuition for the
noiseless case: if the min $\ell_2$-norm and max-$\ell_2$-margin
interpolators have high risks as $\lambda\to 0$, the $\ell_2$-norm
induced bias is potentially suboptimal and hence increasing the
penalty weight $\lambda >0$ should only degrade performance.
%% trading off data fit for an
%% even smaller $\ell_2$ norm
%% In this paper, we study linear models for which intuition would
%% suggest that explicit regularization should degrade estimation performance on
%% noiseless data generated by a linear ground truth.
In this paper, we prove that this intuition in fact does not hold true
in general in the high dimensional overparameterized regime.
%% In the quest to disentangle the effects of noise and finite sampling \fy{high-dimensionality?},
As noise is known to have negligible effects in the overparameterized
regime, we focus on consistent training losses and noiseless
observations -- precisely the scenarios that are expected to benefit
the least from a non-zero $\ell_2$ penalty. In particular, we study
point-wise losses averaged over the original data points or consistent
adversarial perturbation sets around the training samples. For the
square and logistic loss with isotropic Gaussian covariates, we then
show that a strictly positive $\ell_2$ penalty leads to a systematic
improvement in robust generalization.  Our results provide the first
rigorous explanation for robust overfitting even in the absence of
noise.

%% and why early stopping may benefit the
%% robustness when it doesn't ... standard. \fy{a bit strong but ...}
%% \fy{argue that image data is noiseless?}
%% While our theoretical results focus on $\ell_2$ regularization, we empirically show that the same also hold for early stopping in Section \ref{sec:gdlogreg}. \fy{specific to logreg maybe not necessary?}
% We prove in contrast to common intuition,
%% in high-dim even for noiselss
%% there can be some parameter error since we don't have enough signal
%% (likely unless GD+model class happens to have the exact right/perfect
%% structural bias with). Ok, but now in this case, would it help to
%% early stop? Should we pick $\lambda \to 0$ or $\lambda > 0$?

%% A natural intuition is that when the signal is noiseless,
%% i.e., consistent with the ground truth, leveraging all signals perfectly
%% should only help to achieve best generalization. Even when there is
%% mismatch in the structural bias.
%% \rh{``leveraging all signals'', and ``even when'' (even when what?) is unclear.}
%% In this paper, we explicitly
%% contradict this intuition.
%% In fact, we are the first to prove for
%linear models, that in contrast to common intuition,
% \fy{now this is
%   tricky, we talked about GD and ES all the time, now suddenly l2, but
%   don't wanna spend time to introduce l2}
%% In contrast to common intuition,  using $\lambda >0$,
%% i.e. weighting an ``imperfect bias'' more, actually leads to \emph{better}
%% robust generalization. For logistic regression, regularization even
%% improves the standard $0-1$ risk. \kd{a bit too strong} From a dual perspective our results
%% also suggest that even when the signal in the loss
%% function is noiseless, it would be better to avoid interpolation
%% for generic distributions/models.

%% should be avoided and an ``imperfect
%% penalty'' should be weighted more even

In Section~\ref{sec:setting} we formally define the evaluation metrics and
training losses used to obtain interpolating and regularized estimators.
We then present our precise asymptotic results for the robust risk of
the minimum norm interpolator in Section~\ref{sec:linreg} and the
max-margin solution of the robust loss for logistic regression in
Section~\ref{sec:logreg}. In each section we also provide additional
insights to build intuition for the phenomenon of robust overfitting
occurring even in the noiseless and linear case.

%% In Section~\ref{sec:linreg} we give precise
%% asymptotics for the robust risk of the ridge estimator and the minimum
%% norm interpolator in the context of linear regression. In
%% Section~\ref{sec:logreg} we show that adversarial training for
%% logistic regression can benefit from a non-zero ridge penalty and
%% provide insights explaining this phenomenon.

\begin{figure*}
  \centering
  \begin{subfigure}[b]{1.8in}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_nn.pdf}
    \caption{Neural networks}
    \label{fig:teaser_plot_nn}
  \end{subfigure}
  \begin{subfigure}[b]{1.8in}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_linreg.pdf}
    \caption{Linear regression}
    \label{fig:teaser_plot_linreg}
  \end{subfigure}
  \begin{subfigure}[b]{1.8in}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_logreg.pdf}
    \caption{Linear classification}
    \label{fig:teaser_plot_logreg}
  \end{subfigure}

  \caption{
  In this plot we exemplify the benefits of early stopping (a) and nonzero $\ell_2$ regularization (b),(c)
    for the robust risk (robust risk decrease).
    The decrease is strictly positive across
    most overparameterization ratios $d/n$ even in the absence of noise.
    (a) Neural networks fit on (binary 1-3) MNIST that arguably
    has minimal noise compared to other image datasets
    and that we further sanitize.
    %% (b) gap
    %% between the standard and distributionally robust risk of the best
    %% regularized and final estimator for a (a) two-layer neural network
    %% with varying width, trained on (binary $1$-$3$) MNIST after using
    %% suggested variance reduction methods (see
    %% Appendix~\ref{sec:appendix_experiments}, regularized using early
    %% stopping .
    (b) Linear regression on noiseless observations for $n=1k$.
    (c) Adversarial training on logistic regression for $n=1k$.
    %% The
    %% robust risk benefits significantly from regularization.
    Note that for small $d/n$, adversarial training
    does not interpolate which leads to better robust accuracy
    %% logistic regression trained with noise is not
    %% capable to overfit the data which also explains why the
    %% overfitting gap when trianing with noise is initially smaller
    (see \suppmat~\ref{sec:logregnoise} for a more detailed discussion).
    Experimental details can be found in \suppmat~\ref{sec:appendix_experiments}.
    See Sections~\ref{sec:linreg} and \ref{sec:logreg} for the precise settings for (b) and (c).\vspace{-0.2in}
  }

  \label{fig:teaser}
\end{figure*}


==> Neurips_submission_version/setting.tex <==
\vspace{-0.1in}
\section{Risk minimization framework}
\label{sec:setting}

In this section, we describe the setup for our theoretical
analysis of linear and logistic regression.  We define the data
generating process, the standard and robust risks, and formally
introduce the estimators that we consider. We present general
concepts that apply for both regression and classification and follow
up with more specific details in the respective sections.

We consider the supervised learning problem of estimating a mapping
from $d$-dimensional real-valued features $x\in \R^d$ to a target $y
\in \YY \subseteq \R$, given a set of input-output pairs $\Traindata =
\{(\xind{i}, \y_i)\}_{i=1}^n$.
%with $(\xind{i}, \y_i) \in \R^d \times \YY$.
The data is generated by drawing $\numsamples$ \iid{} feature vectors
$x$ from the marginal distribution of the inputs $\probx$ and
observing targets $y$ that follow a conditional distribution depending
on the linear ground truth function $\langle \thetatrue, x\rangle$.
%% joint distribution
%% $\prob = \prob_X \prob_{Y\vert X}$. Intuitively, the predictor variable $Y$ is
%% generated from a deterministic linear function of the covariates $X$, i.e.\
%% $\langle \thetastar, X\rangle$, which we call the ground truth estimator, and
%% noise.
The exact expressions for regression and classification are given in
Sections~\ref{sec:linreg} and~\ref{sec:logreg}, respectively.

%\rh{The sentence below is not necessary, as this is introduced in the respective section on linear and logistic regression; ok to delete?}
%We assume that $\prob_X = \Normal(\mu,\inputcov)$ \fy{dependence on $\mu$?} and the conditional  distribution of $Y$ depends on $X$ via a linear function
%  $\ytrue(X) = \langle\thetatrue, X\rangle$ and \iid{} %random noise $\xi$.

%% More specifically, we focus on regression with $\YY = \R$ and binary
%% classification with $\YY = \{-1, +1\}$.  In the following we denote with
%% $\|\cdot\|_p$ the $\ell_p$ norm and with $\sgn$ the signum function.

Throughout this paper, we assume $\probx$ to be an isotropic Gaussian distribution,
and study the high dimensional asymptotic regime
where $d/n \to \gamma$ as both the dimensionality $d$
and the number of samples $n$ tend to infinity.
This regime \cite{Buhlmann11,Wainwright19} is widely studied as it yields
precise predictions for many real world problems
where both the input dimension and the data set size are large. It is
also the predominant setting considered in previous theoretical papers
that discuss overparameterized linear models~\cite{Ali20,Deng20,Dobriban15,
  Hastie19,Javanmard20a,Javanmard20b,Sur19}.
%   \fy{maybe cite more or sth? cause if you get reviewer}.
%
% Without loss of generality our analysis considers input distributions
% $\prob$ with identity covariance matrix. However, as we explain in
% Section~\ref{sec:highdim} our observations hold for any effectively
% high-dimensional setting, that is where
% $\frac{\trace(\inputcov)}{n}\to \gamma$. In the case where the input
% data is inherently low-dimensional classical asymptotic theory applies
% and

%% For an overview of this topic we refer to the standard
%% works \cite{Buhlmann11,Wainwright19} and references therein.




\subsection{\Natrisk{} and robust risk}


%% \rh{I think ``standard'' risk is more common than ``natural'' risk; Fanny can decide on what's better}
%% \fy{yes lets try standard since we don't mention standard training that much anyway!}
%% \fy{after writing, if you really want the denote all the risks with $f$ instead of $\langle\theta,x\rangle$
%%   thats also ok I guess - looks a bit more general and simple, potentially sells better, but is additional notation I guess}

% TODO: maybe we can move this to evaluation Further, for a ground truth vector
% $\thetanull \in \RR^p$ we denote with $\Pi_{\parallel} =
% \frac{\thetanull\thetanull^\top}{\|\thetanull\|^2_2} $ the projection onto the
% one dimensional subspace spanned by $\thetanull$ and by $\Pi_{\perp} =
% \idmat_d
% - \Pi_{\parallel}$ the projection onto the orthogonal subspace.

We now introduce the \natrisk{} and robust evaluation metrics for regression and
classification that we study in this paper. %\fy{Sometimes we also refer to standard as natural to avoid confusion with standard training - need to decide on this} \rh{let's use `standard' throughout. more confusing to use both standard and natural}
For a given test loss $\losstest \colon \R \times \R \to \R$, we define the \natrisk{} risk of an estimator
$\thetahat$ as
\begin{equation}
  \label{eq:SR}
  \SR(\thetahat) :=  \EE_{X\sim\probx} \losstest\left(\langle \thetahat, X\rangle, \langle
  \thetastar, X\rangle\right),
\end{equation}
%% We use two different evaluation metrics to capture different properties of
%% learned estimators: the standard risk and the robust risk.  Unless
%% otherwise stated we use the population variants of these quantities for our
%% theoretical analysis.  In practice, the population risks can be estimated on a
%% held-out test set drawn \iid{} from the training data distribution.
%% The standard risk assesses the prediction error of a model $\yhattheta$ and is
%% defined as
where the expectation is taken over the marginal feature distribution $\probx$.
Note that conditioned on the training data, this risk is fixed,
and our asymptotic bounds hold almost surely over draws of the training set. For
regression tasks we choose $\losstest(u,v)= (u-v)^2$ which yields the population
mean squared error, and for classification we choose the 0-1 loss
$\losstest(u,v) = \indicator_{\sgn(u) \neq \sgn(v)}$ which yields the
probability of making a classification error.

%Instead of finding an estimator with low standard risk,
As more ML models are productionalized, there are increasing requirements
on their robustness.
%Another desirable robustness property in the ML literature is
One popular notion is robustness with respect to
$\epsilon$-bounded $\ell_p$ perturbations with $p=2$ or $p =\infty$.
We assume that $\thetatrue$ is indeed robust to begin with, that is $\thetatrue$ minimizes the population robust risk (see also for example \cite{Raghunathan19}). The perturbations then have to be \emph{consistent} in the sense that they do not change the ground truth label.
%% \emph{consistent}
%% (``imperceptible'' for image) perturbations of the input data that do
%% not change the ground truth label. In the literature,
%% $\epsilon$-bounded $\ell_p$ perturbations, in particular for $p=2,
%% \infty$ are often studied for simplicity and for linear models,
%% consistent perturbations are restricted to the null space of the
%% ground truth $\thetanull$ \cite{Raghunathan19}.
%whence the consistent $\ell_p$ perturbation set reads
Consequently, we can write the adversarially robust risk with respect to $\ell_p$
perturbations as
% \begin{align}
%   \label{eq:AR}
%   \AR(\thetahat) &\define \EE_{X\sim\prob} \max_{\delta \in \pertset{p}(\epsilon)
%   }\losstest(\langle \thetahat, X + \delta\rangle, \langle \thetastar, X\rangle) \: \text{ with}\\
% %% \end{equation}
% %% \begin{equation}
% %%   \label{eq:consistent}
% \pertset{p}(\epsilon) &\define \{\delta \in \R^d: \|\delta\|_p \leq \epsilon~\textrm{and} ~\langle \thetatrue,\delta\rangle = 0\}. \nonumber
% \end{align}
\begin{align}
  \label{eq:AR}
  \AR(\thetahat) \define \EE_{X\sim\prob} \max_{\delta \in \pertset{p}(\epsilon)
  }\losstest(\langle \thetahat, X + \delta\rangle, \langle \thetastar, X\rangle) \:,
%% \end{equation}
%% \begin{equation}
%%   \label{eq:consistent}
\end{align}
%% \fy{might want to also do subscript $p$ for $\pertset$} For both the
%% 0-1 and the square loss, the adversarially robust risk upper bounds
%% the distributionally robust risk for $p\geq 1$ (see
%% Lemma~\ref{lem:dro}).
%% In applications where linear models
%% \fy{(eg bio etc.)}, it might be hard to argue the relevance of
%% robustness against $\ell_p$ attacks.
with $\pertset{p}(\epsilon) \define \{\delta \in \R^d: \|\delta\|_p \leq \epsilon~\textrm{and} ~\langle \thetatrue,\delta\rangle = 0\}. $
In many application scenarios, robustness against adversarial $\ell_p$-perturbations is not a main
security concern. Instead, the estimator should be robust against small distribution
shifts of the training and test data.
%% \emph{Distribution shift
%%   robustness} and distributionally robust optimization captures
%% robustness against worst-case shifts in a neighborhood of the original
%% risk.
As earlier work \cite{sinha18} pointed out, distribution shift
robustness and adversarial robustness are equivalent for losses
that are convex in the parameter $\theta$.
%and the corresponding choices of neighborhoods and perturbation set.
In particular, for consistent $\ell_p$ perturbations, the
adversarially robust risk upper bounds the distributionally robust
risk in a neighborhood of mean-shifted distributions (see
\suppmat{}~\ref{sec:dro}). Hence, a small adversarially robust risk
implies a small distributionally robust risk.

%% where $\probneighbor(\probx;\epsilon)$ most generally denotes an
%% (loosely defined) $\epsilon-$neighborhood of $\probx$ in the space of
%% probability distributions. \fy{trying to avoid metrics, }
%% %is some metric on the space of distributions.


%neighborhood of distributions $\probneighbor(\probx)$ \fy{metric/neighborhood}.
%We refer to Sections \fy{bla} for a detailed discussion.

% The distinction between consistent and inconsistent perturbations is necessary
% in order to avoid an ill-posed problem. Concretely, the ground truth
% $\thetanull$ is not the optimum of the population adversarial risk defined
% using inconsistent perturbations. In contrast, $\thetanull$ is the unique
% optimum of the consistent adversarial risk, which means that the problem of
% finding an estimator with both good prediction performance and robustness, has
% a unique solution.

%% \paragraph{Adversarial perturbations} In this paper, we focus on $\ell_2$ and
%% $\ell_{\infty}$ attacks.  Adversarial attacks with respect to $\ell_2$
%% perturbations result in a robust risk equal to the risk of the worst case causal
%% invariant distributed shift.  That is, assuming isotropic Gaussian features, the
%% adversarial robust risk is equivalent to the standard population risk when
%% drawing the test samples from the shifted distribution $X \sim \mathcal{N}(\mu,
%% \idmat_d)$ where the shift $\mu$ is orthogonal to the ground truth $\thetanull$.
%% Hence $\ell_2$ attacks connect advesrarial robustness and distribution shifts.

%% On the other hand, $\ell_{\infty}$ attacks are commonly studied in practice,
%% since they have the particular property that they allow an attacker to
%% concentrate the attack budget only on a few input dimensions, which makes the
%% attacks more effective and, in the case of image data, more imperceivable.

\subsection{Interpolation and regularization}

In order to find an estimator $\thetahat$ with small population risk,
we minimize an average training loss $\losstrain(\langle \theta, x\rangle, y)$. Even
though our results include the general setting for noisy observations,
the fact that regularization helps generalization is much more
surprising in the noiseless setting. Furthermore, the effect of noise is
diminishing in the overparameterized regime.
Hence, throughout this paper, we focus on the setting where all labels $y$ in the loss
follow the ground truth function and the signal is noiseless.

This also includes the adversarially robust loss \eqref{eq:AR} where
the average is taken over worst-case bounded $\ell_p$ perturbations around the training points.
We choose consistent perturbations orthogonal to the ground truth $\thetatrue$
for the same reason that we focus on the noiseless setting.
Even though the orthogonal subspace constraint
is not standard, inconsistent perturbations add noisy signal to the
training loss --- which is what we want to disentangle from finite-sample effects.
Yet, our results are not limited to consistent attacks;
we empirically show in \suppmat{}~\ref{sec:inconsistent} that they also
hold when training with inconsistent attacks.
% \fy{sth about disentangle
%   also in intro?}
% As motivated in the introduction, we choose to study $\epstrain$ so
% that GD has imperfect structural bias soh that the final
% training loss does not lead to a consistent estimator.

In the noiseless overparameterized setting where $d > n$,
many \emph{interpolating estimators} $\thetaeps$ with
vanishing average loss $ \frac{1}{n} \sum_{i=1}^n \max_{\delta \in
  \pertset{p}(\epstrain)} \losstrain(\langle \thetaeps, x\rangle, y)$
may exist.
In order to resolve ambiguity, we choose the solution of gradient
descent on the average loss as our implicit bias.
For the logistic and square loss
$\losstrain$ the resulting estimator is equivalent to the minimizer of
\emph{ridge-regularized} objective
\begin{align}
  \label{eq:ridgeloss}
  \empriskrob(\theta) &:= \frac{1}{n} \sum_{i=1}^n \max_{\delta \in
    \pertset{p}(\epstrain)} \losstrain(\langle\theta,\x_i +
  \delta\rangle, \y_i) + \lambda \|\theta\|_2^2
\end{align}
as $\lambda \to 0$ \cite{Rosset04}.
Our goal is to compare the interpolating estimators with
\emph{regularized} estimators that minimize $\empriskrob$ with
$\lambda>0$ and do not achieve vanishing training loss.
%% We study the
%% arguably most popular regularization technique---adding an $\ell_2$
%% penalty to the loss.  An alternative regularization technique is to
%% stop an iterative training process before convergence.
Finally, we remark that for linear regression on isotropic Gaussian features,
it is well known that ridge regularization corresponds to early stopping
\cite{Ali19,Ali20,Suggala18}.
% \fy{early stopping interesting cause
%   1. computational efficient for model choice 2. where robust
%   overfitting was observed}.

%% we consider are motivated by
%% \fy{we look at losses that give consistent signal with noiseless data. Because its easy to argue the noisy case, i.e. if it hurts noiseless it also hurts noisy. Such risks can be square or logistic loss. But also includes robust losses wrt consistent perturbations. Definition blabla We want to stress that the consistent perturbations are chosen for the biggest surprise. In practice when we use inconsistent perturbations, we expect any RO effect only to amplify.}
%% \fy{We consider interpolators that are a result of  GD on such a noiseless loss. Can often be written as minimizer of $L+\lambda \| \|_2$ with $\lambda \to 0$. The regularized estimator is then $\lambda > 0$}

%% A standard procedure for learning an estimator with small population risk is to minimize the average of a loss function $\losstrain$ on the training set $\{(x_i,y_i)\}$, and a standard procedure for learning an adversarially robust estimator is to minimizing the maximum loss over an $\ell_p$ ball around the original covariates.
%% Our definition of (unregularized) training loss encompasses both notation:
%% %% \begin{align}
%% %%   \label{eq:emprisks}
%% %%   \emprisk(\theta) &:= \frac{1}{n} \sum_{i=1}^n  \lossf(\langle\theta,\x_i + \delta\rangle, \y_i) ,
%% %%   \end{align}
%% %% and/or small robust empirical risk
%% \begin{align*}
%%   \empriskrob(\theta) &:= \frac{1}{n} \sum_{i=1}^n \max_{\delta \in \pertset{p}(\epstrain)} \losstrain(\langle\theta,\x_i + \delta\rangle, \y_i).
%% \end{align*}
%We consider the cases where $\epstrain$ matches the perturbation size in the risk (as in adversarial training) and when $\epstrain=0$ in the train loss (as in standard training).
%% In particular, $\epstrain = 0$ corresponds to
%% standard training while choosing $\epstrain=\epstest$ corresponds to consistent
%% adversarial training.
%\footnote{The attentive reader might note that the set of consistent perturbations for linear models is not available during training unless one
%% %knows the direction of the ground truth $\thetatrue$.  \fy{rephrase} We study
%% consistent training since it falls into the category of ``ground
%% truth''/noiseless signals - hence if overfitting occurs for consistent, then it
%% can only be at least as worse for inconsistent. We show that in the respective
%% settings}

%% We say an estimator $\thetahat$ is \emph{interpolating} if
%% $\empriskrob(\thetahat)$ is near zero.
%% %\fy{and $\sim 0$ for classification or is this ok?}.
%% In this paper we study the overparameterized setting $d>n$ where interpolation is feasible. Since in the overparameterized regime, the minimizer of the training loss is not unique, the particular
%% choice of the interpolator plays an important role in the analysis. We study
%% standard interpolators in the literature that are the final iterates/solutions
%% \fy{imprecise} of gradient descent on the unregularized loss: the minimum norm
%% solution~\eqref{eq:minnorm} for regression and $\epstrain$-max-margin solution~\eqref{eq:maxmarginAE} for the logistic loss.
%% \fy{something with well-defined re Hastie?}




%% \rh{I removed the def. of ridge regularization here, because its defined for linear and logistic regression below. Let's keep it notation wise as simple as possible.}
%Our goal is to compare the  interpolating estimators with \emph{regularized}
%estimators that do not achieve vanishing training loss.  Without prior knowledge
%on the structure of the ground truth, a common regularization
%technique that prevent interpolation is to add an $\ell_2$-penalty to the
%loss or to stop an iterative training process before convergence.
%For linear regression, it is well known for standard normal inputs
%that early stopping corresponds to ridge regularization \cite{Suggala18,Ali19,Ali20}. \fy{early stopping interesting cause 1. computational efficient for model choice 2. where robust overfitting was observed}.
%Hence, for the ease of presentation our theoretical analysis focuses on the
%ridge regression estimate
%minimizing a penalized training loss
%\begin{equation}
%\label{eq:ridge}
%  \thetalambda = \arg\min_{\theta} \empriskrob(\theta) + \lambda \|\theta\|_2^2,
%\end{equation}
%where $\lambda \geq 0$ is the regularization parameter.
%% and $\lossf(u,v)$ a
%%convex training loss that is minimized by an interpolating estimator.
%\fy{When structure is known can also use other norms Lasso aeh}
%% Our theoretical results focus on ridge regression estimate as it
%% for ease of presentation.
%% However, for linear regression there are well known results that show the
%% correspondence between early stopping and ridge regularization
%% \cite{Suggala18,Ali19,Ali20} for homogeneous features \fy{some qualifying
%%   statement for Reinhard ;)}.


%% \rh{The above is not necessary and potentially misleading, since ridge regularization and early stoping can behave quite differently. Better to leave it out, or just something general as of `we focus on $\ell_2$-regularization as it is one of the most popular techniques, but there are other interesting regularization techniques such as early stopping which many or may not have a similar effect, depending on the setup.'}


%that is convex in $\theta$.
%% Here, $\lossf(u,v)$ a convex
%% training loss.
%% \rh{Do we have to be so general here? Better to be concrete; if we need to be general we have to be specific and say in which the loss needs to be convex, or say convex in both .. .}

%% We exploit this
%% correspondence and primarily study ridge-regularized estimators in this paper.
%% However, as shown in ~\suppmat~1, we arrive at the same conclusions when
%% regularizing with early stopping.

%% A common regularization technique used in conjunction with gradient
%% descent on the loss $\Lossfemp_{\epstrain}(\theta)$ respective
%% $\Lossfemp(\theta)$ is early stoppping, where optimization is halted before the
%% solution convergences. This prevents the estimator form overfitting on the train
%% data and hence results in the well known bias variance tradeoff \kd{cite?}.  A
%% related regularization techniques is ridge regularization where the $\ell_2$
%% norm of a solution $\theta$ is penalized by adding it to the empirical risk a



% For general loss functions, including the logistic loss, no closed-form
% solutions of neither the standard nor the adversarial estimator exist.  The
% max margin solutions from Equation \eqref{eq:maxmargin},\eqref{eq:maxmarginAE}
% and min norm solution form Equation \eqref{eq:minnorm} A typical alternative
% is to iteratively minimize the empirical risk $\Lossfemp_{\epstrain}(\theta)$
% using gradient descent.  For convex losses, using a sufficiently small
% learning rate, gradient descent converges to a global solution of the
% optimization problems defined in Equation~\eqref{eq:SE} and
% Equation~\eqref{eq:AE} respectively.  Whenever interpolation of the respective
% loss is possible, gradient descent recovers the min norm interpolator
% \eqref{eq:minnorm} for the squared loss~\cite{Hastie19}, the max margin
% interpolator \eqref{eq:maxmargin} for the logistic loss under standard
% training~\cite{Ji19}, and the modified max margin interpolator
% \eqref{eq:maxmarginAE} for the logistic loss under adversarial
% training~\cite{Javanmard20}.


==> intro.tex <==
\section{Introduction}

Classical machine learning theory and practice suggest caution when fitting a
model to data: exactly fitting the training data, without regularization, can
result in high variance, and thus, sub-optimal prediction performance. This rule
of thumb seemingly does not apply to large, overparameterized models: Large
neural networks, for example, have excellent generalization performance on
\iid{} sales despite their ability to interpolate the training
set~\cite{Zhang16}. 

Empirical evidence suggests that interpolating the training data can even help
neural networks to generalize better as the model size grows~\cite{Nakkiran20},
and theoretical work for linear models \cite{Dobriban15, Mei19, Bartlett20,
Muthukumar20, Muthukumar20a} and kernel methods \cite{Liang20a, Ghorbani19} has
shown that increasing the dimensionality of the data decreases the variance. 


These findings promote the perspective that there is no need for regularization
for modern, high-dimensional models. However, these prior works focus
exclusively on the impact of interpolation on the \emph{standard} test risk that
assumes \iid{} training and test data.

This measure of performance, however, may not reflect the accuracy of model
deployed in the real world, where robustness to distribution shifts, adversarial
attacks, or fairness metrics such as the worst-group risk play an increasingly
important role.
 %to distribution shifts and other notions of robustness.  In order to evaluate
%and enhance reliability, alternative performance metrics have recently gained
%popularity, such as distributionally and adversarially robust risks, or
%fairness metrics including the worst-group risk. 

%The robust notions of risk are governed by two terms that feature prominently in the statistical literature: the first is due to noise in the data (\emph{variance}), and the second persists even in the noiseless case (\emph{bias}).


%Classical wisdom \cite{Hastie01} suggests to use regularization in order to reduce variance, at the cost of an increased bias that prevents models from achieving vanishing training loss (which we refer to as \emph{interpolating}).
% to prevent an estimator to achieve vanishing training loss (we say it
% \emph{interpolates}) and hence fit noise. % RH: rewritten because potentially
% misleading, because not clear whether the estimator literally fits noise when
% it is regularized

% With the emergence of heavily overparameterized models that generalize well
% despite interpolating the data (i.e.\ achieving vanishing training loss),
% significant attention has been directed to understanding interpolation in the
% overparameterized regime. In particular, increasing width in neural networks
% also seems to remove the need to avoid interpolation.\fy{cite DDD} \rh{I don't
% get the last sentence-increasing width makes the network more linear; how does
% that remove the need for interpolation?}. The theory community has since
% presented multiple results to explain this phenomenon for linear, kernel and
% RF regression models: in particular they find that increasing dimensionality
% \rh{do you mean model size? If yes, let's better use model size.} decreases
% variance \fy{cite everybody} \fy{also kernels doesn't quite fit here}.
% Therefore, the dominant narrative/conclusion in the current literature on
% overparameterized models is that there is no need for regularization in high
% dimensions.

% However, those findings presume that the data is noisy; for example, DDD shows
% the double descent phenomenon only after adding artificial label \rh{We have
% to be careful here; Mei and Montanari establish double descent ``The
% generalization error of random features regression'' for the noise-less case.
% Here, the missfit of the models (data geneated linearly, estimator is random
% feature model) ``noise'' has an effect just like noise. Can we say ``those
% findings presume that the data is noisy or that there is a model missfit'', or
% is this not accurate any more?} %However there are a few shortcomings that
% this conclusion does not explain: For one, is the data really noisy? .
% CIFAR10 can achieve 99.7\% on the latest models .  

In fact, mounting empirical evidence challenges the narrative that there is no
need for regularization for modern, high-dimensional models, and suggests that
regularization actually improves \emph{robust test risks}, for instance in the
context of adversarial perturbations \cite{Rice20} or for worst-group
generalization \cite{Sagawa20a, Sagawa20b}, even in the highly overparameterized
regime! This phenomenon persists even after we perform data sanitization
procedures to drastically reduce the noise in the training data, as illustrated
by our experiments in Figure~\ref{fig:teaser_plot_nn} (we provide details on the
experimental setup in Section~\ref{sec:appendix_experiments} of the Appendix).

% These experimental findings suggest that robust notions of performance still
% require regularization even for overparameterized models. The goal of this
% paper is to understand the causes of this phenomenon and investigate the
% following question theoretically: 
% 
% \begin{center} 
% 
% %   \emph{If the data is noiseless/In the highly overparameterized regime where
%   %   variance is low, when is it still beneficial to avoid perfectly fitting
%   %   the training data/minimizing the training loss?}
%   \emph{In the highly overparameterized regime in which variance is low, why is
%   it still beneficial to avoid perfectly fitting the training data?}
% 
% \end{center}
% 
% \rh{This formulation of a question is too vague, can we formulated it
% differently? Also, the question should contain some reference to robustness,
% because that is central. Perhaps this question: ``Is there a provable robustness
% benefit of regularizing interpolating models in the noiseless regime?''. If we
% can't find a good formulation here, we can also work without posing a concrete
% question.}
%``....'' Here we need a more concrete question that we actually answer, than
%the one emphasized below.  }

%These experimental findings indicate that the current perspective on
%the benefits of interpolation in high dimensions may be incomplete,
%and that one may arrive at a different conclusion if robustness is
%considered for evaluation \fy{imprecise sentence in part due to
%  passive voice. which different conclusion?}. In this paper we aim to
%fill this gap and study the following question:
%


\fy{not sure I'd use ``interpolate'' here}
% Further, it seems that when measuring the adversarially robust risk or
% worst-group generalization, early stopping before the training loss vanishes in
% fact improves generalization (\emph{robust overfitting}), even for very wide
% overparameterized models! \fy{cite rice, pangwei} Also, even after proposed
% noise sanitization procedures on very simple images,~\ref{fig:teaser}, we still
% observe robust overfitting.

%% Generalization performance measure using risk / test metric.
%% Risks that
%%  we care about: natural/standard + robust 
%% distributional robustness
%% adversarial robustness (related)
%% Image experiments also find robust overfitting but only give explanation for noisy and argue noiseless 
%% Generalization / excess risk depends on a term that is nonzero only when there’s noise (we say variance…?) and another term that is driven by optimization procedure, averaged over training data (we call bias)

These experimental findings suggest that robust notions of performance still
require regularization even for overparameterized models. When the training data
does not contradict the ground truth, for example for noiseless observations or
for adversarial training with consistent perturbations \cite{Raghunathan20},
then a natural intuition is that leveraging all signals perfectly should help to
achieve best generalization.
% contains samples of the ground truth  \fy{I want to include consistent
% adversarial perturbations here} without noise, a natural intuition is that
% leveraging all signals perfectly should help to achieve best generalization.
%% Even though when working with noiseless data a natural reflex is to
%% use all the signal in the training set and interpolate to achieve the
%% best generalization, there exist examples \fy{of what?} that indicate
%% otherwise.
For instance, it is well-known that when the ground truth has a low-dimensional
structure matched by the implicit bias of the estimator, we can hope to achieve
good generalization even with relatively little data, as is the case for the
lasso estimator \cite{Tibshirani96}. However, in the case of a structural
mismatch, interpolation may not suffice to find a satisfactory overparameterized
estimator.

In particular, our main contribution is that we show theoretically that
achieving zero training loss does not lead to an optimal adversarially robust
risk for linear regression and classification, even in noiseless settings.
Moreover, we prove that $\ell_2$ regularization or early stopping can
significantly improve performance even for robust estimators trained with
adversarial training, a phenomenon previously observed empirically for neural
networks and referred to as robust overfitting \cite{Rice20}.

The next section introduces notation used throughout the paper and makes a
connection between adversarial and distributional robustness for linear models.
In Section~\ref{sec:linreg} we give precise asymptotics for the robust risk of
the ridge estimator and the minimum norm interpolator in the context of linear
regression. Then, in Section~\ref{sec:logreg} we show that adversarial training
for logistic regression can benefit from ridge regularization and provide
insights explaining this phenomenon.

% When the amount of noise in the data is insignificant, a natural reflex is to
% use all the signal in the training set and interpolate to achieve the best
% generalization. 

% A natural reflex is to say that even though in the overparameterized regime we
% are given little information about the function, we should use as much true data
% as possible, and deliberately avoiding interpolation would not help
% generalization. It is well known that in the case when the implicit bias of the
% interpolator matches a ground truth that has low-dimensional structure, we can
% hope to achieve good generalization even with relatively little data \fy{lasso
% etc.} However in the case of a structural mismatch, this might not be the case.
% For example, a recent paper shows for linear regression, how adding a new
% noiseless data point data can decrease prediction accuracy when the test
% distribution favors certain directions.  \fy{could cite our tradeoff paper - it
% is the only work in this direction that I know but its very ehm toy ...  don't
% have to cite, also makes the sentence harder}
% 
% In this work, we prove for linear regression and classification, that perfectly
% fitting all available noiseless samples is often undesirable in many scenarios,
% in particular for the robust risk. In Section bla we do bla.




%% Motivated by the observation that large deep neural networks \fy{cite
%%   Chiyuan,openai} \rh{perhaps zhang UnderstandingDeepLearning 2016} perform well, in recent years increasing attention has been
%% devoted in the field of learning theory to study when
%% estimators that achieve perfect train accuracy still generalize well.
%% %% interpolation \fy{maybe zero empirical risk sth...? unclear for classification}
%% %% with overparameterized models
%% %% still yields estimators with good
%% %% generalization properties \fy{a bit long}.
%% These papers show that overparameterization acts as implicit regularization as it reduces the variance in the high-dimensional regime when
%% $d,n\to\infty$ \fy{not sure if good to bring up here}. For certain distributions, it is even possible to
%% reach consistency \fy{cite benign, vidya, ghorbani etc.}. This
%% phenomenon is often manifested in a double descent shaped risk curve, where the risk as a function of the amount of overparameterization first decreases, then increases, and finally decreases again.
%% This is observed for a variety of machine learning models, including linear and logistic regression, random features and kernel
%% regression. \fy{citestuff}
%% %\rh{Perhaps better to not mention double descent so prominently here, because this is not central to the storyline (unless I'm missing something)}


%% %A common story and conclusion of these papers is to just interpolate without the need to regularize as the overparameterization ratio increases.  
%% This development suggests that training to interpolation without regularization is sufficient to obtain a well-performing model. 
%% However these conclusions were based on studying the
%% standard population risk only. Modern machine learning practice
%% often requires models to also exhibit certain degrees of reliability
%% and fairness such as robust against distribution shifts,
%% adversarial perturbations, and the ability to achieve good worst-group performances
%% \fy{citestuff}. Lately, there has been rising empirical evidence that
%% common methods to tackle these \emph{robust risks} in fact
%% \emph{benefit from regularization that prevent interpolation} even in
%% the overparameterized regime. This phenomenon, referred to as
%% \emph{robust overfitting} in some contexts, has been observed for
%% $\ell_\infty$ robustness and worst-group generalization for images.
%% \fy{cite pangwei and rice}. This raises the question:

%% \begin{center}

%% When does regularization regain its merits when measuring robust generalization?

%% \end{center}

%% Some works following the observations of \rh{cite pangwei and rice again} conjectured explanations based on experimental
%% evidence.  In particular they argue that robust overfitting is caused
%% by noisy or ambiguous samples in the training data
%% \cite{Amartya20,Dong21} and suggest filtering methods that can eradicate/mitigate
%% the phenomenon.
%% %That is, the robust risk and adversarial
%% %training amplify the variance due to noise and hence benefit more from
%% %regularization.
%% %reminiscent of similar geometric arguments  made in
%% %earlier work \fy{Gilmerblowup, goldstein stuff?}.
%% \fy{is it that we contradict the tautology paper with mnist 1,3
%%   or is it just that we show for pruned and unpruned, gap doesn't change?}
%% %% However recent results suggest that CIFAR-10 \fy{is not really that noisy},
%% %% and furthermore
%% However, as shown in Figure~\ref{fig:teaser}, simple experiments using the proposed variance
%% reduction methods \fy{is that true} suggest that robust overfitting persists even on MNIST
%% with a simple RELU MLP when the bootstrap estimated variance is below \fy{bla}.
%% \fy{explain gap in one sentence}

%% It is hard to rigorously verify or falsify that datasets such as CIFAR-10 are indeed noisy,
%% even though small bootstrap estimated variances \fy{steinhardt} and $99.7\%$
%% test performance with the latest architecture \fy{cite} suggest that label noise is indeed neglible.
%% To challenge this hypothesis, Figure~\ref{fig:teaser} shows that even after
%% noise reduction with a final variance of ..., robust accuracy persists
%% the overfitting gap of a
%% neural network trained on a pruned binary classification task where only classes
%% 1 and 3 from the MNIST data set were considered. We can still observe robust
%% overfitting in this sanitized setting, where the noise has been reduced
%% significantly. Perhaps surprisingly, even overparameterized models with
%% remarkably low variance still exhibit robust overfitting and benefit from
%% early-stopping regularization. This observation raises the following question:

%% \begin{center}

%%   \emph{Are there situations when preventing interpolation can actually be
%%   beneficial for overparameterized models?}

%% \end{center}


\begin{figure*}
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_nn.pdf}
    \caption{Neural network}
    \label{fig:teaser_plot_nn}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_linreg.pdf}
    \caption{Linear regression}
    \label{fig:teaser_plot_linreg}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_logreg.pdf}
    \caption{Linear classification}
    \label{fig:teaser_plot_logreg}
  \end{subfigure}

  \caption{ In this plot we show the gap between the standard and
    distributionally robust risk of the best regularized and final estimator for
    a (a) two-layer neural network with varying width, trained on (binary
    $1$-$3$) MNIST after using suggested variance reduction methods (see
    Appendix~\ref{sec:appendix_experiments}, regularized using early stopping .
    (b) linear regression on noiseless observations (c) distributionally robust
    training on logistic regression. The robust risk benefits significantly from
    regularization. For logistic regression, the standard risk also overfits
    however to a lesser extent than the robust risk.
    %% Performance gap between unregularized and optimally regularized estimators
    %% in simple noiseless interpolating settings.
    %% Subfigure \ref{fig:teaser_plot_nn} shows the performance of a two-layer neural networks with varying width, trained on (binary $1$-$3$) MNIST and evaluated with respect to $\ell_{\infty}$-perturbations.
    %% To reduce variance, we discard all training samples which a separately trained estimator cannot easily fit. We refer to
    %% \suppmat~\ref{sec:appendix_experiments} for the details.
    %% \ref{fig:teaser_plot_linreg} is linear regression standard training on noiseless synthetic data
    %% evaluated wrt $\ell_2$ perturbations.
    %% \ref{fig:teaser_plot_logreg} is logistic regression adversarial training on noiseless synthetic data
    %% trained and evaluated wrt $\ell_\infty$ perturbations. 
    %% The experiments shows that--even with the suggested variance reduction technique--the robust risk overfits (i.e., there is a non-zero gap between optimally regularized and the non-regularized estimate). 
%    \rh{Can we have a sentence summarizing the main conclusion from the
    %    experiment here, like: ``Even with the suggested variance reduction
    %    method, the robust overfitting phenomena persists.} a) The gap between
    %    optimal early stopped and final standard and robust risk with respect
    %    to $\ell_{\infty}$ perturbations for a single
%     hidden layer neural network with varying width on the binary $1$-$3$
    %     MNIST.  To reduce the variance, we additionally prune the samples
    %     which are not fitted by a separately trained estimator after early
    %     stopping.\ b) The estimated variance of the original and pruned data
    %     set. We refer to \suppmat~\ref{sec:appendix_experiments} for the
    %     details.
%   To reduce potential noise in the training set and fitting procedure, we
    %   discard all training samples which are not correctly classified within
    %   the first 100 epochs of training Nevertheless, we still observe
    %   significant robust overfitting in \ref{fig:teaser_overfitting}.  In
    %   order to quantify the amount of noise at hand,
%   we estimate model variances on the test set for each number of hidden units.
    %   \ref{fig:teaser_variances} shows the estimated variance averaged all
    %   test samples with bars indicating one empirical standard deviation.
    %   While the estimated variance for the full training set is already low,
    %   our pruning procedure further reduces it.
%   Artificial low-noise setting which exhibits significant robust overfitting.
    %   We fit a single hidden layer neural network with varying width on two
    %   MNIST classes.  To reduce potential noise in the training set and
    %   fitting procedure, we discard all training samples which are not
    %   correctly classified within the first 100 epochs of training
%   Nevertheless, we still observe significant robust overfitting in
    %   \ref{fig:teaser_overfitting}.  In order to quantify the amount of noise
    %   at hand, we estimate model variances on the test set for each number of
    %   hidden units.  \ref{fig:teaser_variances} shows the estimated variance
    %   averaged all test samples with bars indicating one empirical standard
    %   deviation.  While the estimated variance for the full training set is
    %   already low, our pruning procedure further reduces it.
  }

  \label{fig:teaser}
\end{figure*}
% 

%% Indeed, in this paper we show that robust overfitting occurs for
%% linear models \emph{even in the noiseless setting} in the heavily
%% overparameterized regime, illustrated in Figure~\ref{fig:teaser}.  We
%% prove robust overfitting of interpolating estimators for linear and
%% logistic regression in the high-dimensional regime.  In particular, we
%% show that in the overparameterized regime, i.e., for large overparameterization ratios $d/n \to \gamma$ and $d,n\to\infty$ regularization significantly improves generalization on the robust risk even though it does not benefit standard generalization. 
%% With this
%% work we'd like to provide a clear \fy{other word} counterpoint to an
%% increasing line of work that focuses on the diminished relevance of
%% regularization in the overparameterized regime.

%% %studies benefitsof overparameterization.

%% In section we do bla.

%% In this paper we answer this question in the positive and show that evaluating
%% adversarial robustness is one such setting where regularization does more than
%% only reduce variance.  Our main \textbf{contribution} is that we show that, for
%% both linear regression and logistic regression, the consistent robust risk
%% benefits from ridge regularization or early stopping even on noiseless
%% observations. Furthermore, this form of overfitting occurs only in the
%% overparameterized regime where the standard error benefits from the implicit
%% regularization that is characteristic for interpolating models. However, our
%% results demonstrate that interpolation can be harmful even when the standard
%% error does not suffer from overfitting.  Thus, we argue that regularization
%% plays a fundamentally different role for the consistent robust risk and acts not
%% just on the variance, but also as a form of bias reduction. To the best of our
%% knowledge, we are the first to study theoretically the impact of early stopping
%% and ridge regularization on the consistent robust risk for overparameterized
%% models. 

%% The double descent phenomenon, which has recently gained popularity in the
%% machine learning community, points to the beneficial effects of
%% overparameterization.  The effect of implicit regularization due to
%% overparameterizating has been first explicitly pointed out by \citet{Zhang17}
%% for deep neural networks where it is shown that these models achieve good
%% generalization performance although interpolating the train data. Surprisingly,
%% these observations put into perspective the classical wisdom on the
%% bias-variance trade-off which tells us us that the bias decreases and variance
%% increases with model complexity [TODO cite textbook]. Since then, a modern line
%% of statistical and machine learning research has emerged studying this effect
%% more carefully. In particular, the paper \cite{Nakkiran20,Yang20} observe that
%% the variance of deep neural networks decreases again after the interpolation
%% threshold when further increasing the model complexity, and hence achieve a
%% similar effect to regularization. 

%% Multiple papers from the statistical side underline this observation by proving
%% that such a behavior also occurs for classical regression and classification
%% algorithms including linear, logistic and random feature regression
%% \cite{Belkin19,Nakkiran20,Hastie19,Mei19,Deng20,Chinot21}. In fact, it has even
%% been shown that for certain spiked covariance data models both logistic and
%% linear regression can be asymptotically consistent in high dimensional regimes
%% albeit interpolating noisy train data \cite{Bartlett20,Muthukumar20}. In
%% summary, these papers suggest that the effect of implicit regularization in
%% overparameterized regimes makes explicit variance reduction techniques like
%% early stopping or ridge regularization redundant. 

%% All of these works have focused on the effect of overparameterization on the
%% prediction error of estimators. However, in many practical applications we are
%% interested in other criteria for evaluation as well, such as ensuring fair
%% predictors [TODO cite], or models that generalize well under covariate shift
%% [TODO cite]. Another example of a desirable property of prediction models, known
%% as \emph{adversarial robustness}, is that they are invariant to small (in
%% $\ell_p$ norm) additive perturbations of the input data \cite{Szegedy14}.
%% % For instance, in the case of image data sets these perturbations are often
%% % imperceptible to a human and, thus, do not change the semantics or the label
%% % of the inputs.
%% In order to avoid an ill-defined problem, it is crucial that the notion of
%% robustness that we use is not at odds with the other goal, which is to recover
%% the ground truth function and to achieve a low prediction error. To ensure that
%% we do not have interfering objectives, we only consider consistent perturbations
%% for evaluating the models, namely perturbations that do not change the value of
%% the ground truth function [TODO cite]. For linear models, consistent adversarial
%% robustness has even more profound consequences: perfect $\ell_p$ robustness
%% against consistent perturbations implies automatically robustness to
%% distribution shifts along any direction perpendicular to the linear ground
%% truth. This invariance to changes along directions that are independent of the
%% ground truth is of great importance in practice, in particular in situations
%% where fairness is important or when we do not wish to make predictions that rely
%% on spurious features.

% On top of achieving a low prediction accuracy on unseen test samples, in
% practical applications we often require the models to be robustness against
% perturbations in the input data.  \textit{say somehting here, but i really
% dont know the literature. This must be good, for instance we could mention
% fairness or distribution shifts? But motivate well why we do want a low robust
% risk BEYOND image data sets! Also motivate consistent perturbations}

% Modern machine learning models have to be vulnerable to imperceptible
% perturbations of the inputs \cite{Szegedy14}. This worrisome behavior has
% garnered a lot of attention in recent years and it spurred several lines of
% work that try to propose ways to defend against such adversarial attacks. Even
% though many of the suggested defences have been breached by carefully designed
% attacks \cite{Tramer20}, there are two approaches that stand out. Firstly,
% adversarial training \cite{Goodfellow15} has consistently been reliable even
% in the face of these newly discovered attacks. Secondly, a number of works
% have proposed certified defences \cite{Salman19, Balunovic19} which come with
% appealing robustness guarantees.

%% One popular approach to improve the robustness of a model to adversarial
%% $\ell_p$-perturbations is to use adversarial training (AT) where we minimize the
%% empirical risk with perturbed input train samples. This method has successfully
%% been applied to various models including deep neural networks
%% \cite{Goodfellow15} but also linear and logistic regression
%% \cite{Javanmard20a,Javanmard20b}. In a recent paper \cite{Rice20} the authors
%% uncover an interesting phenomenon: When minimizing the adversarial training loss
%% using an iterative algorithm (e.g.\ stochastic gradient descent), the
%% optimization path passes through a more robust solution first, before it
%% converges to a less robust one. Hence, an early-stopped model has better robust
%% accuracy, as measured on a hold out test set, than a model trained to
%% convergence. What makes this phenomenon surprising is that the authors observe
%% it for highly overparameterized deep neural networks where the natural test
%% error does not suffer from overfitting despite interpolating the train samples. 

%  A natural approach is to try and understand robust overfitting through the
%  lens of regular overfitting of the standard accuracy.  For a long time, the
%  classical statistics literature has pointed at noise as the major culprit for
%  overfitting.  More recently, a new story line has started to emerge:
%  overparameterization alone can mitigate overfitting by reducing the variance,
%  a phenomenon that is often referred to as `double descent`. One important
%  conclusion stressed by this line of work is that regularization is redundant
%  in the highly overparameterized regime.



% Our contributions are as follows:
% \begin{itemize}[leftmargin=*]
% 
%   \item for linear regression, we show that the consistent $\ell_2$ robust risk
%     benefits from ridge regularization or early stopping even on completely
%     noiseless observations. Furthermore, the described effect is only observed
%     in the overparameterized regime where the standard error benefits from the
%     implicit regularization described in \cite{Hastie19}.
% 
%   \item for classification, we study the consistent $\ell_{\infty}$ robust risk
%     for logistic regression and show that the adversarially trained estimator
%     suffers from overfitting of both the standard and robust risk, even in the
%     noiseless case. \at{TODO need to fit the next two sentences with the rest of
%     the story} Finally, we show that when adding label noise we need a higher
%     degree of overparameterization $d/n$ to interpolate the train data.
%     Surprisingly, this leads to the observation that the unregularized estimator
%     trained with noise achieves a lower final robust and standard risk compared
%     to the one trained without label noise.

%   \item for classification, we study the consistent $\ell_{\infty}$ robust
%     for logistic regression. Since standard training achieves only very poor robust risk, we focus on the adversarially trained estimator and show that this suffers from overfitting of both the standard and robust risk, even in the
%     noiseless case.
% \end{itemize}

% As a first contribution, we show that the consistent $\ell_2$-adversarial robust
% risk of linear regression benefits form ridge regularization or equivalently
% early stopping even on completely noiseless observations.  In this case, the
% variance of the standard risk is zero and hence suffers from explicit
% regularization. Our results demonstrate that interpolation can be harmful even
% when the standard error does not suffer from overfitting. Thus, we can conclude
% that regularization plays a fundamental different role for the consistent robust
% risk and Furthermore, the described effect is only observed in the
% overparameterized regime where the standard error benefits form the effect of
% implicit regularization as describe in the paper \cite{Hastie19}. 

% As a second contribution this paper studies the consistent
% $\ell_{\infty}$-adversarial robust risk for logistic regression on a
% discriminative sparse linear data model. While the standard trained estimator
% achieves very poor robust population accuracy close to $0$, the adversarially
% trained estimator trained with inconsistent adversarial $\ell_{\infty}$ attacks
% achieves a significantly better standard and robust test accuracy albeit still
% being able to interpolate the train samples. Surprisingly, however, we show that
% even in the noiseless case the estimator suffers from overfitting of both the
% standard and robust risk. While inconsistent attacks may induce some noise
% during training even for noiseless data, we also show that the we observe
% overfitting of the risks when training with consistent adversarial attacks
% assuming that we have full knowledge of the ground truth during training.
% Finally, we show that when adding label noise we need a higher degree of
% overparameterization $d/n$ to interpolate the train data. Surprisingly, this
% leads to the effect that the unregularized estimator trained with noise achieves
% a lower final robust and standard risk compared to the one trained without label
% noise. 

% Both examples demonstrate how interpolation suffers from overfitting in the
% overparameterized regime even for noiseless train data. As a result, this paper
% puts into perspective the modern story line on the implicit regularization due
% to overparameterization by highlighting that additional robustness constrains
% still require additional explicit regularization to prevent the model from
% interpolation. 





% This puts the modern story line on regularization into perspecti observes a
% vanishing In particular, we show that the robust risk suffers from overfitting
% even on noiseless which questions the 
% 
% 






% « In the paper \cite{Amatya20} the authors show that the robust accuracy is
% much more sensitive to noise in the train data than the standard accuracy.
% Although the experiments in the paper \cite{Rice20} are conducted on the
% original \textit{CIFAR-10} \cite{Krizhevsky09} dataset without any additional
% label noise, the authors from the paper \cite{Amatya20} highlight that these
% there are still misslabeled/wrong samples contained in the dataset. Therefore,
% the authors suggest that the overfitting of the robust risk may be explained
% due to a higher sensitivity to noise fitted by the estimator. A similar
% conclusion is suggested by the paper \cite{Dong21}, where the authors observe
% that the robust risk does not overfit when removing problematic samples which
% are not fit by a early stopped estimator form the data. 


% Yet this phenomenon not yet well understood and existing attempts to explain
% the phenomenon have predominantly linked it to noise respectively problematic
% samples in the train data. In the paper \cite{Amatya20} the authors show that
% the robust accuracy is much more sensitive to noise in the train data than the
% standard accuracy.  Although the experiments in the paper \cite{Rice20} are
% conducted on the original \textit{CIFAR-10} \cite{Krizhevsky09} dataset
% without any additional label noise, the authors from the paper \cite{Amatya20}
% highlight that these there are still misslabeled/wrong samples contained in
% the dataset. Therefore, the authors suggest that the overfitting of the robust
% risk may be explained due to a higher sensitivity to noise fitted by the
% estimator. A similar conclusion is suggested by the paper \cite{Dong21}, where
% the authors observe that the robust risk does not overfit when removing
% problematic samples which are not fit by a early stopped estimator form the
% data. 
% 
% While noisy/problematic samples in the train data certainly have an effect on
% the robust accuarcy, we observe in Figure~\ref{fig:teaser} that the robust
% accuracy overfits even on binary 1-3-MNIST with additional pruning of unfitted
% samples by a early stopped neural network. In this paper we aim to better
% understand 



% ttempt to explain the overfitting of the robust accuarcy due to an
% oversensitivity to noise in the train data.  samples. While noise in the train
% data clearly has an impact on robust overfitting (see Figure \ref{fig:asdf}),
% this paper shows that robust overfitting also occurs   noiseless settings
% where the natural accuracy does not benefit from regularization at all. Hence,
% this paper challenges the role of regularization: In the classical
% understanding we have that in the well specified setting, regularization leads
% to a bias-variance tradeoff, meaning that we increase bias but decrease
% variance. In particualr, this suggests that if you have no noise,
% regularization does not improve performance.  More specifically, this paper is
% the first one theoretically studying overfitting of the robust loss. Unlike
% existing literature we \kd{continue to write soon }


% 
% Mission of the paper: Hence we seek to complete the picture by proving the
% conjecture for lin reg The conjecture: in settings: ST, AT, noiseless … … when
% evaluating the robust error, early stopping is needed for a much wider range
% of d/n and p/n ratios, compared to testing using the std error Our
% contributions: We prove … … this conjecture is true in the settings above for
% linear models (lin reg).  in particular our claim is that …. causes it. (proof
% intuition) We also show experimentally that indeed RO happens in these
% settings and second the intuition carries through to images. 






% \kd{A bit a repetition from the intro}
% Robust overfitting is the intriguing phenomenon that has been observed by
% \cite{Rice20} on neural networks trained with adversarial training: early
% stopping regularization has a significant effect in reducing the robust test
% error, while, in contrast, the standard test error is always non-increasing as a
% function of time. \kd{Rice does this as well, need to write more here} In this
% section we provide empirical evidence that robust overfitting occurs even in a
% noiseless setting, raising questions about the nature of the phenomenon.

% \kd{this is already contained in the intro: A natural approach is to try and
% understand robust overfitting through the lens of regular overfitting of the
% standard accuracy. For a long time, the classical statistics literature has
% pointed at noise as the major culprit for overfitting.  More recently, a new
% story line has started to emerge: overparameterization alone can mitigate
% overfitting by reducing the variance, a phenomenon that is often referred to
% as `double descent`. One important conclusion stressed by this line of work is
% that regularization is redundant in the highly overparameterized regime.
% 
% Robust overfitting is indeed exacerbated by noise. Adding artificial label
% noise to the training data makes robust overfitting much more pronounced, as
% we show in Appendix TODO for overparameterized fully-connected neural
% networks. However, going in the opposite direction and \textit{reducing} the
% amount of noise of the prediction problem to a minimum reveals a surprising
% situation. In a noiseless setting where the variance vanishes, it seems like a
% sensible hypothesis is that regularization has no effect on the test robust
% error.  }

% \citet{Rice20} showed that the robust loss overfits when training
% overparameterized deep neural networks on CIFAR \cite{Krizhevsky09} without
% adding any additional label noise. However, as highlighted by \citet{Sanyal21}
% the original data set itself cointains noisy samples. Hence, we cannot
% conclude from the presented experiments that robust overfitting occurs even in
% the absence of noise. 

% , the following experiments indicate that, for overparameterized models, the
% role of regularization is not lpimited to just reducing the variance.




% The observation that regularization is beneficial even in a noiseless setting
% raises the following question:
% 
% \begin{center}
% 
%   \textit{Can regularization reduce the bias of overparameterized models \\
%   with respect to certain evaluation metrics?}
% 
% \end{center}
% 
% In particular, is it the case that certain traditional regularization
% techniques are better suited at priming estimators for robust evaluation? In
% the sequel we analyze lineapr and logistic regression in the context of
% adversarial robustness and prove that, in high dimensions, early stopping and
% ridge regularization lead to more robust predictors.


==> intro_old.tex <==
\section{Introduction}

Classical machine learning theory and practice suggest caution when fitting a
model to data: exactly fitting the training data, without regularization, can
result in high variance, and thus, sub-optimal prediction performance. This rule
of thumb seemingly does not apply to large, overparameterized models: Large
neural networks, for example, have excellent generalization performance on
\iid{} samples despite their ability to interpolate the training
set~\cite{Zhang16}. 
%Classical wisdom \cite{Hastie01} suggests to use regularization in order to
%reduce variance, at the cost of an increased bias that prevents models from
%achieving vanishing training loss (which we refer to as \emph{interpolating}).
Empirical evidence suggests that interpolating the training data can even help
neural networks to generalize better as the model size grows~\cite{Nakkiran20},
and theoretical work for linear models \cite{Dobriban15, Mei19, Bartlett20,
Muthukumar20, Muthukumar20a} and kernel methods \cite{Liang20a, Ghorbani19} has
shown that increasing the dimensionality of the data decreases the variance. 
% which in turn leads to a decreasing risk curve past the interpolation
% threshold and the double descent phenomenon \cite{Belkin19}.  
% This variance reducing phenomenon has also been shown for RKHS
% \cite{Liang20a}\fy{cite Ghorbani} in the high-dimensional regime. %,when kernels
% % converge to their polynomial approximation.
% \rh{last part is too much detail}

%Those findings pertain to the classical evaluation mode where prediction
%performance is evaluated on a test distribution that coincides with the
%training distribution. 
These findings promote the perspective that there is no need for regularization
for modern, high-dimensional models. However, these prior works focus
exclusively on the impact of interpolation on the \emph{standard} test risk that
assumes \iid{} training and test data.
%Machine learning-based prediction models are usually evaluated based on their
%performance on a test distribution that often coincides with the training
%distribution.  usually evaluated with respect to population risks, that are
%expectations over a pointwise loss with the same distribution as the training
%set. 
This measure of performance, however, may not reflect the accuracy of model
deployed in the real world, where robustness to distribution shifts, adversarial
attacks, or fairness metrics such as the worst-group risk play an increasingly
important role.
 %to distribution shifts and other notions of robustness.  In order to evaluate
%and enhance reliability, alternative performance metrics have recently gained
%popularity, such as distributionally and adversarially robust risks, or
%fairness metrics including the worst-group risk. 

%The robust notions of risk are governed by two terms that feature prominently in the statistical literature: the first is due to noise in the data (\emph{variance}), and the second persists even in the noiseless case (\emph{bias}).


%Classical wisdom \cite{Hastie01} suggests to use regularization in order to reduce variance, at the cost of an increased bias that prevents models from achieving vanishing training loss (which we refer to as \emph{interpolating}).
% to prevent an estimator to achieve vanishing training loss (we say it
% \emph{interpolates}) and hence fit noise. % RH: rewritten because potentially
% misleading, because not clear whether the estimator literally fits noise when
% it is regularized

% With the emergence of heavily overparameterized models that generalize well
% despite interpolating the data (i.e.\ achieving vanishing training loss),
% significant attention has been directed to understanding interpolation in the
% overparameterized regime. In particular, increasing width in neural networks
% also seems to remove the need to avoid interpolation.\fy{cite DDD} \rh{I don't
% get the last sentence-increasing width makes the network more linear; how does
% that remove the need for interpolation?}. The theory community has since
% presented multiple results to explain this phenomenon for linear, kernel and
% RF regression models: in particular they find that increasing dimensionality
% \rh{do you mean model size? If yes, let's better use model size.} decreases
% variance \fy{cite everybody} \fy{also kernels doesn't quite fit here}.
% Therefore, the dominant narrative/conclusion in the current literature on
% overparameterized models is that there is no need for regularization in high
% dimensions.

% However, those findings presume that the data is noisy; for example, DDD shows
% the double descent phenomenon only after adding artificial label \rh{We have
% to be careful here; Mei and Montanari establish double descent ``The
% generalization error of random features regression'' for the noise-less case.
% Here, the missfit of the models (data geneated linearly, estimator is random
% feature model) ``noise'' has an effect just like noise. Can we say ``those
% findings presume that the data is noisy or that there is a model missfit'', or
% is this not accurate any more?} %However there are a few shortcomings that
% this conclusion does not explain: For one, is the data really noisy? .
% CIFAR10 can achieve 99.7\% on the latest models .  

In fact, mounting empirical evidence challenges the narrative that there is no
need for regularization for modern, high-dimensional models, and suggests that
regularization actually improves \emph{robust test risks}, for instance in the
context of adversarial perturbations \cite{Rice20} or for worst-group
generalization \cite{Sagawa20a, Sagawa20b}, even in the highly overparameterized
regime! This phenomenon persists even after we perform data sanitization
procedures to drastically reduce the noise in the training data, as illustrated
by our experiments in Figure~\ref{fig:teaser_plot_nn} (we provide details on the
experimental setup in Section~\ref{sec:appendix_experiments} of the Appendix).

% These experimental findings suggest that robust notions of performance still
% require regularization even for overparameterized models. The goal of this
% paper is to understand the causes of this phenomenon and investigate the
% following question theoretically: 
% 
% \begin{center} 
% 
% %   \emph{If the data is noiseless/In the highly overparameterized regime where
%   %   variance is low, when is it still beneficial to avoid perfectly fitting
%   %   the training data/minimizing the training loss?}
%   \emph{In the highly overparameterized regime in which variance is low, why is
%   it still beneficial to avoid perfectly fitting the training data?}
% 
% \end{center}
% 
% \rh{This formulation of a question is too vague, can we formulated it
% differently? Also, the question should contain some reference to robustness,
% because that is central. Perhaps this question: ``Is there a provable robustness
% benefit of regularizing interpolating models in the noiseless regime?''. If we
% can't find a good formulation here, we can also work without posing a concrete
% question.}
%``....'' Here we need a more concrete question that we actually answer, than
%the one emphasized below.  }

%These experimental findings indicate that the current perspective on
%the benefits of interpolation in high dimensions may be incomplete,
%and that one may arrive at a different conclusion if robustness is
%considered for evaluation \fy{imprecise sentence in part due to
%  passive voice. which different conclusion?}. In this paper we aim to
%fill this gap and study the following question:
%


\fy{not sure I'd use ``interpolate'' here}
% Further, it seems that when measuring the adversarially robust risk or
% worst-group generalization, early stopping before the training loss vanishes in
% fact improves generalization (\emph{robust overfitting}), even for very wide
% overparameterized models! \fy{cite rice, pangwei} Also, even after proposed
% noise sanitization procedures on very simple images,~\ref{fig:teaser}, we still
% observe robust overfitting.

%% Generalization performance measure using risk / test metric.
%% Risks that
%%  we care about: natural/standard + robust 
%% distributional robustness
%% adversarial robustness (related)
%% Image experiments also find robust overfitting but only give explanation for noisy and argue noiseless 
%% Generalization / excess risk depends on a term that is nonzero only when there’s noise (we say variance…?) and another term that is driven by optimization procedure, averaged over training data (we call bias)

These experimental findings suggest that robust notions of performance still
require regularization even for overparameterized models. When the training data
does not contradict the ground truth, for example for noiseless observations or
for adversarial training with consistent perturbations \cite{Raghunathan20},
then a natural intuition is that leveraging all signals perfectly should help to
achieve best generalization.
% contains samples of the ground truth  \fy{I want to include consistent
% adversarial perturbations here} without noise, a natural intuition is that
% leveraging all signals perfectly should help to achieve best generalization.
%% Even though when working with noiseless data a natural reflex is to
%% use all the signal in the training set and interpolate to achieve the
%% best generalization, there exist examples \fy{of what?} that indicate
%% otherwise.
For instance, it is well-known that when the ground truth has a low-dimensional
structure matched by the implicit bias of the estimator, we can hope to achieve
good generalization even with relatively little data, as is the case for the
lasso estimator \cite{Tibshirani96}. However, in the case of a structural
mismatch, interpolation may not suffice to find a satisfactory overparameterized
estimator.

In particular, our main contribution is that we show theoretically that
achieving zero training loss does not lead to an optimal adversarially robust
risk for linear regression and classification, even in noiseless settings.
Moreover, we prove that $\ell_2$ regularization or early stopping can
significantly improve performance even for robust estimators trained with
adversarial training, a phenomenon previously observed empirically for neural
networks and referred to as robust overfitting \cite{Rice20}.

The next section introduces notation used throughout the paper and makes a
connection between adversarial and distributional robustness for linear models.
In Section~\ref{sec:linreg} we give precise asymptotics for the robust risk of
the ridge estimator and the minimum norm interpolator in the context of linear
regression. Then, in Section~\ref{sec:logreg} we show that adversarial training
for logistic regression can benefit from ridge regularization and provide
insights explaining this phenomenon.

% When the amount of noise in the data is insignificant, a natural reflex is to
% use all the signal in the training set and interpolate to achieve the best
% generalization. 

% A natural reflex is to say that even though in the overparameterized regime we
% are given little information about the function, we should use as much true data
% as possible, and deliberately avoiding interpolation would not help
% generalization. It is well known that in the case when the implicit bias of the
% interpolator matches a ground truth that has low-dimensional structure, we can
% hope to achieve good generalization even with relatively little data \fy{lasso
% etc.} However in the case of a structural mismatch, this might not be the case.
% For example, a recent paper shows for linear regression, how adding a new
% noiseless data point data can decrease prediction accuracy when the test
% distribution favors certain directions.  \fy{could cite our tradeoff paper - it
% is the only work in this direction that I know but its very ehm toy ...  don't
% have to cite, also makes the sentence harder}
% 
% In this work, we prove for linear regression and classification, that perfectly
% fitting all available noiseless samples is often undesirable in many scenarios,
% in particular for the robust risk. In Section bla we do bla.




%% Motivated by the observation that large deep neural networks \fy{cite
%%   Chiyuan,openai} \rh{perhaps zhang UnderstandingDeepLearning 2016} perform well, in recent years increasing attention has been
%% devoted in the field of learning theory to study when
%% estimators that achieve perfect train accuracy still generalize well.
%% %% interpolation \fy{maybe zero empirical risk sth...? unclear for classification}
%% %% with overparameterized models
%% %% still yields estimators with good
%% %% generalization properties \fy{a bit long}.
%% These papers show that overparameterization acts as implicit regularization as it reduces the variance in the high-dimensional regime when
%% $d,n\to\infty$ \fy{not sure if good to bring up here}. For certain distributions, it is even possible to
%% reach consistency \fy{cite benign, vidya, ghorbani etc.}. This
%% phenomenon is often manifested in a double descent shaped risk curve, where the risk as a function of the amount of overparameterization first decreases, then increases, and finally decreases again.
%% This is observed for a variety of machine learning models, including linear and logistic regression, random features and kernel
%% regression. \fy{citestuff}
%% %\rh{Perhaps better to not mention double descent so prominently here, because this is not central to the storyline (unless I'm missing something)}


%% %A common story and conclusion of these papers is to just interpolate without the need to regularize as the overparameterization ratio increases.  
%% This development suggests that training to interpolation without regularization is sufficient to obtain a well-performing model. 
%% However these conclusions were based on studying the
%% standard population risk only. Modern machine learning practice
%% often requires models to also exhibit certain degrees of reliability
%% and fairness such as robust against distribution shifts,
%% adversarial perturbations, and the ability to achieve good worst-group performances
%% \fy{citestuff}. Lately, there has been rising empirical evidence that
%% common methods to tackle these \emph{robust risks} in fact
%% \emph{benefit from regularization that prevent interpolation} even in
%% the overparameterized regime. This phenomenon, referred to as
%% \emph{robust overfitting} in some contexts, has been observed for
%% $\ell_\infty$ robustness and worst-group generalization for images.
%% \fy{cite pangwei and rice}. This raises the question:

%% \begin{center}

%% When does regularization regain its merits when measuring robust generalization?

%% \end{center}

%% Some works following the observations of \rh{cite pangwei and rice again} conjectured explanations based on experimental
%% evidence.  In particular they argue that robust overfitting is caused
%% by noisy or ambiguous samples in the training data
%% \cite{Amartya20,Dong21} and suggest filtering methods that can eradicate/mitigate
%% the phenomenon.
%% %That is, the robust risk and adversarial
%% %training amplify the variance due to noise and hence benefit more from
%% %regularization.
%% %reminiscent of similar geometric arguments  made in
%% %earlier work \fy{Gilmerblowup, goldstein stuff?}.
%% \fy{is it that we contradict the tautology paper with mnist 1,3
%%   or is it just that we show for pruned and unpruned, gap doesn't change?}
%% %% However recent results suggest that CIFAR-10 \fy{is not really that noisy},
%% %% and furthermore
%% However, as shown in Figure~\ref{fig:teaser}, simple experiments using the proposed variance
%% reduction methods \fy{is that true} suggest that robust overfitting persists even on MNIST
%% with a simple RELU MLP when the bootstrap estimated variance is below \fy{bla}.
%% \fy{explain gap in one sentence}

%% It is hard to rigorously verify or falsify that datasets such as CIFAR-10 are indeed noisy,
%% even though small bootstrap estimated variances \fy{steinhardt} and $99.7\%$
%% test performance with the latest architecture \fy{cite} suggest that label noise is indeed neglible.
%% To challenge this hypothesis, Figure~\ref{fig:teaser} shows that even after
%% noise reduction with a final variance of ..., robust accuracy persists
%% the overfitting gap of a
%% neural network trained on a pruned binary classification task where only classes
%% 1 and 3 from the MNIST data set were considered. We can still observe robust
%% overfitting in this sanitized setting, where the noise has been reduced
%% significantly. Perhaps surprisingly, even overparameterized models with
%% remarkably low variance still exhibit robust overfitting and benefit from
%% early-stopping regularization. This observation raises the following question:

%% \begin{center}

%%   \emph{Are there situations when preventing interpolation can actually be
%%   beneficial for overparameterized models?}

%% \end{center}


\begin{figure*}
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_nn.pdf}
    \caption{Neural network}
    \label{fig:teaser_plot_nn}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_linreg.pdf}
    \caption{Linear regression}
    \label{fig:teaser_plot_linreg}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_plot_logreg.pdf}
    \caption{Linear classification}
    \label{fig:teaser_plot_logreg}
  \end{subfigure}

  \caption{ In this plot we show the gap between the standard and
    distributionally robust risk of the best regularized and final estimator for
    a (a) two-layer neural network with varying width, trained on (binary
    $1$-$3$) MNIST after using suggested variance reduction methods (see
    Appendix~\ref{sec:appendix_experiments}, regularized using early stopping .
    (b) linear regression on noiseless observations (c) distributionally robust
    training on logistic regression. The robust risk benefits significantly from
    regularization. For logistic regression, the standard risk also overfits
    however to a lesser extent than the robust risk.
    %% Performance gap between unregularized and optimally regularized estimators
    %% in simple noiseless interpolating settings.
    %% Subfigure \ref{fig:teaser_plot_nn} shows the performance of a two-layer neural networks with varying width, trained on (binary $1$-$3$) MNIST and evaluated with respect to $\ell_{\infty}$-perturbations.
    %% To reduce variance, we discard all training samples which a separately trained estimator cannot easily fit. We refer to
    %% \suppmat~\ref{sec:appendix_experiments} for the details.
    %% \ref{fig:teaser_plot_linreg} is linear regression standard training on noiseless synthetic data
    %% evaluated wrt $\ell_2$ perturbations.
    %% \ref{fig:teaser_plot_logreg} is logistic regression adversarial training on noiseless synthetic data
    %% trained and evaluated wrt $\ell_\infty$ perturbations. 
    %% The experiments shows that--even with the suggested variance reduction technique--the robust risk overfits (i.e., there is a non-zero gap between optimally regularized and the non-regularized estimate). 
%    \rh{Can we have a sentence summarizing the main conclusion from the
    %    experiment here, like: ``Even with the suggested variance reduction
    %    method, the robust overfitting phenomena persists.} a) The gap between
    %    optimal early stopped and final standard and robust risk with respect
    %    to $\ell_{\infty}$ perturbations for a single
%     hidden layer neural network with varying width on the binary $1$-$3$
    %     MNIST.  To reduce the variance, we additionally prune the samples
    %     which are not fitted by a separately trained estimator after early
    %     stopping.\ b) The estimated variance of the original and pruned data
    %     set. We refer to \suppmat~\ref{sec:appendix_experiments} for the
    %     details.
%   To reduce potential noise in the training set and fitting procedure, we
    %   discard all training samples which are not correctly classified within
    %   the first 100 epochs of training Nevertheless, we still observe
    %   significant robust overfitting in \ref{fig:teaser_overfitting}.  In
    %   order to quantify the amount of noise at hand,
%   we estimate model variances on the test set for each number of hidden units.
    %   \ref{fig:teaser_variances} shows the estimated variance averaged all
    %   test samples with bars indicating one empirical standard deviation.
    %   While the estimated variance for the full training set is already low,
    %   our pruning procedure further reduces it.
%   Artificial low-noise setting which exhibits significant robust overfitting.
    %   We fit a single hidden layer neural network with varying width on two
    %   MNIST classes.  To reduce potential noise in the training set and
    %   fitting procedure, we discard all training samples which are not
    %   correctly classified within the first 100 epochs of training
%   Nevertheless, we still observe significant robust overfitting in
    %   \ref{fig:teaser_overfitting}.  In order to quantify the amount of noise
    %   at hand, we estimate model variances on the test set for each number of
    %   hidden units.  \ref{fig:teaser_variances} shows the estimated variance
    %   averaged all test samples with bars indicating one empirical standard
    %   deviation.  While the estimated variance for the full training set is
    %   already low, our pruning procedure further reduces it.
  }

  \label{fig:teaser}
\end{figure*}
% 

%% Indeed, in this paper we show that robust overfitting occurs for
%% linear models \emph{even in the noiseless setting} in the heavily
%% overparameterized regime, illustrated in Figure~\ref{fig:teaser}.  We
%% prove robust overfitting of interpolating estimators for linear and
%% logistic regression in the high-dimensional regime.  In particular, we
%% show that in the overparameterized regime, i.e., for large overparameterization ratios $d/n \to \gamma$ and $d,n\to\infty$ regularization significantly improves generalization on the robust risk even though it does not benefit standard generalization. 
%% With this
%% work we'd like to provide a clear \fy{other word} counterpoint to an
%% increasing line of work that focuses on the diminished relevance of
%% regularization in the overparameterized regime.

%% %studies benefitsof overparameterization.

%% In section we do bla.

%% In this paper we answer this question in the positive and show that evaluating
%% adversarial robustness is one such setting where regularization does more than
%% only reduce variance.  Our main \textbf{contribution} is that we show that, for
%% both linear regression and logistic regression, the consistent robust risk
%% benefits from ridge regularization or early stopping even on noiseless
%% observations. Furthermore, this form of overfitting occurs only in the
%% overparameterized regime where the standard error benefits from the implicit
%% regularization that is characteristic for interpolating models. However, our
%% results demonstrate that interpolation can be harmful even when the standard
%% error does not suffer from overfitting.  Thus, we argue that regularization
%% plays a fundamentally different role for the consistent robust risk and acts not
%% just on the variance, but also as a form of bias reduction. To the best of our
%% knowledge, we are the first to study theoretically the impact of early stopping
%% and ridge regularization on the consistent robust risk for overparameterized
%% models. 

%% The double descent phenomenon, which has recently gained popularity in the
%% machine learning community, points to the beneficial effects of
%% overparameterization.  The effect of implicit regularization due to
%% overparameterizating has been first explicitly pointed out by \citet{Zhang17}
%% for deep neural networks where it is shown that these models achieve good
%% generalization performance although interpolating the train data. Surprisingly,
%% these observations put into perspective the classical wisdom on the
%% bias-variance trade-off which tells us us that the bias decreases and variance
%% increases with model complexity [TODO cite textbook]. Since then, a modern line
%% of statistical and machine learning research has emerged studying this effect
%% more carefully. In particular, the paper \cite{Nakkiran20,Yang20} observe that
%% the variance of deep neural networks decreases again after the interpolation
%% threshold when further increasing the model complexity, and hence achieve a
%% similar effect to regularization. 

%% Multiple papers from the statistical side underline this observation by proving
%% that such a behavior also occurs for classical regression and classification
%% algorithms including linear, logistic and random feature regression
%% \cite{Belkin19,Nakkiran20,Hastie19,Mei19,Deng20,Chinot21}. In fact, it has even
%% been shown that for certain spiked covariance data models both logistic and
%% linear regression can be asymptotically consistent in high dimensional regimes
%% albeit interpolating noisy train data \cite{Bartlett20,Muthukumar20}. In
%% summary, these papers suggest that the effect of implicit regularization in
%% overparameterized regimes makes explicit variance reduction techniques like
%% early stopping or ridge regularization redundant. 

%% All of these works have focused on the effect of overparameterization on the
%% prediction error of estimators. However, in many practical applications we are
%% interested in other criteria for evaluation as well, such as ensuring fair
%% predictors [TODO cite], or models that generalize well under covariate shift
%% [TODO cite]. Another example of a desirable property of prediction models, known
%% as \emph{adversarial robustness}, is that they are invariant to small (in
%% $\ell_p$ norm) additive perturbations of the input data \cite{Szegedy14}.
%% % For instance, in the case of image data sets these perturbations are often
%% % imperceptible to a human and, thus, do not change the semantics or the label
%% % of the inputs.
%% In order to avoid an ill-defined problem, it is crucial that the notion of
%% robustness that we use is not at odds with the other goal, which is to recover
%% the ground truth function and to achieve a low prediction error. To ensure that
%% we do not have interfering objectives, we only consider consistent perturbations
%% for evaluating the models, namely perturbations that do not change the value of
%% the ground truth function [TODO cite]. For linear models, consistent adversarial
%% robustness has even more profound consequences: perfect $\ell_p$ robustness
%% against consistent perturbations implies automatically robustness to
%% distribution shifts along any direction perpendicular to the linear ground
%% truth. This invariance to changes along directions that are independent of the
%% ground truth is of great importance in practice, in particular in situations
%% where fairness is important or when we do not wish to make predictions that rely
%% on spurious features.

% On top of achieving a low prediction accuracy on unseen test samples, in
% practical applications we often require the models to be robustness against
% perturbations in the input data.  \textit{say somehting here, but i really
% dont know the literature. This must be good, for instance we could mention
% fairness or distribution shifts? But motivate well why we do want a low robust
% risk BEYOND image data sets! Also motivate consistent perturbations}

% Modern machine learning models have to be vulnerable to imperceptible
% perturbations of the inputs \cite{Szegedy14}. This worrisome behavior has
% garnered a lot of attention in recent years and it spurred several lines of
% work that try to propose ways to defend against such adversarial attacks. Even
% though many of the suggested defences have been breached by carefully designed
% attacks \cite{Tramer20}, there are two approaches that stand out. Firstly,
% adversarial training \cite{Goodfellow15} has consistently been reliable even
% in the face of these newly discovered attacks. Secondly, a number of works
% have proposed certified defences \cite{Salman19, Balunovic19} which come with
% appealing robustness guarantees.

%% One popular approach to improve the robustness of a model to adversarial
%% $\ell_p$-perturbations is to use adversarial training (AT) where we minimize the
%% empirical risk with perturbed input train samples. This method has successfully
%% been applied to various models including deep neural networks
%% \cite{Goodfellow15} but also linear and logistic regression
%% \cite{Javanmard20a,Javanmard20b}. In a recent paper \cite{Rice20} the authors
%% uncover an interesting phenomenon: When minimizing the adversarial training loss
%% using an iterative algorithm (e.g.\ stochastic gradient descent), the
%% optimization path passes through a more robust solution first, before it
%% converges to a less robust one. Hence, an early-stopped model has better robust
%% accuracy, as measured on a hold out test set, than a model trained to
%% convergence. What makes this phenomenon surprising is that the authors observe
%% it for highly overparameterized deep neural networks where the natural test
%% error does not suffer from overfitting despite interpolating the train samples. 

%  A natural approach is to try and understand robust overfitting through the
%  lens of regular overfitting of the standard accuracy.  For a long time, the
%  classical statistics literature has pointed at noise as the major culprit for
%  overfitting.  More recently, a new story line has started to emerge:
%  overparameterization alone can mitigate overfitting by reducing the variance,
%  a phenomenon that is often referred to as `double descent`. One important
%  conclusion stressed by this line of work is that regularization is redundant
%  in the highly overparameterized regime.



% Our contributions are as follows:
% \begin{itemize}[leftmargin=*]
% 
%   \item for linear regression, we show that the consistent $\ell_2$ robust risk
%     benefits from ridge regularization or early stopping even on completely
%     noiseless observations. Furthermore, the described effect is only observed
%     in the overparameterized regime where the standard error benefits from the
%     implicit regularization described in \cite{Hastie19}.
% 
%   \item for classification, we study the consistent $\ell_{\infty}$ robust risk
%     for logistic regression and show that the adversarially trained estimator
%     suffers from overfitting of both the standard and robust risk, even in the
%     noiseless case. \at{TODO need to fit the next two sentences with the rest of
%     the story} Finally, we show that when adding label noise we need a higher
%     degree of overparameterization $d/n$ to interpolate the train data.
%     Surprisingly, this leads to the observation that the unregularized estimator
%     trained with noise achieves a lower final robust and standard risk compared
%     to the one trained without label noise.

%   \item for classification, we study the consistent $\ell_{\infty}$ robust
%     for logistic regression. Since standard training achieves only very poor robust risk, we focus on the adversarially trained estimator and show that this suffers from overfitting of both the standard and robust risk, even in the
%     noiseless case.
% \end{itemize}

% As a first contribution, we show that the consistent $\ell_2$-adversarial robust
% risk of linear regression benefits form ridge regularization or equivalently
% early stopping even on completely noiseless observations.  In this case, the
% variance of the standard risk is zero and hence suffers from explicit
% regularization. Our results demonstrate that interpolation can be harmful even
% when the standard error does not suffer from overfitting. Thus, we can conclude
% that regularization plays a fundamental different role for the consistent robust
% risk and Furthermore, the described effect is only observed in the
% overparameterized regime where the standard error benefits form the effect of
% implicit regularization as describe in the paper \cite{Hastie19}. 

% As a second contribution this paper studies the consistent
% $\ell_{\infty}$-adversarial robust risk for logistic regression on a
% discriminative sparse linear data model. While the standard trained estimator
% achieves very poor robust population accuracy close to $0$, the adversarially
% trained estimator trained with inconsistent adversarial $\ell_{\infty}$ attacks
% achieves a significantly better standard and robust test accuracy albeit still
% being able to interpolate the train samples. Surprisingly, however, we show that
% even in the noiseless case the estimator suffers from overfitting of both the
% standard and robust risk. While inconsistent attacks may induce some noise
% during training even for noiseless data, we also show that the we observe
% overfitting of the risks when training with consistent adversarial attacks
% assuming that we have full knowledge of the ground truth during training.
% Finally, we show that when adding label noise we need a higher degree of
% overparameterization $d/n$ to interpolate the train data. Surprisingly, this
% leads to the effect that the unregularized estimator trained with noise achieves
% a lower final robust and standard risk compared to the one trained without label
% noise. 

% Both examples demonstrate how interpolation suffers from overfitting in the
% overparameterized regime even for noiseless train data. As a result, this paper
% puts into perspective the modern story line on the implicit regularization due
% to overparameterization by highlighting that additional robustness constrains
% still require additional explicit regularization to prevent the model from
% interpolation. 





% This puts the modern story line on regularization into perspecti observes a
% vanishing In particular, we show that the robust risk suffers from overfitting
% even on noiseless which questions the 
% 
% 






% « In the paper \cite{Amatya20} the authors show that the robust accuracy is
% much more sensitive to noise in the train data than the standard accuracy.
% Although the experiments in the paper \cite{Rice20} are conducted on the
% original \textit{CIFAR-10} \cite{Krizhevsky09} dataset without any additional
% label noise, the authors from the paper \cite{Amatya20} highlight that these
% there are still misslabeled/wrong samples contained in the dataset. Therefore,
% the authors suggest that the overfitting of the robust risk may be explained
% due to a higher sensitivity to noise fitted by the estimator. A similar
% conclusion is suggested by the paper \cite{Dong21}, where the authors observe
% that the robust risk does not overfit when removing problematic samples which
% are not fit by a early stopped estimator form the data. 


% Yet this phenomenon not yet well understood and existing attempts to explain
% the phenomenon have predominantly linked it to noise respectively problematic
% samples in the train data. In the paper \cite{Amatya20} the authors show that
% the robust accuracy is much more sensitive to noise in the train data than the
% standard accuracy.  Although the experiments in the paper \cite{Rice20} are
% conducted on the original \textit{CIFAR-10} \cite{Krizhevsky09} dataset
% without any additional label noise, the authors from the paper \cite{Amatya20}
% highlight that these there are still misslabeled/wrong samples contained in
% the dataset. Therefore, the authors suggest that the overfitting of the robust
% risk may be explained due to a higher sensitivity to noise fitted by the
% estimator. A similar conclusion is suggested by the paper \cite{Dong21}, where
% the authors observe that the robust risk does not overfit when removing
% problematic samples which are not fit by a early stopped estimator form the
% data. 
% 
% While noisy/problematic samples in the train data certainly have an effect on
% the robust accuarcy, we observe in Figure~\ref{fig:teaser} that the robust
% accuracy overfits even on binary 1-3-MNIST with additional pruning of unfitted
% samples by a early stopped neural network. In this paper we aim to better
% understand 



% ttempt to explain the overfitting of the robust accuarcy due to an
% oversensitivity to noise in the train data.  samples. While noise in the train
% data clearly has an impact on robust overfitting (see Figure \ref{fig:asdf}),
% this paper shows that robust overfitting also occurs   noiseless settings
% where the natural accuracy does not benefit from regularization at all. Hence,
% this paper challenges the role of regularization: In the classical
% understanding we have that in the well specified setting, regularization leads
% to a bias-variance tradeoff, meaning that we increase bias but decrease
% variance. In particualr, this suggests that if you have no noise,
% regularization does not improve performance.  More specifically, this paper is
% the first one theoretically studying overfitting of the robust loss. Unlike
% existing literature we \kd{continue to write soon }


% 
% Mission of the paper: Hence we seek to complete the picture by proving the
% conjecture for lin reg The conjecture: in settings: ST, AT, noiseless … … when
% evaluating the robust error, early stopping is needed for a much wider range
% of d/n and p/n ratios, compared to testing using the std error Our
% contributions: We prove … … this conjecture is true in the settings above for
% linear models (lin reg).  in particular our claim is that …. causes it. (proof
% intuition) We also show experimentally that indeed RO happens in these
% settings and second the intuition carries through to images. 






% \kd{A bit a repetition from the intro}
% Robust overfitting is the intriguing phenomenon that has been observed by
% \cite{Rice20} on neural networks trained with adversarial training: early
% stopping regularization has a significant effect in reducing the robust test
% error, while, in contrast, the standard test error is always non-increasing as a
% function of time. \kd{Rice does this as well, need to write more here} In this
% section we provide empirical evidence that robust overfitting occurs even in a
% noiseless setting, raising questions about the nature of the phenomenon.

% \kd{this is already contained in the intro: A natural approach is to try and
% understand robust overfitting through the lens of regular overfitting of the
% standard accuracy. For a long time, the classical statistics literature has
% pointed at noise as the major culprit for overfitting.  More recently, a new
% story line has started to emerge: overparameterization alone can mitigate
% overfitting by reducing the variance, a phenomenon that is often referred to
% as `double descent`. One important conclusion stressed by this line of work is
% that regularization is redundant in the highly overparameterized regime.
% 
% Robust overfitting is indeed exacerbated by noise. Adding artificial label
% noise to the training data makes robust overfitting much more pronounced, as
% we show in Appendix TODO for overparameterized fully-connected neural
% networks. However, going in the opposite direction and \textit{reducing} the
% amount of noise of the prediction problem to a minimum reveals a surprising
% situation. In a noiseless setting where the variance vanishes, it seems like a
% sensible hypothesis is that regularization has no effect on the test robust
% error.  }

% \citet{Rice20} showed that the robust loss overfits when training
% overparameterized deep neural networks on CIFAR \cite{Krizhevsky09} without
% adding any additional label noise. However, as highlighted by \citet{Sanyal21}
% the original data set itself cointains noisy samples. Hence, we cannot
% conclude from the presented experiments that robust overfitting occurs even in
% the absence of noise. 

% , the following experiments indicate that, for overparameterized models, the
% role of regularization is not lpimited to just reducing the variance.




% The observation that regularization is beneficial even in a noiseless setting
% raises the following question:
% 
% \begin{center}
% 
%   \textit{Can regularization reduce the bias of overparameterized models \\
%   with respect to certain evaluation metrics?}
% 
% \end{center}
% 
% In particular, is it the case that certain traditional regularization
% techniques are better suited at priming estimators for robust evaluation? In
% the sequel we analyze lineapr and logistic regression in the context of
% adversarial robustness and prove that, in high dimensions, early stopping and
% ridge regularization lead to more robust predictors.


==> neurips_poster/AMS_commands.tex <==
%  Commands related to theorems, definitions, lemma etc.



\theoremstyle{plain}

\newtheorem{theo}{Theorem}[section]
\newtheorem{theonosec}{Theorem}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{cor}{Corollary}[section]

\theoremstyle{definition} 

\newtheorem{nota}{Notation}[section]
\newtheorem{de}{Definition}[section]
\newtheorem{exa}{Example}[section]
\newtheorem{as}{Assumption}[section]
\newtheorem{alg}{Algorithm}[section]


\newcommand{\btheo}{\begin{theo}}
\newcommand{\bde}{\begin{de}}
\newcommand{\ble}{\begin{lem}}
\newcommand{\bpr}{\begin{prop}}
\newcommand{\bno}{\begin{nota}}
\newcommand{\bex}{\begin{exa}}
\newcommand{\bcor}{\begin{cor}}
\newcommand{\spro}{\begin{proof}}
\newcommand{\bas}{\begin{as}}
\newcommand{\balg}{\begin{alg}}

\newcommand{\etheo}{\end{theo}}
\newcommand{\ede}{\end{de}}
\newcommand{\ele}{\end{lem}}
\newcommand{\epr}{\end{prop}}
\newcommand{\eno}{\end{nota}}
\newcommand{\eex}{\end{exa}}
\newcommand{\ecor}{\end{cor}}
\newcommand{\fpro}{\end{proof}}
\newcommand{\eas}{\end{as}}
\newcommand{\ealg}{\end{alg}}


%%%%%%%%
\theoremstyle{plain}

\newtheorem{theos}{Theorem}
\newtheorem{props}{Proposition}
\newtheorem{lems}{Lemma}
\newtheorem{cors}{Corollary}
\newtheorem{rems}{Remark}

\theoremstyle{definition}
\newtheorem{exas}{Example}
\newtheorem{algs}{Algorithm}
\newtheorem{asss}{Assumption}
\newtheorem{defns}{Definition}

\newcommand{\btheos}{\begin{theos}}
\newcommand{\etheos}{\end{theos}}
\newcommand{\brems}{\begin{remark}}
\newcommand{\erems}{\end{remark}}
\newcommand{\bprops}{\begin{props}}
\newcommand{\eprops}{\end{props}}
\newcommand{\bdes}{\begin{defns}}
\newcommand{\edes}{\end{defns}}
\newcommand{\blems}{\begin{lems}}
\newcommand{\elems}{\end{lems}}
\newcommand{\bcors}{\begin{cors}}
\newcommand{\ecors}{\end{cors}}
\newcommand{\bexs}{\begin{exas}}
\newcommand{\eexs}{\end{exas}}
\newcommand{\balgs}{\begin{algs}}
\newcommand{\ealgs}{\end{algs}}
\newcommand{\bass}{\begin{asss}}
\newcommand{\eass}{\end{asss}}



==> neurips_poster/BookMacros <==



\newcommand{\CliqueNum}{\ensuremath{\mathcal{C}}}



\newcommand{\INDSTARI}{\ensuremath{\mathbb{I}[|\inprod{\thetastar}{x_i}|
      \leq T]}}
\newcommand{\INDSTAR}{\ensuremath{\mathbb{I}[|\inprod{\thetastar}{x}|
      \leq T]}}
\newcommand{\INDSTARCOM}{\ensuremath{\mathbb{I}[|\inprod{\thetastar}{x}|
      > T]}}
\newcommand{\TRUNFUNSPEC}[1]{\ensuremath{\varphi_{\trunpar(#1)}}}

\newcommand{\trunpar}{\ensuremath{\tau}}

\newcommand{\TRUNFUNTWO}{\ensuremath{\widetilde{\varphi}_\trunpar}}

\newcommand{\Excess}{\ensuremath{E}}

\newcommand{\myparagraph}[1]{\noindent {\bf{#1}} $\;$}
\newcommand{\MYPARAGRAPH}[1]{\noindent {\bf{#1}} $\;$}

\newcommand{\realepscrit}{\ensuremath{\varepsilon_\numobs}}

\newcommand{\mccon}{\ensuremath{\beta}}

\newcommand{\NSUP}{\ensuremath{N_{\mbox{\tiny{sup}}}}}

\newcommand{\Qbar}{\ensuremath{\widebar{\qprob}}}
\newcommand{\mypackdens}[1]{\ensuremath{f_{#1}}}
\newcommand{\mypackprob}[1]{\ensuremath{\mprob_{#1}}}

\newcommand{\SetClassZero}{\ensuremath{\SetClass_0}}
\newcommand{\SetClassOne}{\ensuremath{\SetClass_1}}


\newcommand{\vcprime}[1]{\ensuremath{\vc'(#1)}}

\newcommand{\MSMALL}{\ensuremath{C}} 

\newcommand{\half}{\ensuremath{\frac{1}{2}}}

\newcommand{\KLETSET}{\ensuremath{\Ball_{2, \Phi}}}
\newcommand{\rad}{\ensuremath{\rho}}
\newcommand{\bigrad}{\ensuremath{R}}

\newcommand{\ScaleFun}{\ensuremath{\Psi}}

\newcommand{\DiagCovHat}{\ensuremath{\mathbf{\widehat{D}}}}
\newcommand{\CovMatTil}{\ensuremath{\widetilde{\CovMat}}} 


\newcommand{\mutil}{\ensuremath{\widetilde{\mu}}}

\newcommand{\fdens}{f_0}

\newcommand{\alphastar}{\ensuremath{\alpha^*}}
\newcommand{\DelHatAlpha}{\ensuremath{\DelHat_{\alpha}}}
\newcommand{\DelHatBeta}{\ensuremath{\DelHat_{\beta}}}
\newcommand{\DeltaAlpha}{\ensuremath{\Delta_{\alpha}}}
\newcommand{\DeltaBeta}{\ensuremath{\Delta_{\beta}}}

\newcommand{\mytiny}[1]{\mbox{\scalebox{.5}{#1}}}
\newcommand{\mylarge}[1]{\mbox{\scalebox{.8}{#1}}}



%\newcommand{\tmpAset}{\ensuremath{\mathbb{L}_0}}
%\newcommand{\tmpBset}{\ensuremath{\mathbb{L}_1}} 
%\newcommand{\clconv}{\ensuremath{\widebar{\mbox{conv}}}}



\newcommand{\delmax}{\ensuremath{\delta_{\numobs, \mbox{\tiny{max}}}}}

\newcommand{\FclassEllOne}{\ensuremath{\Fclass_{\ell_1}}}

\newcommand{\Jlow}{\ensuremath{\GamMat_{\mbox{\tiny{low}}}}}

\newcommand{\pertvec}{\ensuremath{\Delta}}

\newcommand{\myspan}{\ensuremath{\operatorname{span}}}
\newcommand{\tagtheta}{\ensuremath{\beta}}


\newcommand{\hildist}{\ensuremath{\rho_\Hil}}


\newcommand{\SUPERSHATTER}[1]{\ensuremath{\Phi_{#1}}}
\newcommand{\UPPER}[1]{\ensuremath{\Psi_{#1}}}
\newcommand{\kindex}{\ensuremath{k}}


\newcommand{\GamMat}{\ensuremath{\mathbf{\Gamma}}}
\newcommand{\ThetaMat}{\ensuremath{\mathbf{\Theta}}}
\newcommand{\ThetaRR}{\ensuremath{\widehat{\ThetaMat}_{\mbox{\tiny{RR}}}}}
\newcommand{\LamMat}{\ensuremath{\mathbf{\Lambda}}}

\newcommand{\specthetatil}{\ensuremath{\widetilde{\gamma}}}

\newcommand{\FclassAdd}{\ensuremath{\Fclass_{\tiny{\mbox{add}}}}}

\newenvironment{carlist}
 {\begin{list}{$\bullet$}
 {\setlength{\topsep}{0in} \setlength{\partopsep}{0in}
  \setlength{\parsep}{0in} \setlength{\itemsep}{\parskip}
  \setlength{\leftmargin}{0.15in} \setlength{\rightmargin}{0.08in}
  \setlength{\listparindent}{0in} \setlength{\labelwidth}{0.08in}
  \setlength{\labelsep}{0.1in} \setlength{\itemindent}{0in}}}
 {\end{list}}

%\newcommand{\bcar}{\begin{carlist}}
%\newcommand{\ecar}{\end{carlist}}

\newcommand{\bcar}{\begin{itemize}}
\newcommand{\ecar}{\end{itemize}}

\newcommand{\tmpAset}{\ensuremath{\mathbb{L}_0}}
\newcommand{\tmpBset}{\ensuremath{\mathbb{L}_1}} 
\newcommand{\clconv}{\ensuremath{\widebar{\mbox{conv}}}}


\newcommand{\Constraint}{\ensuremath{\mathcal{C}}}
\newcommand{\hackxi}{z}
\newcommand{\HackXi}{Z}
\newcommand{\hackxitil}{\widetilde{\hackxi}}
\newcommand{\HackXiTil}{\widetilde{\HackXi}}


\newcommand{\matpar}{\ensuremath{\nu}}

\newcommand{\PsiEllOne}{\ensuremath{\Psi_{\ell_1}}}
\newcommand{\PsiHuber}{\ensuremath{\Psi_{\mbox{\scriptsize{Huber}}}}}
\newcommand{\HUBERCUT}{\ensuremath{\tau}}


\newcommand{\RealConstraint}{\ensuremath{\mathcal{C}}}

\newcommand{\delstar}{\ensuremath{\delta^*}}

\newcommand{\Fconvex}{\ensuremath{\Fclass_{\mbox{\tiny{conv}}}}}

\newcommand{\SEQTWO}[2]{\ensuremath{(#1_{#2})_{#2=1}^\infty}}
\newcommand{\SEQTHREE}[3]{\ensuremath{(#1_{#2})_{#2=1}^{#3}}}

\newcommand{\Fsparsecone}{\ensuremath{\Fclass_{\mbox{\tiny{spcone}}}}}

%\newcommand{\EYE}[1]{\ensuremath{\mymathbf{I}_{#1 \times #1}}}
\newcommand{\EYE}[1]{\ensuremath{\mymathbf{I}_{#1}}}
\newcommand{\EYETWO}[2]{\ensuremath{\mymathbf{I}_{#1 \times #2}}}
\newcommand{\ZEROMAT}[1]{\ensuremath{\mymathbf{0}_{#1}}}

%\newcommand{\ZeroMat}{\ensuremath{\mymathbf{0}}}

\newcommand{\Fadditive}{\ensuremath{\Fclass_{\mbox{\tiny{add}}}}}
\newcommand{\Fspam}{\ensuremath{\Fclass_{\mbox{\tiny{spam}}}}}

\newcommand{\MCON}{\ensuremath{C}}
\newcommand{\ftrun}{\ensuremath{f_\trunlevel}}



\newcommand{\Ytilspace}{\ensuremath{\widetilde{\Yspace}}}


\newcommand{\delcrittil}{\ensuremath{\widetilde{\delta}_\numobs}}
\newcommand{\delcritstar}{\ensuremath{\delta^*_\numobs}}

\newcommand{\TrunFunT}{\ensuremath{\varphi_\trunlevel}}
\newcommand{\trunlevel}{\ensuremath{\tau}}
\newcommand{\TrunFun}[1]{\ensuremath{\varphi_{#1}}}

\newcommand{\Zn}{\ensuremath{Z_\numobs}}

\newcommand{\HACKCONTWO}{16}

\newcommand{\EQUIVHACKCON}{64}
\newcommand{\Flip}{\ensuremath{\Fclass_{\mbox{\tiny{Lip}}}}}
\newcommand{\Flinear}{\ensuremath{\Fclass_{\mbox{\tiny{lin}}}}}

\newcommand{\Sevent}{\ensuremath{\mathcal{S}}}

\newcommand{\Scal}{\ensuremath{\mathcal{S}}}

\newcommand{\SpecBall}[2]{\ensuremath{\Ball_\numobs(#1; #2)}}



\newcommand{\starhull}[2]{\ensuremath{\mbox{star}(#1; \, #2)}} 
\newcommand{\plstarhull}[1]{\ensuremath{\mbox{star}(#1)}}

% Set difference notation
\newcommand{\DIFF}[1]{\ensuremath{\partial #1}}

\newcommand{\Fridge}{\ensuremath{\Fclass_{2}}}
\newcommand{\Fqpar}{\ensuremath{\Fclass_{\qpar}}}

%\newcommand{\SHIFT}[1]{\ensuremath{{#1}_{\fstar}}}
\newcommand{\SHIFT}[1]{\ensuremath{{#1}^*}}

\newcommand{\SEQ}[1]{\ensuremath{(#1)_{j=1}^\infty}}
\newcommand{\RKHS}{reproducing kernel Hilbert space}
\newcommand{\gindex}[1]{\index{general}{#1}}



\newcommand{\indpar}{\ensuremath{\gamma}}

\newcommand{\vstar}{\ensuremath{v^*}}
\newcommand{\vhat}{\ensuremath{\widehat{v}}}

\newcommand{\SamCovPert}{\ensuremath{\Pmat}}
\newcommand{\SamCovPertTil}{\ensuremath{\widetilde{\SamCovPert}}}

\newcommand{\pcamult}{\ensuremath{\xi}}



\newcommand{\RWIDTHPL}{\ensuremath{\mathcal{W}}}
\newcommand{\RWIDTH}[1]{\ensuremath{\RWIDTHPL(#1)}}
\newcommand{\RWIDTHSQ}[1]{\ensuremath{\RWIDTHPL^2(#1)}}

\newcommand{\DWIDTHPL}{\ensuremath{D}}
\newcommand{\DWIDTH}[1]{\ensuremath{\DWIDTHPL(#1)}}
\newcommand{\DWIDTHSQ}[1]{\ensuremath{\DWIDTHPL^2(#1)}}

\newcommand{\MYDATA}{\ensuremath{\{x_i\}_{i=1}^\numobs}}
\newcommand{\MVAL}{\ensuremath{\sqrt{M}}}
\newcommand{\MVALSQ}{\ensuremath{M}}

\newcommand{\eigengap}{\ensuremath{\nu}}


% Wedge and vee min and max
%\newcommand{\wmin}{\ensuremath{\wedge}}
%\newcommand{\vmax}{\ensuremath{\vee}}

\newcommand{\GRAPHSAM}[1]{\ensuremath{\{x_i\}_{i=1}^{#1}}}

\newcommand{\TRUNFUN}{\varphi_\trunlev}
\newcommand{\trunlev}{\ensuremath{\tau}}

\newcommand{\ASET}{\ensuremath{\mathbb{A}}}

\newcommand{\missfrac}{\ensuremath{\nu}}

\newcommand{\ThetaINCON}{\ensuremath{\widehat{\ThetaBf}_{\mbox{\tiny{NAI}}}}}

\newcommand{\UNICON}{\ensuremath{c}}


%\newcommand{\threshlev}{\ensuremath{\mu_\numobs}}
\newcommand{\threshlev}{\ensuremath{\nu_\numobs}}
\newcommand{\threshtil}{\ensuremath{\widetilde{\mu}_\numobs}}
\newcommand{\opbound}{\ensuremath{\nu_\numobs}}

\newcommand{\ej}{\ensuremath{j}}
\newcommand{\ek}{\ensuremath{k}}
\newcommand{\aind}{\ensuremath{a}}
\newcommand{\bind}{\ensuremath{b}}


\newcommand{\hana}{+}
\newcommand{\ThetaShack}{\ensuremath{\ThetaBf_{\ej \hana}}}
\newcommand{\ThetaShackHat}{\ensuremath{\widehat{\ThetaBf}_{\ej \hana}}}

\newcommand{\thetashack}{\ensuremath{\theta_{\ej \hana}}}
\newcommand{\thetashackhat}{\ensuremath{\widehat{\theta}_{\ej \hana}}}



\newcommand{\clipot}{\ensuremath{\phi}}
\newcommand{\statenum}{\ensuremath{M}}

\newcommand{\Fish}{\ensuremath{\mathbf{J}}}
\newcommand{\FishPlain}{\ensuremath{J}}
\newcommand{\FishStar}{\ensuremath{\Fish^*}}


\newcommand{\GamHat}{\ensuremath{\widehat{\GammaBf}}}
\newcommand{\GamHatPlain}{\ensuremath{\widehat{\Gamma}}}
\newcommand{\PlainGamHat}{\ensuremath{\GamHatPlain}}
\newcommand{\gamhat}{\ensuremath{\widehat{\gamma}}}


\newcommand{\ThetaHackStar}{\ensuremath{\ThetaBf^\diamond}}

\newcommand{\mateltone}[1]{\ensuremath{\|#1\|_{\tiny{\ell_1}}}}

\newcommand{\CutSet}{\ensuremath{S}}
\newcommand{\compat}{\ensuremath{\psi}}

\newcommand{\muparn}{\ensuremath{\mu_\numobs}}

\newcommand{\EMPPLAIN}[2]{\ensuremath{\mathcal{E}(#1 \, ; #2)}}
\newcommand{\LossPlain}{\ensuremath{\mathcal{L}}}
\newcommand{\RegOver}[1]{\Regplain_{\mbox{\tiny{over}}}(#1)}


\newcommand{\HACKZSAMP}{\ensuremath{Z}}

% Wedge and vee min and max
\newcommand{\wmin}{\ensuremath{\wedge}}
\newcommand{\vmax}{\ensuremath{\vee}}

\newcommand{\UsubR}{\ensuremath{\Usub^\rdim}}
\newcommand{\VsubR}{\ensuremath{\Vsub^\rdim}}

\newcommand{\fprime}{\ensuremath{\fbar}}
\newcommand{\alphabar}{\ensuremath{\bar{\alpha}}}
\newcommand{\nbar}{\ensuremath{\bar{\numobs}}} 


\newcommand{\omegan}{\ensuremath{\omega_\numobs}}
\newcommand{\omegansq}{\ensuremath{\omega^2_\numobs}}
\newcommand{\omegahat}{\ensuremath{\widehat{\omega}}}

\newcommand{\supp}{\ensuremath{\mbox{supp}}}

\newcommand{\DelSparse}{\ensuremath{\PertMat_{\Sparse}}}
\newcommand{\DelLowRank}{\ensuremath{\PertMat_{\LowRank}}}
\newcommand{\DelSparseHat}{\ensuremath{\PertMat_{\SparseHat}}}
\newcommand{\DelLowRankHat}{\ensuremath{\PertMat_{\LowRankHat}}}
\newcommand{\atil}{\ensuremath{\tilde{a}}}


\newcommand{\phasecon}{\ensuremath{c_0}}


\newcommand{\prad}{\ensuremath{\sqrt{\pradsq}}}
\newcommand{\pradsq}{\ensuremath{\rho}}


\newcommand{\USEGAM}{\ensuremath{\sqrt{\newgamma}}}
\newcommand{\newgamma}{\widebar{\gamma}}
\newcommand{\newkappa}{\ensuremath{\widebar{\kappa}}}


\newcommand{\TbarSmall}{\ensuremath{\bar{\Tmat}}}
\newcommand{\SUMN}{\ensuremath{\sum_{i=1}^\numobs}}
\newcommand{\SUMNF}{\ensuremath{\frac{1}{\numobs} \SUMN}}



\newcommand{\usedimmin}{\ensuremath{\usedim'}}

\newcommand{\BIGCON}{\ensuremath{C}}



\newcommand{\SEV}{\ensuremath{\sqrt{\frac{ \log \usedim}{\numobs}}}}
\newcommand{\SevVar}{\ensuremath{T}}
\newcommand{\lrad}{\ensuremath{r_\ell}}
\newcommand{\urad}{\ensuremath{r_u}}
\newcommand{\ESEV}{\ensuremath{2}}

\newcommand{\myemphparagraph}[1]{\noindent \emph{#1}}
\newcommand{\mybfparagraph}[1]{\noindent {\bf{#1}}}

\newcommand{\SpecSset}{\ensuremath{\mathbb{S}}}
\newcommand{\SHORTQ}{\ensuremath{\Qmat}}
\newcommand{\SpecSetTil}{\ensuremath{\widetilde{\SpecSet}}}
\newcommand{\SpecSsetTil}{\ensuremath{\widetilde{\SpecSset}}}



\newcommand{\myeigval}{\ensuremath{\gamma}}
\newcommand{\mysingval}{\ensuremath{\sigma}}

\newcommand{\mylammax}{\ensuremath{\myeigval_{\tiny{\mbox{max}}}}}
\newcommand{\mylammin}{\ensuremath{\myeigval_{\tiny{\mbox{min}}}}}
\newcommand{\myxsam}{\ensuremath{x}}
\newcommand{\CEXP}[1]{\ensuremath{e^{#1}}}
\newcommand{\CEXPBIG}[1]{\ensuremath{\exp \big(#1 \big)}}
\newcommand{\CEXPSUPERBIG}[1]{\ensuremath{\exp \Big(#1 \Big)}}
\newcommand{\matlam}{\ensuremath{\lambda}}
\newcommand{\mytrace}[1]{\ensuremath{\operatorname{tr} \big(#1 \big)}}

% Matrix regression X
\newcommand{\mrX}{\ensuremath{\Zmat}}



%\newcommand{\atil}{\ensuremath{a}}

\newcommand{\maxval}{\ensuremath{\alpha}}
\newcommand{\rscprecon}{\ensuremath{c_0}}
\newcommand{\HACK}{\ensuremath{\mathcal{K}}}
\newcommand{\DALCON}{\ensuremath{\ALCON}}
\newcommand{\ALCON}{\ensuremath{\alpha}}
\newcommand{\FERRSQ}[2]{\ensuremath{e^2(#1, \, #2)}}
\newcommand{\EventTil}{\ensuremath{\widetilde{\Event}}}


% Special notation for multivariate regression, number of predictors
\newcommand{\mrusedim}{\ensuremath{p}}

\newcommand{\MatA}{\ensuremath{\alpha}}
\newcommand{\MatB}{\ensuremath{\beta}}
\newcommand{\DeltaA}{\ensuremath{\Delta_\MatA}}
\newcommand{\DeltaB}{\ensuremath{\Delta_\MatB}}

\newcommand{\MatATil}{\ensuremath{\widebar{\MatA}}}
\newcommand{\MatBTil}{\ensuremath{\widebar{\MatB}}}

\newcommand{\SUPERSUB}{\ensuremath{\ModelSetOver(\BigSgroup)}}

\newcommand{\Row}{\ensuremath{\mathbf{\RowPlain}}}
\newcommand{\RowHat}{\ensuremath{\widehat{\Row}}}
\newcommand{\RowPlain}{\ensuremath{\Omega}}

\newcommand{\SUBA}{\ensuremath{\mathbb{M}_\MatA}}
\newcommand{\SUBB}{\ensuremath{\mathbb{M}_\MatB}}
\newcommand{\SUBAPERP}{\ensuremath{\SUBA^\perp}}
\newcommand{\SUBBPERP}{\ensuremath{\SUBB^\perp}}

\newcommand{\MatDecompNorm}[1]{\ensuremath{\Phi_{\omega}(#1)}}

\newcommand{\MatDecompNormSq}[1]{\ensuremath{\Phi^2_{\omega}(#1)}}

\newcommand{\smallxbar}{\ensuremath{\bar{x}}}

\newcommand{\sval}{\ensuremath{\mysingval}}


\newcommand{\Nrad}{\ensuremath{r}} 
\newcommand{\nradone}{\ensuremath{\Nrad_1}}
\newcommand{\nradtwo}{\ensuremath{\Nrad_2}}

\newcommand{\Lvar}{\ensuremath{Q}}


\newcommand{\sym}{\ensuremath{\operatorname{sym}}}

\newcommand{\rnum}{\ensuremath{r}}

%\newcommand{\BigSgroup}{\ensuremath{\Sset_{\mbox{\tiny{group}}}}}
%\newcommand{\BigSgroupTil}{\ensuremath{\widetilde{\Sset}_{\mbox{\tiny{group}}}}}


\newcommand{\BigSelt}{\ensuremath{\Sset_{\mbox{\tiny{elt}}}}}

\newcommand{\BigSgroup}{\ensuremath{\Sset_\Group}}
\newcommand{\BigSgroupTil}{\ensuremath{\widetilde{\Sset}_{\Group}}}



\newcommand{\Good}{\ensuremath{\mathbb{G}}}

\newcommand{\PiMat}{\ensuremath{\mathbf{\Pi}}}

\newcommand{\PINC}[1]{\ensuremath{\delta_{\mbox{\tiny{PW}}}(#1)}}
\newcommand{\perthat}{\ensuremath{\widehat{\perturb}}}


\newcommand{\lweight}{\ensuremath{\nu}}
\newcommand{\wellone}[1]{\ensuremath{\|#1\|_{\lweight(1)}}}
\newcommand{\wellinfty}[1]{\ensuremath{\|#1\|_{\lweight(\infty)}}}

\newcommand{\NewCset}{\ensuremath{\mathbb{T}}}

\newcommand{\ZmatHat}{\ensuremath{\widehat{\Zmat}}}

\newcommand{\Tbset}{\ensuremath{\mathbb{T}}}

\newcommand{\tworad}{\ensuremath{R}}
\newcommand{\twourad}{\ensuremath{\tworad_u}}
\newcommand{\twolrad}{\ensuremath{\tworad_\ell}}
\newcommand{\ANNOYPEEL}{\ensuremath{M_\numobs(\RegPlain; \tworad)}}


\newcommand{\Aset}{\ensuremath{\mathbb{A}}}

\newcommand{\RIP}[1]{\ensuremath{\delta_{#1}}}

\newcommand{\PlainReg}{\RegPlain}
\newcommand{\TayErrSing}{\ensuremath{\mathcal{E}}}
\newcommand{\TaySing}{\ensuremath{\TayErrSing}}

\newcommand{\EMPTAYPLAIN}{\ensuremath{\delLike}}
\newcommand{\POPTAYPLAIN}{\ensuremath{\delLikeBar}}
\newcommand{\EMPTAY}[1]{\ensuremath{\delLike(#1)}}
\newcommand{\POPTAY}[1]{\ensuremath{\delLikeBar(#1)}}

\newcommand{\SYM}[1]{\ensuremath{\mbox{sym}(#1)}}

\newcommand{\MYSCORE}[1]{\ensuremath{\nabla \Loss(#1)}}
\newcommand{\MYLOSS}[1]{\ensuremath{\Loss(#1)}}
\newcommand{\MYLOSSBAR}[1]{\ensuremath{\LossBar(#1)}}

\newcommand{\tbar}{\ensuremath{\widebar{t}}}

\newcommand{\LinkBound}{\ensuremath{B}}

\newcommand{\MYDUALREG}{\ensuremath{\mu_\numobs(\RegPlain^*)}}
\newcommand{\MYDUALREGSQ}{\ensuremath{\mu^2_\numobs(\RegPlain^*)}}

\newcommand{\PlainCovMat}{\ensuremath{\Sigma}}

\newcommand{\bspikeplain}{\ensuremath{\alpha}}
\newcommand{\nrad}{\ensuremath{\rho}}

\newcommand{\MYMAX}[2]{\ensuremath{\max\{#1, \, #2\}}}
\newcommand{\MYMAXX}[2]{\ensuremath{\max \Big\{#1, \, #2 \Big\}}}
\newcommand{\MYMIN}[2]{\ensuremath{\min\{#1, \, #2\}}}
\newcommand{\MYMINN}[2]{\ensuremath{\min \Big\{#1, \, #2 \Big\}}}
%\newcommand{\MYMIN}[2]{\ensuremath{ \{ #1 \wedge #2 \}}}

\newcommand{\BUHL}{\index{author}{B\"{u}hlmann, P.}}
\newcommand{\GEER}{\index{author}{van de Geer, S.}}
\newcommand{\CANDES}{\index{author}{Candes, E.}}
\newcommand{\TAO}{\index{author}{Tao, T.}}
\newcommand{\DON}{\index{author}{Donoho, D.}}

\newcommand{\ObsZ}{\ensuremath{Z}}
\newcommand{\BadEvent}{\ensuremath{\mathcal{E}}}
\newcommand{\BadEventZero}{\ensuremath{\BadEvent_0}}
\newcommand{\BadEventOne}{\ensuremath{\BadEvent_1}}



\newcommand{\Poly}{\ensuremath{\mathcal{P}}}

\newcommand{\Prob}{\ensuremath{\mprob}}



\newcommand{\subexpvarstar}{\ensuremath{\nu_*}}


\newcommand{\xprime}{\ensuremath{x'}}
\newcommand{\FrancisSet}{\ensuremath{\mathbb{S}}}

\newcommand{\usedimmax}{\ensuremath{\usedim{\,'}}}

\newcommand{\betaspike}{\ensuremath{\alpha_{\mbox{\tiny{sp}}}}}

\newcommand{\CovMatHat}{\ensuremath{\widehat{\CovMat}}}

\newcommand{\thetamin}{\ensuremath{\theta_{\mbox{\tiny{min}}}}}
\newcommand{\thetaminsq}{\ensuremath{\theta^2_{\mbox{\tiny{min}}}}}
\newcommand{\thetabar}{\widebar{\theta}}

\newcommand{\mprobbar}{\ensuremath{\bar{\mprob}}}
\newcommand{\qprobbar}{\ensuremath{\bar{\qprob}}}

\newcommand{\SPEC}{\ensuremath{K}}
\newcommand{\SPECSQ}{\ensuremath{\SPEC^2}}

\newcommand{\qprobbarn}{\ensuremath{\widebar{\qprob}^\numobs}}

\newcommand{\Hrandvar}{\ensuremath{Z}}
\newcommand{\HrandSpace}{\ensuremath{\mathcal{Z}}}
\newcommand{\hvalue}{\ensuremath{z}}

\newcommand{\qprobone}{\ensuremath{\qprob_1}}
\newcommand{\qprobtwo}{\ensuremath{\qprob_2}}

\newcommand{\Jrand}{\ensuremath{\Jrandpl_\delta}}
\newcommand{\Jrandpl}{\ensuremath{J}}

\newcommand{\MinFun}{\ensuremath{\Phi}}
\newcommand{\MYEXP}[1]{\ensuremath{\exp \big({#1} \big)}}
\newcommand{\MYEXPUP}[1]{\ensuremath{e^{#1}}}

\newcommand{\Emask}{\ensuremath{E}}

\newcommand{\GenSub}{\ensuremath{\mathbb{S}}}

\newcommand{\GamBar}{\ensuremath{\bar{\Gamma}}}

\newcommand{\vect}{\ensuremath{\mbox{vec}}}

\newcommand{\MYMCON}{\ensuremath{\frac{\NewMcon}{2}}}

\newcommand{\NewMconPrime}{\ensuremath{\widebar{\NewMcon}}}
\newcommand{\NewMconPrimeSmall}{\ensuremath{\bar{\NewMcon}}}

\newcommand{\ThetaBad}{\ensuremath{\ThetaBf^{\tiny{\mbox{bad}}}}}

\newcommand{\PertGood}{\ensuremath{\PertMat_{\mbox{\tiny{good}}}}}
\newcommand{\PertBad}{\ensuremath{\PertMat_{\mbox{\tiny{bad}}}}}
\newcommand{\pertgood}{\ensuremath{\perturb_{\mbox{\tiny{good}}}}}
\newcommand{\pertbad}{\ensuremath{\perturb_{\mbox{\tiny{bad}}}}}
\newcommand{\TELE}{\ensuremath{\PLAINTELE(\CovMat)}}
\newcommand{\TELESQRT}{\ensuremath{\PLAINTELESQRT(\CovMat)}}
\newcommand{\PLAINTELE}{\ensuremath{\rho^2}}
\newcommand{\PLAINTELESQRT}{\ensuremath{\rho}}

\newcommand{\SPLINONE}{(G1)} 
\newcommand{\SPLINONEPRIME}{(G1)$'$} 
\newcommand{\SPLINTWO}{(G2)} 


\newcommand{\stepsize}{\ensuremath{\alpha}}
\newcommand{\RegPlain}{\ensuremath{\Phi}}

\newcommand{\Vset}{\ensuremath{\mathcal{V}}}

%\newcommand{\Usub}{\ensuremath{\mathcal{U}}}
%\newcommand{\Vsub}{\ensuremath{\mathcal{V}}}
\newcommand{\Usub}{\ensuremath{\mathbb{U}}}
\newcommand{\Vsub}{\ensuremath{\mathbb{V}}}


\newcommand{\colsp}{\ensuremath{\colspan}}
\newcommand{\rowsp}{\ensuremath{\rowspan}}


\newcommand{\colspan}{\ensuremath{\mbox{colspan}}}
\newcommand{\rowspan}{\ensuremath{\mbox{rowspan}}}

\newcommand{\tasknum}{\ensuremath{T}}
\newcommand{\numtask}{\ensuremath{T}}

\newcommand{\bigN}{\ensuremath{N}}

\newcommand{\zhangslop}{\ensuremath{\tau_\numobs}}
\newcommand{\zhangcurve}{\ensuremath{\NewMcon}}
\newcommand{\zhangrad}{\ensuremath{R}}


\newcommand{\subgauss}{\ensuremath{\sigma}}

\newcommand{\SUPERCONEPLAIN}{\ensuremath{\ConeSet(\ModelSet,
\ModelSetPerp)}}

\newcommand{\SUPERCONE}{\ensuremath{\ConeSet_{\tparam}(\ModelSet,
\BsetPerp)}}

% Expected value of dual norm (in ChapterDecomposable)
\newcommand{\CUPPA}{\ensuremath{c_\numobs(\Regdplain)}}

% Annoying hacking commands
\newcommand{\SERENA}{\ensuremath{\theta^*_{\ModelSetPerp}}}
\newcommand{\SERENAMODEL}{\ensuremath{\theta^*_{\ModelSet}}}

% Generic subspace
\newcommand{\SubSpace}{\ensuremath{{\mathbb{S}}}}
\newcommand{\NewSubSpace}{\ensuremath{{\mathbb{V}}}}

% Length of a time series
\newcommand{\Tlength}{\ensuremath{N}}

\newcommand{\Avar}{\ensuremath{A}}
\newcommand{\Zvar}{\ensuremath{Z}}
\newcommand{\zvar}{\ensuremath{z}}

\newcommand{\xbar}{\ensuremath{\widebar{x}}}

\newcommand{\GenErr}[1]{\ensuremath{\| #1\|}}
\newcommand{\GenErrSq}[1]{\ensuremath{\| #1\|^2}}



\newcommand{\Cset}{\ensuremath{\mathbb{C}}}

%\newcommand{\gmax}{\ensuremath{g_{\mbox{\tiny{max}}}}}
\newcommand{\gmax}{\ensuremath{m}}

\newcommand{\group}{\ensuremath{g}}
\newcommand{\hgroup}{\ensuremath{h}}
\newcommand{\Group}{\ensuremath{\mathcal{G}}}
\newcommand{\groupnum}{\ensuremath{T}}
\newcommand{\Sgroup}{\ensuremath{\mathcal{S}}}
\newcommand{\SgroupBar}{\ensuremath{\Sgroup^c}}
\newcommand{\BigSgroupBar}{\ensuremath{\BigSgroup^c}}
\newcommand{\SgroupTil}{\ensuremath{\widetilde{\Sgroup}}}


\newcommand{\pval}{\ensuremath{p}}
\newcommand{\qval}{\ensuremath{q}}

\newcommand{\LinkFun}{\ensuremath{\psi}}
\newcommand{\LinkFunTwo}{\ensuremath{\LinkFun''}}

\newcommand{\betahatlam}{\ensuremath{\widehat{\betapar}_{\regpar}}}





\newcommand{\HACKER}{\ensuremath{9 \, \LipCon}}
\newcommand{\trad}{\ensuremath{r}}
\newcommand{\AVAR}{\ensuremath{A}}
\newcommand{\BVAR}{\ensuremath{B}}
\newcommand{\CVAR}{\ensuremath{C}}



\newcommand{\BigProjModel}[1]{\ensuremath{\Pi_{\ModelSet}(#1)}}
\newcommand{\BigProjModelPerp}[1]{\ensuremath{\Pi_{\ModelSet^\perp}(#1)}}
\newcommand{\BigProjBset}[1]{\ensuremath{\Pi_{\BsetSmall}(#1)}}
\newcommand{\BigProjBsetPerp}[1]{\ensuremath{\Pi_{\BsetSmallPerp}(#1)}}

\newcommand{\ProjModel}[1]{#1_{\ModelSet}}
\newcommand{\ProjModelPerp}[1]{#1_{\ModelSet^\perp}}
\newcommand{\ProjBset}[1]{#1_{\BsetSmall}}
\newcommand{\ProjBsetPerp}[1]{#1_{\BsetSmall^\perp}}

\newcommand{\betapar}{\ensuremath{\theta}}


\newcommand{\BigReg}[1]{\ensuremath{\Regplain \big(#1 \big)}}

\newcommand{\RSC}{\ensuremath{\operatorname{RSC}}}

\newcommand{\pdima}{\ensuremath{{\pdim_1}}}
\newcommand{\pdimb}{\ensuremath{{\pdim_2}}}
\newcommand{\Apperr}{\ensuremath{\mathcal{E}_{\operatorname{app}}}}
\newcommand{\Esterr}{\ensuremath{\mathcal{E}_{\operatorname{err}}}}
\newcommand{\Nullerr}{\ensuremath{\mathcal{E}_{\operatorname{null}}}}
\newcommand{\SuperConvSet}{\ensuremath{\ConvSet(\ModelSet, \Bset;
    \thetastar)}}
\newcommand{\SuperKeySet}{\ensuremath{\KeySet(\ErrRad; \ModelSet,
    \Bset, \thetastar)}}

\newcommand{\SuperRSC}{\ensuremath{ \RSC(\epsilon, \NewMcon;
    \ModelSet, \BsetPerp)}}

\newcommand{\Stau}{\ensuremath{\Sset_\taupar}}

\newcommand{\Gfun}{\ensuremath{\mathcal{F}}}

\newcommand{\TmpVarA}{\ensuremath{\alpha}}
\newcommand{\TmpVarB}{\ensuremath{\beta}}

%\newcommand{\Regplain}{\ensuremath{\mathcal{R}}}

\newcommand{\Regplain}{\ensuremath{\Phi}}

\newcommand{\Regd}[1]{\ensuremath{\Regplain^*(#1)}}
\newcommand{\Regdplain}{\ensuremath{\Regplain^*}}

\newcommand{\Reg}[1]{\ensuremath{\Regplain(#1)}}
\newcommand{\RegSq}[1]{\ensuremath{\Regplain^2(#1)}}


\newcommand{\ModelSet}{\ensuremath{\mathbb{M}}}
\newcommand{\ModelSetPerp}{\ensuremath{\ModelSet^\perp}}

\newcommand{\Bset}{\widebar{\ModelSet}}
\newcommand{\BsetSmall}{\bar{\ModelSet}}
\newcommand{\BsetPerp}{\Bset^\perp}
\newcommand{\BsetSmallPerp}{\BsetSmall^\perp}



\newcommand{\ConvSet}{\ensuremath{\mathbb{C}}}
\newcommand{\KeySet}{\mathbb{K}}



\newcommand{\delpar}{\ensuremath{\Delta}}
\newcommand{\delparhat}{\ensuremath{\widehat{\delpar}}}

\newcommand{\Uhat}{\ensuremath{\widehat{U}}}
\newcommand{\Vhat}{\ensuremath{\widehat{V}}}

\newcommand{\TINYO}{{\ensuremath{\mbox{\scriptsize{O}}}}}
\newcommand{\TINYOO}{{\ensuremath{\mbox{\scriptsize{OO}}}}}
\newcommand{\TINYH}{{\ensuremath{\mbox{\scriptsize{H}}}}}
\newcommand{\TINYHH}{{\ensuremath{\mbox{\scriptsize{HH}}}}}



%\newcommand{\LowRank}{\ensuremath{L}}

\newcommand{\LowRankHat}{\ensuremath{\widehat{\LowRank}}}
\newcommand{\SparseHat}{\ensuremath{\widehat{\Sparse}}}
\newcommand{\regparone}{\ensuremath{\regparn}}
\newcommand{\regpartwo}{\ensuremath{\mu_\numobs}}


\newcommand{\rdim}{\ensuremath{r}}

\newcommand{\astar}{\ensuremath{a^*}}

\newcommand{\Wstil}{\ensuremath{\tilde{\Wmat}}}

\newcommand{\CovBound}{\ensuremath{b}}
\newcommand{\RON}{\ensuremath{7}}

\newcommand{\ahat}{\ensuremath{\widehat{a}}}


\newcommand{\sminus}{\ensuremath{s^{\scriptsize{-}}}}
\newcommand{\sback}{\ensuremath{\backslash \{\ej\}}}

\newcommand{\ntheta}[1]{\ensuremath{\theta^{#1}}}
\newcommand{\xnot}[1]{\ensuremath{x_{\backslash \{#1\}}}}
\newcommand{\Xnot}[1]{\ensuremath{\Xmat_{\backslash \{#1\}}}}
\newcommand{\XnotPlain}[1]{\ensuremath{X_{\backslash \{#1\}}}}
\newcommand{\XnotData}[2]{\ensuremath{\Xmat_{#1 \backslash \{#2\}}}}
\newcommand{\xnotdata}[2]{\ensuremath{x_{#1 \backslash \{#2\}}}}
\newcommand{\Znot}[1]{\ensuremath{Z_{\backslash \{#1\}}}}
\newcommand{\ZnotSmall}[1]{\ensuremath{z_{\backslash \{#1\}}}}

\newcommand{\Wme}[1]{\ensuremath{W_{#1}}}


\newcommand{\nthetas}[2]{\ensuremath{\theta^{#1}_{#2}}}
\newcommand{\Xnots}[2]{\ensuremath{X_{#2; \backslash \{#1\}}}}
\newcommand{\Wnots}[2]{\ensuremath{W_{#2; \backslash \{#1\}}}}

\newcommand{\vinda}{\ensuremath{s}}


%\newcommand{\degmax}{\ensuremath{\rho}}
%\newcommand{\degmax}{\ensuremath{D}}
%\newcommand{\degmax}{\ensuremath{k}}
\newcommand{\degmax}{\ensuremath{m}}

\newcommand{\PHIQ}{\ensuremath{\varphi(\qprob, \sigma_w)}}

\newcommand{\GamStar}{\ensuremath{\GammaBf^*}}

%\newcommand{\OffNorm}[1]{\ensuremath{\| #1 \|_{\mbox{\tiny{1,off}}}}}
%\newcommand{\OffNormMax}[1]{\ensuremath{\| #1 \|_{\mbox{\tiny{max,off}}}}}

\newcommand{\OffNormMax}[1]{\ensuremath{\matsnorm{#1}{\mbox{\tiny{max,off}}}}}
\newcommand{\OffNorm}[1]{\ensuremath{\matsnorm{#1}{\mbox{\tiny{1,off}}}}}


\newcommand{\neigh}{\ensuremath{\mathcal{N}}}
\newcommand{\neighplus}{\ensuremath{\neigh^+}}
\newcommand{\neighhat}{\ensuremath{\widehat{\neigh}}}

% Notation for an image vector (compressed sensing)
\newcommand{\image}{\ensuremath{\beta}}


\newcommand{\LogLike}{\ensuremath{\ell}}

%\newcommand{\Data}{\ensuremath{X_1^\numobs}}

\newcommand{\expcompat}{\ensuremath{\psi}}

\newcommand{\ENCMIN}[1]{\ensuremath{\Big \{ #1 \Big \}}}

\newcommand{\Xop}{\ensuremath{\mathfrak{X}_\numobs}}

\newcommand{\Sparse}{\ensuremath{\GammaBf}}
\newcommand{\PlainSparse}{\ensuremath{\Gamma}}
\newcommand{\SparsePlain}{\ensuremath{\Gamma}}
\newcommand{\LowRank}{\ensuremath{\LambdaBf}}
\newcommand{\PlainLowRank}{\ensuremath{\Lambda}}
\newcommand{\TrueSparse}{\ensuremath{\Sparse^*}}
\newcommand{\TrueLowRank}{\ensuremath{\LowRank^*}}

\newcommand{\PlainTrueSparse}{\ensuremath{\PlainSparse^*}}
\newcommand{\PlainTrueLowRank}{\ensuremath{\PlainLowRank^*}}
\newcommand{\PlainSparseHat}{\ensuremath{\widehat{\PlainSparse}}}
\newcommand{\PlainLowRankHat}{\ensuremath{\widehat{\PlainLowRank}}}


\newcommand{\CliqueSet}{\ensuremath{\mathfrak{C}}}

\newcommand{\condind}{\ensuremath{\perp\!\!\!\perp}}

\newcommand{\Plaincon}{\ensuremath{C}}

\newcommand{\blinvec}{\ensuremath{\beta}}
\newcommand{\Fsparse}{\Fclass_{\mbox{\tiny{spar}}}}

\newcommand{\PolyClass}{\ensuremath{\mathcal{P}}}

\newcommand{\phitil}{\ensuremath{\widetilde{\phi}}}

\newcommand{\FclassT}[1]{\ensuremath{\Fclass_{\mbox{\tiny{ortho}}}(#1;
T)}}

\newcommand{\IID}{i.i.d.~}
\newcommand{\IIDNOSPACE}{i.i.d.}
\newcommand{\ER}{Erd\"{o}s-R\'{e}nyi}

\newcommand{\Fconv}{\ensuremath{\Fclass_{\tiny{\mbox{conv}}}}}
\newcommand{\boutil}{\ensuremath{\tilde{\bou}}}

%\newcommand{\LOW}{\ensuremath{\eta}}
\newcommand{\LOW}{\ensuremath{\nu}}

\newcommand{\ChelHat}{\ensuremath{\widehat{Z}_\numobs}}
\newcommand{\Chel}{\ensuremath{\widebar{Z}_\numobs}}


\newcommand{\SAM}[2]{\ensuremath{\mathcal{C}({#1},{#2})}}
\newcommand{\LipCon}{\ensuremath{L}}




%\newcommand{\MYLOSS}[1]{\ensuremath{\Loss_{#1}}}
\newcommand{\HACKLOSS}[1]{\ensuremath{\LossSing_{#1}}}
\newcommand{\QUADFUN}{\ensuremath{\mathcal{Q}}}

%\newcommand{\Curv}{\ensuremath{C}}
\newcommand{\Curv}{\ensuremath{\gamma}}

\newcommand{\DELTA}[1]{\ensuremath{\HACKLOSS{#1} - \HACKLOSS{\fstar}}} 


\newcommand{\TINYLIP}{\ensuremath{\scriptsize{\mbox{Lip}}}} 
\newcommand{\TINYAND}{\ensuremath{\scriptsize{\mbox{AND}}}} 
\newcommand{\TINYOR}{\ensuremath{\scriptsize{\mbox{OR}}}} 


\newcommand{\LocRadPop}{\ensuremath{\widebar{\mathcal{R}}_\numobs}}
\newcommand{\LocRadPopSmall}{\ensuremath{\bar{\mathcal{R}}_\numobs}}

\newcommand{\Aevent}{\ensuremath{\mathcal{A}}}

\newcommand{\Bevent}{\ensuremath{\mathcal{B}}}

\newcommand{\FUNNORM}[2]{\ensuremath{\matsnorm{#1}{#2}}}

\newcommand{\Xhack}[1]{\ensuremath{X^{#1}}}
\newcommand{\xhack}[1]{\ensuremath{x^{#1}}}

\newcommand{\Yhack}[1]{\ensuremath{Y^{#1}}}
\newcommand{\yhack}[1]{\ensuremath{y^{#1}}}

\newcommand{\Zhack}[1]{\ensuremath{Z^{#1}}}
\newcommand{\zhack}[1]{\ensuremath{z^{#1}}}

\newcommand{\SpecConeSub}[2]{\ensuremath{\ConeSub_{#2}(#1)}}

\newcommand{\Can}[1]{\ensuremath{\Delta^{#1}}}

\newcommand{\cprob}{\ensuremath{\mathbb{M}}}
\newcommand{\cdens}{\ensuremath{m}}

\newcommand{\LAUR}{\ensuremath{c}}

\newcommand{\LaurentBset}{\ensuremath{\mathcal{B}}}

\newcommand{\SigTil}{\ensuremath{\widetilde{\CovMat}}}

\newcommand{\xannoy}[1]{\ensuremath{x_{#1}}}
\newcommand{\yannoy}[1]{\ensuremath{y_{#1}}}
\newcommand{\Xannoy}[1]{\ensuremath{X_{#1}}}
\newcommand{\Yannoy}[1]{\ensuremath{Y_{#1}}}

%\newcommand{\Shannon}{\ensuremath{\mathbb{S}}}
\newcommand{\Shannon}{\ensuremath{H}}

\newcommand{\PSIFUN}{\ensuremath{\psi}}


\newcommand{\realplus}{\ensuremath{\real_+}}


\newcommand{\GoodEnt}{\ensuremath{\mathbb{H}}}
\newcommand{\ELAMX}{\ensuremath{e^{\lambda X}}}
\newcommand{\MOM}{\ensuremath{\varphi}}
\newcommand{\CUM}{\ensuremath{\Phi}}
\newcommand{\MOMX}{\ensuremath{\varphi_{\mathrm{x}}}}
\newcommand{\MOMXTIL}{\ensuremath{\varphi_{\mathrm{\tilde{x}}}}}

\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}

\newcommand{\PhiMap}{\ensuremath{\Phi}}
\newcommand{\kereig}{\ensuremath{\mu}}
\newcommand{\kereighat}{\ensuremath{\widehat{\kereig}}}

\newcommand{\LINSP}{\ensuremath{\widetilde{{\mathbb{H}}}}}
\newcommand{\plainin}[2]{\ensuremath{\inprod{#1}{#2}_{\LINSP}}}


\newcommand{\Null}{\ensuremath{\mathbb{N}}}

\newcommand{\Lin}{\ensuremath{L}}
\newcommand{\smoothpar}{\ensuremath{\alpha}}

\newcommand{\xtil}{\ensuremath{\widetilde{x}}}

\newcommand{\pdeg}{\ensuremath{\polydeg}}

\newcommand{\HilRad}{\ensuremath{R}}

\newcommand{\linvec}{\ensuremath{\theta}}
\newcommand{\linvecstar}{\ensuremath{\linvec^*}}
\newcommand{\linvechat}{\ensuremath{\widehat{\linvec}}}



\newcommand{\LinSpace}{\ensuremath{\mathbb{L}}}
\newcommand{\Cost}{\ensuremath{\mathcal{C}}}

\newcommand{\MyCost}{\ensuremath{\mathcal{C}}}



\newcommand{\PsiMat}{\ensuremath{\mathbf{\Psi}}}

\newcommand{\PertMat}{\ensuremath{\mathbf{\Delta}}}
\newcommand{\pertmat}{\ensuremath{p}}
\newcommand{\PertMatTil}{\ensuremath{\widetilde{\PertMat}}}
\newcommand{\pertmattil}{\ensuremath{\tilde{\pertmat}}}
\newcommand{\thetahatsm}{\ensuremath{\hat{\theta}}}
\newcommand{\wbar}{\ensuremath{\bar{w}}}
\newcommand{\HACKC}{\ensuremath{r}}
%\newcommand{\MatUp}{\ensuremath{\widehat{\Gamma}}}
\newcommand{\MatUp}{\ensuremath{\SamCovPert_3}}
\newcommand{\tailpar}{\ensuremath{\delta}}
\newcommand{\etain}{\ensuremath{\varrho}}
\newcommand{\orthvec}{\ensuremath{\xi}}
\newcommand{\PLAINCON}{\ensuremath{C}}
\newcommand{\HACKREG}{\ensuremath{\Phi_{\tiny{\regparn}}}}
\newcommand{\SamTil}{\ensuremath{\widetilde{\Sigma}}}
\newcommand{\ShanghaiPsi}{\ensuremath{\Psi}}
\newcommand{\clam}{\ensuremath{\plaincon_\regpar}}
\newcommand{\regparnsq}{\ensuremath{\regpar^2_\numobs}}
\newcommand{\NOISEFUN}{\ensuremath{\varphi_\eigengap}}
\newcommand{\NOISEFUNTWO}{\ensuremath{\psi_\eigengap}}

\newcommand{\rscslop}{\tau^2_\numobs}
\newcommand{\rscslopsq}{\tau^2_\numobs}

\def\loss{\Loss} 
\def\gradloss{\nabla \loss} 
\def\tparam{\theta^{*}}



\newcommand{\ConeSet}{\ensuremath{\mathbb{C}}}
\newcommand{\twoafun}{\ensuremath{\ddot{A}}}


\newcommand{\xitil}{\ensuremath{\tilde{\xi}}}
\newcommand{\Xitil}{\ensuremath{\widetilde{\Xi}}}


\newcommand{\Vtil}{\ensuremath{\widetilde{V}}}

\newcommand{\Dhat}{\ensuremath{\widehat{D}}}
\newcommand{\DmatHat}{\ensuremath{\widehat{\Dmat}}}

\newcommand{\BauxEvent}{\ensuremath{\mathcal{B}}}

\newcommand{\GammaBf}{\ensuremath{\mathbf{\Gamma}}}
\newcommand{\PhiBf}{\ensuremath{\mathbf{\Phi}}}
\newcommand{\LambdaBf}{\ensuremath{\mathbf{\Lambda}}}
\newcommand{\SigmaBf}{\ensuremath{\mathbf{\Sigma}}}

\newcommand{\ThetaStar}{\ensuremath{\ThetaBf^*}}
\newcommand{\ThetaStarPlain}{\ensuremath{\Theta^*}}
\newcommand{\ThetaHat}{\ensuremath{\widehat{\ThetaBf}}}
\newcommand{\ThetaHatPlain}{\ensuremath{\widehat{\Theta}}}
\newcommand{\ThetaTil}{\ensuremath{\widetilde{\ThetaBf}}}
\newcommand{\PlainThetaTil}{\ensuremath{\widetilde{\Theta}}}
\newcommand{\PlainThetaHat}{\ensuremath{\widehat{\Theta}}}

\newcommand{\SigHat}{\ensuremath{\widehat{\CovMat}}}


\newcommand{\Fnorm}[1]{\ensuremath{\|#1\|_{\Fclass}}}
\newcommand{\regparn}{\ensuremath{{\regpar_{\numobs}}}}
\newcommand{\regparnhalf}{\ensuremath{\frac{\regparn}{2}}}

\newcommand{\JointCost}{\ensuremath{\phi}}
\newcommand{\DelTil}{\ensuremath{\widetilde{\Delta}}}
\newcommand{\DelStar}{\ensuremath{\Delta^*}}

\newcommand{\delhat}{\estim{\delpar}}


% General noise for non-parametric regression
\newcommand{\gennoise}[1]{\ensuremath{\varepsilon_{#1}}}

\newcommand{\DelHat}{\ensuremath{\widehat{\Delta}}}
\newcommand{\hilnorm}[1]{\ensuremath{\|#1\|_{\Hil}}}
\newcommand{\hilin}[2]{\ensuremath{\inprod{#1}{#2}_{\Hil}}}


\newcommand{\HilSub}{\ensuremath{\mathbb{J}}}
\newcommand{\ghat}{\ensuremath{\widehat{g}}}

% Rescaled kernel function
\newcommand{\Kernew}{\ensuremath{K}}
\newcommand{\CritFun}{\ensuremath{F}}




\newcommand{\Pclass}{\ensuremath{\mathcal{P}}}
\newcommand{\Pzero}{\ensuremath{\Pclass_0}}
\newcommand{\Pone}{\ensuremath{\Pclass_1}}
\newcommand{\mprobone}{\ensuremath{\mprob_1}}
\newcommand{\mprobzero}{\ensuremath{\mprob_0}}

\newcommand{\mprobn}{\ensuremath{\mprob^{1:\numobs}}}
\newcommand{\qprobn}{\ensuremath{\qprob^{1:\numobs}}}
\newcommand{\uprobn}{\ensuremath{\uprob^{1:\numobs}}}



\newcommand{\Fdiv}[2]{\ensuremath{D_f(#1 \, \| \, #2)}}
\newcommand{\Vdist}[2]{\ensuremath{V(#1 \, \| \, #2)}}
\newcommand{\Hell}[2]{\ensuremath{H(#1 \, \| \, #2)}}
\newcommand{\HellSq}[2]{\ensuremath{H^2(#1 \, \| \, #2)}}
\newcommand{\BigHellSq}[2]{\ensuremath{H^2 \Big(#1 \, \| \, #2 \Big)}}
\newcommand{\ChiSq}[2]{\ensuremath{\chi^2(#1 \, \| \, #2)}}

\newcommand{\conv}{\ensuremath{\operatorname{conv}}}

\newcommand{\Mpack}{\ensuremath{M}}
\newcommand{\MpackPlain}{\ensuremath{M}}
\newcommand{\MpackDelta}{\ensuremath{\Mpack(2 \delta)}}

\newcommand{\perr}{\ensuremath{q_e}}
\newcommand{\psistar}{\ensuremath{\psi^*}}

\newcommand{\Aclass}{\ensuremath{\mathcal{A}}}
\newcommand{\Bclass}{\ensuremath{\mathcal{B}}}
\newcommand{\uprob}{\ensuremath{\mathbb{U}}}



\newcommand{\smooth}{\ensuremath{\alpha}}

\newcommand{\sparsedim}{\ensuremath{s}}

\newcommand{\gamlow}{\ensuremath{\eta_{\ell}}}
\newcommand{\gamup}{\ensuremath{\eta_{u}}}
\newcommand{\gammin}{\ensuremath{\eta_{\mbox{\scriptsize{min}}}}}
\newcommand{\gammax}{\ensuremath{\eta_{\mbox{\scriptsize{max}}}}}

\newcommand{\gamminsq}{\ensuremath{\eta^2_{\mbox{\scriptsize{min}}}}}
\newcommand{\gammaxsq}{\ensuremath{\eta^2_{\mbox{\scriptsize{max}}}}}



\newcommand{\introthresh}{\ensuremath{t}} 


\newcommand{\Uni}{\ensuremath{\operatorname{Uni}}}

\newcommand{\none}{\ensuremath{{\numobs_{1}}}}
\newcommand{\ntwo}{\ensuremath{{\numobs_{2}}}}

\newcommand{\XsamOne}{\ensuremath{\{X_i\}_{i=1}^\none}}
\newcommand{\XsamTwo}{\ensuremath{\{X'_i\}_{i=1}^\ntwo}}

\newcommand{\XbigFullSam}{\ensuremath{{\{X_i\}_{i=1}^{\none + \ntwo}}}}

% Discriminant function
\newcommand{\DiscFun}{\ensuremath{\Psi}}
\newcommand{\DiscFunHat}{\ensuremath{\widehat{\DiscFun}}}
\newcommand{\DiscFunTil}{\ensuremath{\widetilde{\DiscFun}}}
\newcommand{\DiscFunHatSimple}{\ensuremath{\DiscFunHat_{\mbox{\tiny{id}}}}}

%\newcommand{\err}{\ensuremath{\epsilon}}
\newcommand{\err}{\ensuremath{\mbox{Err}}}



% Marcenko-Pastur law
\newcommand{\FMP}{\ensuremath{f_{\operatorname{MP}}}}

% Upper and lower limits in Marceko-Pastur law
\newcommand{\tmin}{\ensuremath{t_{\small{\operatorname{min}}}}}
\newcommand{\tmax}{\ensuremath{t_{\small{\operatorname{max}}}}}




\newcommand{\MatCumFunc}[1]{\ensuremath{\Phi_{#1}}}
\newcommand{\MatCumFun}{\MatCumFunc{\Qmat}}

\newcommand{\MatMomFunc}[1]{\ensuremath{\Psi_{#1}}}
\newcommand{\MatMomFun}{\MatMomFunc{\Qmat}}


\newcommand{\bernbou}{\ensuremath{b}}

\newcommand{\sigtil}{\ensuremath{\tilde{\sigma}}}
\newcommand{\ThreshOp}[1]{\ensuremath{T_{#1}}}



\newcommand{\Vprime}{\ensuremath{\Vset'}}
\newcommand{\Rcrow}{\ensuremath{R}}



\newcommand{\ksubgauss}{\ensuremath{\sigma}}

\newcommand{\SpecSet}{\ensuremath{\mathbb{K}}}

\newcommand{\SpecSetCov}{\ensuremath{\Sphere{\usedim}(\CovMat^{-1})}}
\newcommand{\CovMatSqrtInv}{\ensuremath{\CovMat^{-\frac{1}{2}}}}
\newcommand{\util}{\ensuremath{\widetilde{u}}}
\newcommand{\uprime}{\ensuremath{u'}}
\newcommand{\vprime}{\ensuremath{v'}}
%\newcommand{\frob}[1]{\ensuremath{\matsnorm{#1}{F}}}
\newcommand{\frob}[1]{\frobnorm{#1}}

\newcommand{\ParSpace}{\ensuremath{\Omega}}
\newcommand{\ParSet}{\ensuremath{\ParSpace}}
\newcommand{\MiniMax}{\ensuremath{\mathfrak{M}}}
\newcommand{\HackMiniMax}{\ensuremath{\MiniMax(\theta(\Pclass),
\MinFun \circ \rhomet)}}

\newcommand{\deltil}{\ensuremath{\widetilde{\delta}}}

%\newcommand{\thetastar}{\ensuremath{\theta^*}}
\newcommand{\Zhat}{\ensuremath{\widehat{Z}}}
\newcommand{\zhat}{\ensuremath{\widehat{z}}}
\newcommand{\Ztil}{\ensuremath{\widetilde{Z}}}
\newcommand{\ztil}{\ensuremath{\widetilde{z}}}


\newcommand{\deln}{\ensuremath{\delta^*}}
\newcommand{\Pbar}{\ensuremath{\widebar{\mathbb{P}}}}
\newcommand{\nullsp}{\ensuremath{\operatorname{null}}}
\newcommand{\Nkull}{\ensuremath{N_{\tiny{\mbox{KL}}}}}

\newcommand{\TermOne}{\ensuremath{\Term_1}}
\newcommand{\TermTwo}{\ensuremath{\Term_2}}
\newcommand{\TermThree}{\ensuremath{\Term_3}}

\newcommand{\NSUM}{\ensuremath{\frac{1}{\numobs} \sum_{i=1}^\numobs}}

\newcommand{\ConeSub}{\ensuremath{\mathbb{C}}}

\newcommand{\perturb}{\ensuremath{\Delta}}
\newcommand{\perturbhat}{\ensuremath{\widehat{\perturb}}}
\newcommand{\Perturb}{\ensuremath{\PertMat}}
\newcommand{\PerturbHat}{\ensuremath{\widehat{\PertMat}}}
\newcommand{\PertHat}{\ensuremath{\widehat{\PertMat}}}
\newcommand{\PertHatPlain}{\ensuremath{\widehat{\Delta}}}

\newcommand{\strongcon}{\ensuremath{\gamma}}
\newcommand{\genparam}{\ensuremath{\theta}}
\newcommand{\genparamstar}{\ensuremath{\genparam^*}}
\newcommand{\genparamhat}{\ensuremath{\widehat{\genparam}}}
\newcommand{\conecon}{\ensuremath{\alpha}}
\newcommand{\ellonerad}{\ensuremath{R_1}}
\newcommand{\nullspace}{\ensuremath{\operatorname{null}}}

\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}


\newcommand{\mupar}{\ensuremath{\mu}}
\newcommand{\jones}{1\!\!1}

\newcommand{\thetastar}{\ensuremath{{\theta^*}}}

\newcommand{\ytil}{\ensuremath{\widetilde{y}}}

\newcommand{\sign}{\ensuremath{\operatorname{sign}}}

\newcommand{\rhopar}{\ensuremath{\rho}}


\newcommand{\mutinco}{\ensuremath{\alpha}}
\newcommand{\cmin}{\ensuremath{c_{\operatorname{min}}}}
\newcommand{\colnorm}{\ensuremath{C}}
%\newcommand{\sign}{\ensuremath{\operatorname{sign}}}
\newcommand{\estim}[1]{\ensuremath{\widehat{#1}}}
%\newcommand{\alhat}{\ensuremath{\widehat{\alpha}}}
%\newcommand{\HyperCube}{\ensuremath{\mathbb{H}}}
\newcommand{\Shat}{\ensuremath{\widehat{S}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\RmaxShort}{\ensuremath{\|\mathbb{S}_\numobs\|_{\Fclass}}}
\newcommand{\Rmax}[1]{\ensuremath{\|\mathbb{S}_\numobs\|_{#1}}}



\newcommand{\metric}{\ensuremath{\rho}}
%\newcommand{\MetSpace}{\ensuremath{\mathbb{X}}}
\newcommand{\MetSpace}{\ensuremath{\Xspace}}

\newcommand{\concfunpl}{\ensuremath{{\large{\alpha}}}}
\newcommand{\concfunal}{\ensuremath{\concfunpl_{\: \mprob}}}
\newcommand{\concfun}{\ensuremath{\concfunpl_{\: {\tiny{\mprob, (\MetSpace, \metric)}}}}}
\newcommand{\Enlarge}[2]{\ensuremath{#1^{#2}}}
\newcommand{\PlSet}{\ensuremath{A}}
\newcommand{\phifun}{\ensuremath{\phi}}
\newcommand{\Entpl}{\ensuremath{\Psi}}
\newcommand{\Ent}[1]{\ensuremath{\Entpl_{#1}}}
\newcommand{\MGF}{\ensuremath{\varphi}} 
\newcommand{\xback}[1]{\ensuremath{x_{\backslash #1}}}
\newcommand{\MyXback}[1]{\ensuremath{X_{\backslash #1}}}
\newcommand{\sobfun}{\ensuremath{g}}

\newcommand{\Hemi}[1]{\ensuremath{H_{#1}}}

\newcommand{\tvnorm}[1]{\ensuremath{\| #1\|_{\mbox{\tiny{TV}}}}}

\newcommand{\rprob}{\ensuremath{\mathbb{R}}}

\newcommand{\wass}[2]{\ensuremath{W_{\metric}(#1, \, #2)}}
\newcommand{\wasstwo}[2]{\ensuremath{W_2(#1, \, #2)}}
\newcommand{\wasshamm}[2]{\ensuremath{W_{\scriptsize{\mbox{Ham}}}(#1, \, #2)}}

\newcommand{\transcost}{\ensuremath{\gamma}}

\newcommand{\SPOT}{\ensuremath{\psi}}

\newcommand{\Htil}{\ensuremath{\widetilde{H}}}

\newcommand{\TayError}{\ensuremath{E}}
\newcommand{\InfConv}{\ensuremath{T}}
\newcommand{\Ltil}{\ensuremath{\widetilde{L}}}
\newcommand{\plwass}{\ensuremath{W_1}}

\newcommand{\Fmax}[1]{\ensuremath{\| #1\|_{\Fclass}}}
\newcommand{\Gmax}[1]{\ensuremath{\| #1\|_{\Gclass}}}
\newcommand{\FmaxShort}{\ensuremath{\Fmax{\EmpDist - \Prob}}}
\newcommand{\GmaxShort}{\ensuremath{\Gmax{\EmpDist - \Prob}}}
\newcommand{\FmaxTwo}[2]{\ensuremath{\| #1\|_{#2}}}

\newcommand{\EmpDist}{\ensuremath{\mprob_\numobs}}

\newcommand{\pProb}{\ensuremath{P}}
\newcommand{\pEmpDist}{\ensuremath{\pProb_\numobs}}

\newcommand{\LossClass}{\ensuremath{\mathfrak{L}}}
\newcommand{\littleloss}{\ensuremath{\mathcal{L}}}
\newcommand{\Rhat}{\ensuremath{\widehat{\Risk}_\numobs}}
\newcommand{\Risk}{\ensuremath{R}}
\newcommand{\SphereSet}{\ensuremath{\mathcal{S}_{\mbox{\tiny{sphere}}}}}

\newcommand{\HalfInt}{\ensuremath{\SetClass_{\tiny{\mbox{left}}}}}
\newcommand{\FullInt}{\ensuremath{\SetClass_{\tiny{\mbox{two}}}}}
\newcommand{\LinClass}{\ensuremath{\mathscr{L}}}

\newcommand{\Zsam}[1]{\ensuremath{Z_{#1}}}
\newcommand{\pdens}{\ensuremath{p}}
\newcommand{\qdens}{\ensuremath{q}}
\newcommand{\udens}{\ensuremath{u}}

\newcommand{\thetaprime}{\ensuremath{\theta_{0}}}
\newcommand{\decrule}{\ensuremath{f}}
\newcommand{\dechat}{\ensuremath{\widehat{\decrule}}}
\newcommand{\decstar}{\ensuremath{\decrule^*}}
\newcommand{\MySet}{\ensuremath{\mathbb{S}}}



\newcommand{\OmegaPrime}{\ensuremath{\Omega_0}}

%\newcommand{\thetastar}{{\ensuremath{\theta^{*}}}}
%\newcommand{\thetatil}{{\ensuremath{\widetilde{\theta}}}}

\newcommand{\AsetRad}{\ensuremath{\mathcal{A}}}


\newcommand{\superrade}[1]{\ensuremath{\rade{1}^{#1}}}
\newcommand{\SAMSUM}{\ensuremath{\sum_{i=1}^\numobs}}
\newcommand{\NORMSAMSUM}{\ensuremath{\frac{1}{\numobs} \SAMSUM}}
\newcommand{\EmpRade}[1]{\ensuremath{\widehat{\mathcal{R}}_\numobs(#1)}}

\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}

\newcommand{\fbar}{\ensuremath{\widebar{f}}}
\newcommand{\fbarunder}{\ensuremath{\bar{f}}}
\newcommand{\myhbar}{\ensuremath{\widebar{h}}}
\newcommand{\myhalf}{\ensuremath{\frac{1}{2}}}

\newcommand{\CovHat}{\ensuremath{\widehat{\CovMat}}}
\newcommand{\cov}{\ensuremath{\operatorname{cov}}}

% Notation for generic (random) matrix
%\newcommand{\Gymat}{\ensuremath{{\mathbf{Y}}}}
\newcommand{\Gymat}{\ensuremath{M}}




\newcommand{\diag}{\ensuremath{\operatorname{diag}}}

\newcommand{\ThetaMLE}{\ensuremath{\widehat{\ThetaBf}_{\tiny{\mbox{MLE}}}}}

\newcommand{\usedima}{\ensuremath{{\usedim_1}}}
\newcommand{\usedimb}{\ensuremath{{\usedim_2}}}

\newcommand{\jdima}{\ensuremath{j_1}}
\newcommand{\jdimb}{\ensuremath{j_2}}


\newcommand{\SymPSD}[1]{\ensuremath{\mathcal{S}^{#1 \times #1}_+}}
\newcommand{\SymMat}[1]{\ensuremath{\mathcal{S}^{#1 \times #1}}}

\newcommand{\mytilde}[1]{\ensuremath{\widetilde{#1}}}

\newcommand{\martbsum}{\ensuremath{b}}
\newcommand{\kind}{\ensuremath{k}}
\newcommand{\iind}{\ensuremath{i}}
\newcommand{\jind}{\ensuremath{j}}

\newcommand{\kerind}{\ensuremath{j}}
\newcommand{\pind}{\ensuremath{m}}

\newcommand{\Xdseq}[2]{\ensuremath{X_{#1}^{#2}}}
\newcommand{\MySeq}[2]{\ensuremath{\{#1_{#2}\}_{#2 = 1}^\infty}}
\newcommand{\MySeqZero}[2]{\ensuremath{\{#1_{#2}\}_{#2 = 0}^\infty}}

\newcommand{\DoubSeq}[3]{\ensuremath{\{(#1_{#3}, #2_{#3})\}_{#3 = 1}^\infty}}
\newcommand{\MyTripSeq}[3]{\ensuremath{#1_{#2}^{#3}}}
\newcommand{\subexpvar}{\ensuremath{\nu}}
\newcommand{\Bou}{\ensuremath{B}}
\newcommand{\bou}{\ensuremath{b}}
\newcommand{\BernPar}{\ensuremath{b}}
\newcommand{\Fil}{\ensuremath{\mathcal{F}}}


\newcommand{\SubexpBou}{\ensuremath{\alpha}}
\newcommand{\SubExpNew}{\SubexpNew}
\newcommand{\SubexpNew}{\ensuremath{\SubexpBou}}
\newcommand{\SubexpMin}{\ensuremath{\SubexpNew_*}}
\newcommand{\SubexpMinWide}{\SubexpMin}
\newcommand{\ZurSub}{\ensuremath{\SubexpBou}}
\newcommand{\ZurSubInv}{\ensuremath{\ZurSub^{-1}}}



%\newcommand{\SubexpMin}{\ensuremath{\bar{\SubexpNew}}}
%\newcommand{\SubexpMinWide}{\ensuremath{\widebar{\SubexpNew}}}


\newcommand{\diam}{\ensuremath{\operatorname{diam}}}

\newcommand{\gausspl}{\ensuremath{z}}
\newcommand{\gauss}[1]{\ensuremath{\gausspl_{#1}}}


\newcommand{\GRAYBOX}[1]{\noindent \begin{graybox} \parbox{#1} \end{graybox}}

\newcommand{\MbernBou}{\ensuremath{b}}
\newcommand{\BernBou}{\ensuremath{M}}
\newcommand{\CumGen}{\ensuremath{\Phi}}

%\newcommand{\sign}{\ensuremath{\operatorname{sign}}}

\newcommand{\Xdomain}{\ensuremath{\mathcal{X}}}

\newcommand{\orpar}{\ensuremath{q}}
\newcommand{\orq}{\ensuremath{\psi_\orpar}}
\newcommand{\ornorm}[1]{\ensuremath{\|#1\|_{\orq}}}
\newcommand{\genpar}{\ensuremath{\theta}}
\newcommand{\genpartwo}{\ensuremath{{\thetatil}}}
\newcommand{\ExsA}{\ensuremath{\Exs_A}}

\newcommand{\CovMatSqrt}{\ensuremath{\sqrt{\CovMat}}}
\newcommand{\vtil}{\ensuremath{\widetilde{v}}}
\newcommand{\plopnorm}[1]{\ensuremath{\matsnorm{#1}{2}}}

\newcommand{\DelMin}{\ensuremath{\Delta_{\operatorname{min}}}}
\newcommand{\DelMax}{\ensuremath{\Delta_{\operatorname{max}}}}
\newcommand{\svmaxbar}{\widebar{\mysingval}_{\operatorname{max}}}
\newcommand{\svminbar}{\widebar{\mysingval}_{\operatorname{min}}}



\newcommand{\iprime}{\ensuremath{{i'}}}
\newcommand{\jprime}{\ensuremath{{j'}}}

\newcommand{\statesp}{\ensuremath{\mathcal{X}}}
\newcommand{\ChainNum}{\ensuremath{L}} 
%\renewcommand{\rhomet}{\ensuremath{d}}
\newcommand{\FunBou}{\ensuremath{B}}
\newcommand{\GenSetTil}{\ensuremath{\widetilde{\GenSet}}}
\newcommand{\SparseSet}{\ensuremath{\mathbb{S}}}
\newcommand{\RankSet}{\ensuremath{\mathbb{M}}}
\newcommand{\fullopnorm}[1]{\ensuremath{\matsnorm{#1}{\ell_2 \rightarrow
      \ell_2}}}
%\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\mbox{\tiny{op}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{2}}}

%\newcommand{\maxnorm}[1]{\ensuremath{\matsnorm{#1}{\mbox{\tiny{max}}}}}
\newcommand{\maxnorm}[1]{\ensuremath{\|#1\|_{\mbox{\tiny{max}}}}}


%\newcommand{\maxnormoff}[1]{\ensuremath{\matsnorm{#1}{\mbox{\tiny{max,off}}}}}
\newcommand{\maxnormoff}[1]{\ensuremath{\|#1\|{\mbox{\tiny{max,off}}}}}

\newcommand{\myvec}{\ensuremath{\operatorname{vec}}}
\newcommand{\MYVEC}[1]{\mathbf{#1}}
\newcommand{\sv}{\ensuremath{\gamma}}
\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\mbox{\tiny{nuc}}}}}
\newcommand{\frobnorm}[1]{\ensuremath{\matsnorm{#1}{\mbox{\tiny{F}}}}}
\newcommand{\SetBB}{\ensuremath{\mathbb{T}}}
\newcommand{\NewSetBB}{\ensuremath{\mathbb{U}}}



\newcommand{\istar}{\ensuremath{i^\ast}}


\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
\newcommand{\smallthetahat}{\ensuremath{\hat{\theta}}}

\newcommand{\Uvar}{\ensuremath{U}}

\newcommand{\Xmatt}[1]{\ensuremath{\Xmat_{#1}}}

\newcommand{\subgrad}{\ensuremath{\widehat{z}}}

\newcommand{\taupar}{\ensuremath{\tau}}
\newcommand{\betaplus}{\ensuremath{\beta^+}}
\newcommand{\betaneg}{\ensuremath{\beta^-}}

\newcommand{\bparam}{\ensuremath{\beta}}

\newcommand{\Mnum}{M}
\newcommand{\usen}{\ensuremath{N}}

\newcommand{\basefun}{\ensuremath{\phi}}

\newcommand{\Fclasspara}{\ensuremath{\mathscr{P}}}

\newcommand{\spectheta}{\gamma}
\newcommand{\TrunEllipse}{\ensuremath{\widetilde{\Ellipse}}}
\newcommand{\EllipseTil}{\TrunEllipse}

\newcommand{\jlnum}{\ensuremath{N}}
\newcommand{\jlprojdim}{\ensuremath{m}}
%\newcommand{\genthtwo}{\ensuremath{{\widetilde{\gentheta}}}}
\newcommand{\genthtwo}{\ensuremath{{\gentheta'}}}

\newcommand{\GcovNum}[3]{\ensuremath{N_{#3}(#1 \, ; \, #2)}}
\newcommand{\GpackNum}[3]{\ensuremath{M_{#3}(#1 \, ; \, #2)}}
\newcommand{\SetDia}{\ensuremath{D}}
\newcommand{\rehamm}{\ensuremath{\widebar{d}_H}}
\newcommand{\HyperCube}{\ensuremath{\mathbb{H}}}


\newcommand{\Ber}{\ensuremath{\operatorname{Ber}}}
\newcommand{\vsmall}{\vspace*{.1in}}
%\newcommand{\vtiny}{\vspace*{.05in}}


\newcommand{\orpsi}[1]{\ensuremath{\| #1\|_{\psi}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% What to use as the dimension in preliminary work on metric entropy
%\newcommand{\usedim}{\ensuremath{\mdim}} 
\newcommand{\usedim}{\ensuremath{d}} 

\newcommand{\taildim}{n}

\newcommand{\Sigal}{\ensuremath{\mathcal{A}}} 

\newcommand{\mydelta}{\ensuremath{\delta}}
\newcommand{\myeps}{\ensuremath{\epsilon}}


\newcommand{\Mcon}{\ensuremath{\kappa}}
%\newcommand{\NewMcon}{\ensuremath{\Mcon_{\LossSing}}}
%\newcommand{\NewMconBar}{\ensuremath{\widebar{\Mcon}_{\LossSing}}}

\newcommand{\NewMcon}{\ensuremath{\Mcon}}
\newcommand{\NewMconBar}{\ensuremath{\widebar{\Mcon}}}


\newcommand{\ErrRad}{\ensuremath{\TOL}}
\newcommand{\tstar}{\ensuremath{t^\ast}} 


\newcommand{\TOL}{\ensuremath{\delta}}

\newcommand{\Err}[1]{\ensuremath{\|#1\|}}



\newcommand{\Con}{\ensuremath{\eta}}
\newcommand{\KeyCon}[1]{\ensuremath{\Psi(#1)}}
\newcommand{\KeyConSq}[1]{\ensuremath{\Psi^2(#1)}}
\newcommand{\KeyRev}[1]{\ensuremath{\Phi(#1)}}
\newcommand{\KeyConOne}[1]{\ensuremath{\eta_{r;r}(#1)}}
\newcommand{\KeyConDual}[1]{\ensuremath{\eta_{r;e^*}(#1)}}
\newcommand{\KeyConFull}[1]{\ensuremath{\eta(#1; R, e)}}
\newcommand{\KeyConTwo}{\ensuremath{\eta_{r;2}}}
\newcommand{\KeyConTwoReg}{\ensuremath{\eta_{2;r}}}
\newcommand{\KeyConQpar}{\ensuremath{\eta_{(1,\qpar);2}}}


\newcommand{\myrad}{r}
%\newcommand{\KeySet}{\ensuremath{\mathcal{D}}}

\newcommand{\gvar}{\ensuremath{g}}
\newcommand{\gsam}[1]{\ensuremath{\gvar_{#1}}}


\newcommand{\EllInt}{\ensuremath{\mathcal{D}}}
\newcommand{\Ellipse}{\ensuremath{\mathcal{E}}}

\newcommand{\FclassTil}{\ensuremath{\widetilde{\Fclass}}}

\newcommand{\martmax}{\ensuremath{M}}
\newcommand{\martvar}{\ensuremath{C}}

\newcommand{\Mbou}{\ensuremath{M}}
\newcommand{\Ehat}{\ensuremath{\widehat{\mathbb{E}}}}

\newcommand{\Hclass}{\ensuremath{\mathcal{H}}}
\newcommand{\Hfclass}{\ensuremath{\mathscr{H}}}

\newcommand{\ones}{\ensuremath{\vec{1}}}
\newcommand{\Iclass}{\ensuremath{\mathcal{I}}}

\newcommand{\vtiny}{\vspace*{.05in}}

%% Gray color
%\definecolor{MyGray}{rgb}{0.96,0.97,0.98}
\definecolor{MyGray}{rgb}{0.9,0.9,0.9}



\makeatletter\newenvironment{graybox}{ 
\begin{lrbox}{\@tempboxa}
\begin{minipage}{1\columnwidth}}{\end{minipage}
\end{lrbox}%
\colorbox{MyGray}{\usebox{\@tempboxa}} }
\makeatother

%\newenvironment{graybox}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter\newenvironment{lemgraybox}{ 
\begin{lrbox}{\@tempboxa}
\begin{minipage}{.98\columnwidth}}{\end{minipage}
\end{lrbox}%
\colorbox{MyGray}{\begin{lemma} \usebox{ \@tempboxa } \end{lemma}} }

\makeatother


%\long\def\greybox#1{%
%    \newbox\contentbox%
%    \newbox\bkgdbox%
%    \setbox\contentbox\hbox to \hsize{%
%        \vtop{
%            \kern\columnsep
%            \hbox to \hsize{%
%                \kern\columnsep%
%                \advance\hsize by -2\columnsep%
%                \setlength{\textwidth}{\hsize}%
%                \vbox{
%                    \parskip=\baselineskip
%                    \parindent=0bp
%                    #1
%                }%
%                \kern\columnsep%
%            }%
%            \kern\columnsep%
%        }%
%    }%
%    \setbox\bkgdbox\vbox{
%        \pdfliteral{0.85 0.85 0.85 rg}
%        \hrule width  \wd\contentbox %
%               height \ht\contentbox %
%               depth  \dp\contentbox
%        \pdfliteral{0 0 0 rg}
%    }%
%    \wd\bkgdbox=0bp%
%    \vbox{\hbox to \hsize{\box\bkgdbox\box\contentbox}}%
%    \vskip\baselineskip%
%}


%\newcommand{\Aclass}{\ensuremath{\mathcal{A}}}


\newcommand{\Dmax}{\ensuremath{D_{\operatorname{max}}}}
\newcommand{\Dmin}{\ensuremath{D_{\operatorname{min}}}}

\newcommand{\edist}{\ensuremath{\stackrel{\mathtiny{d}}{=}}}

\newcommand{\condnum}{\kappa}
\newcommand{\condnumsq}{\kappa^2}

\newcommand{\Xtil}{\ensuremath{\widetilde{X}}}

\newcommand{\Zback}[1]{\ensuremath{Z^{\backslash i}}}

\newcommand{\argmin}{\ensuremath{\operatorname{argmin}}}

\newcommand{\range}{\ensuremath{\operatorname{range}}}
\newcommand{\rank}{\ensuremath{\operatorname{rank}}}

\newcommand{\pseurad}{\ensuremath{D}}
\newcommand{\Dudley}{\ensuremath{\mathcal{J}}}
\newcommand{\setproj}{\ensuremath{\pi}}
\newcommand{\uind}{\ensuremath{u}}

\newcommand{\Qprob}{\ensuremath{\mathbb{Q}}}

\newcommand{\SubClass}{\mathcal{S}} 
\newcommand{\SubGraph}{\ensuremath{S}}

\newcommand{\mathtiny}[1]{\ensuremath{\text{\tiny{#1}}}}
\newcommand{\mathsmall}[1]{\ensuremath{\text{\small{#1}}}}

\newcommand{\prevc}{\ensuremath{\vc}}
\newcommand{\vc}{\ensuremath{\nu}}
%\newcommand{\vc}{\ensuremath{d_{\operatorname{{\text{\tiny{VC}}}}}}}

\newcommand{\mycard}[1]{\ensuremath{|#1|}}
\newcommand{\plcard}[1]{\ensuremath{\card(#1)}}

\newcommand{\xsamstack}[1]{\ensuremath{x_1^\numobs}}
\newcommand{\Xsamstack}[1]{\ensuremath{X_1^\numobs}}
\newcommand{\Fhat}{\ensuremath{\widehat{F}}}

\newcommand{\card}{\ensuremath{\operatorname{card}}}

\newcommand{\Sclass}{\ensuremath{\mathcal{S}}}
\newcommand{\Uclass}{\ensuremath{\mathcal{U}}}

\newcommand{\NatInt}{\ensuremath{\mathbb{N}}}

\newcommand{\SetClass}{\ensuremath{\mathcal{S}}}
\newcommand{\TsetClass}{\ensuremath{\mathcal{T}}}

\newcommand{\htil}{\ensuremath{\widetilde{h}}}
\newcommand{\hstar}{\ensuremath{h^*}}
%\newcommand{\ftil}{\ensuremath{\widetilde{f}}}
\newcommand{\gtil}{\ensuremath{\widetilde{g}}}
\newcommand{\altil}{\ensuremath{\widetilde{\alpha}}}

\newcommand{\newspan}{\ensuremath{\operatorname{span}}}

\newcommand{\Newfclass}{\ensuremath{\mathbb{F}}}
%\newcommand{\Null}{\ensuremath{\mathcal{N}}} 

\newcommand{\zplus}[1]{\ensuremath{(#1)_+}}

\newcommand{\NOTS}{\ensuremath{\backslash \{\ej\}}}

\newcommand{\graph}{\ensuremath{G}}
\newcommand{\graphhat}{\ensuremath{\widehat{\graph}}}
\newcommand{\vertex}{\ensuremath{V}}
\newcommand{\edge}{\ensuremath{E}}
\newcommand{\edgehat}{\ensuremath{\widehat{\edge}}}

\newcommand{\convprob}{\ensuremath{\stackrel{\mathtiny{prob.}}{\longrightarrow}}}
\newcommand{\convas}{\ensuremath{\stackrel{a.s.}{\longrightarrow}}}
\newcommand{\convdist}{\ensuremath{\stackrel{d}{\longrightarrow}}}

\newcommand{\Zfn}{\ensuremath{\Zf_\numobs}}
\newcommand{\Xsamtil}[1]{\ensuremath{\widetilde{X}_{#1}}}
\newcommand{\Xsamprime}[1]{\ensuremath{\Xprime_{#1}}}
\newcommand{\Xback}[1]{\ensuremath{X^{\backslash #1}}}
\newcommand{\funbound}{\ensuremath{b}}
\newcommand{\funbou}{\ensuremath{\funbound}}
\newcommand{\Xprime}{\ensuremath{X'}}
\newcommand{\Ninf}[2]{\ensuremath{N_\infty(#1; #2)}}


\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}



\newcommand{\Radeplain}{\ensuremath{\mathcal{R}}}
\newcommand{\Rade}[1]{\ensuremath{\Radeplain(#1)}}
\newcommand{\Raden}[1]{\ensuremath{\Radeplain_\numobs(#1)}}
\newcommand{\RadeSq}[1]{\ensuremath{\Radeplain^2(#1)}}
\newcommand{\RadenSq}[1]{\ensuremath{\Radeplain_\numobs^2(#1)}}

\newcommand{\noisestd}{\ensuremath{\sigma}}
\newcommand{\noisevar}{\ensuremath{\sigma}}

\newcommand{\pdiff}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand{\kerpsi}{\ensuremath{\psi}}
\newcommand{\gnoisepl}{\ensuremath{g}}
\newcommand{\gnoise}[1]{\ensuremath{\gnoisepl_{#1}}}
\newcommand{\muhat}{\ensuremath{\widehat{\mu}}}


\newcommand{\radq}{\ensuremath{R_\qpar}}

\newcommand{\NoiseSeq}{\ensuremath{\{\regnoise{i}\}_{i=1}^\numobs}}

\newcommand{\NonGaussCompSpec}[1]{\ensuremath{\mathcal{G}_{#1}}}

\newcommand{\delcrit}{\ensuremath{\delta_\numobs}}
\newcommand{\delcrithat}{\ensuremath{\widehat{\delta}_\numobs}}
\newcommand{\delcritsmallhat}{\ensuremath{\hat{\delta}_\numobs}}

\newcommand{\AUSRIDGE}{8}

\newcommand{\secondnasty}{\ensuremath{128}}
\newcommand{\MyMax}{\ensuremath{Z_\numobs}}
\newcommand{\DeltaHat}{\ensuremath{\widehat{\Delta}}}

\newcommand{\NonGaussComp}{\ensuremath{\mathcal{G}_\numobs}}
\newcommand{\NonGaussCompTil}{\ensuremath{\mathcal{\widetilde{G}}_\numobs}}

\newcommand{\plregnoise}{\ensuremath{w}}
\newcommand{\regnoisepl}{\ensuremath{\plregnoise}}
\newcommand{\regnoise}[1]{\ensuremath{\plregnoise_{#1}}}


\newcommand{\NonRad}{\ensuremath{W_\numobs}}


\newcommand{\plxsam}{\ensuremath{x}}
\newcommand{\plysam}{\ensuremath{y}}
\newcommand{\plcapysam}{\ensuremath{Y}}

\newcommand{\EdgeHat}{\ensuremath{\widehat{\edge}}}

\newcommand{\EmpRad}{\ensuremath{\LocRad}}
\newcommand{\Data}[1]{\ensuremath{x_1^{#1}}}
\newcommand{\DataCap}[1]{\ensuremath{X_1^{#1}}}
\newcommand{\Zdata}[1]{\ensuremath{Z_1^{#1}}}
\newcommand{\ZdataCap}[1]{\ensuremath{Z_1^{#1}}}

\newcommand{\InterSet}{\ensuremath{\mathbb{S}}}


\newcommand{\nastyplus}{\ensuremath{257}}
\newcommand{\nastycon}{\ensuremath{256}}

\newcommand{\specrad}{\ensuremath{R}}
\newcommand{\wannoy}{\ensuremath{z}}
\newcommand{\Term}{\ensuremath{T}}
\newcommand{\sg}{\ensuremath{\kappa}}

\newcommand{\SamCov}{\ensuremath{\widehat{\CovMat}}}
\newcommand{\SamCovPlain}{\ensuremath{\widehat{\Sigma}}}
\newcommand{\PlainSamCov}{\SamCovPlain}
\newcommand{\SamCovN}{\ensuremath{\SamCov_\numobs}}

\newcommand{\Grat}{\ensuremath{G_\numobs}}



\newcommand{\AuxEvent}{\ensuremath{\mathcal{A}}}

\newcommand{\Ytil}{\ensuremath{\widetilde{Y}}}

\newcommand{\radesq}[1]{\ensuremath{\varepsilon^2(#1)}}
\newcommand{\radepl}{\ensuremath{\varepsilon}}
\newcommand{\rade}[1]{\ensuremath{\radepl_{#1}}}
\newcommand{\LocRad}{\ensuremath{\mathcal{R}_\numobs}}
\newcommand{\LocRadEmp}{\ensuremath{\widehat{\mathcal{R}}_\numobs}}



\newcommand{\epsuse}{\ensuremath{\delta}}
\newcommand{\epscrittil}{\ensuremath{\widetilde{\epsuse}_\numobs}}
\newcommand{\epscrit}{\ensuremath{\epsuse_\numobs}}
\newcommand{\newepscrit}{\ensuremath{\varepsilon_\numobs}}


\newcommand{\felltwo}[1]{\ensuremath{\|#1\|_{L^2(\mprob)}}}
\newcommand{\genfelltwo}[2]{\ensuremath{\|#1\|_{L^2(#2)}}}
\newcommand{\SpecRad}{\ensuremath{R}}


\newcommand{\kerbound}{\ensuremath{\kappa}}

\newcommand{\newrad}{\ensuremath{r}}
\newcommand{\mycon}{\ensuremath{\mu}}


\newcommand{\Event}{\ensuremath{\mathcal{E}}}
\newcommand{\Eventtil}{\ensuremath{\widetilde{\Event}}}

\newcommand{\Tset}{\ensuremath{T}}
\newcommand{\TsetCom}{\ensuremath{{\Tset^c}}}

\newcommand{\Gvar}[1]{\ensuremath{X_{#1}}}
\newcommand{\tind}{\ensuremath{t}}
\newcommand{\sind}{\ensuremath{s}}
\newcommand{\sgstan}[1]{\ensuremath{\sigma(#1)}}
\newcommand{\sgstansq}[1]{\ensuremath{\sigma^2(#1)}}
\newcommand{\pseux}{\ensuremath{\rho_X}}

%\newcommand{\Fclass}{\ensuremath{\mathcal{F}}}
%\newcommand{\Fclass}{\ensuremath{\mathbb{F}}}
\newcommand{\Fclass}{\ensuremath{\mathscr{F}}}
\newcommand{\Gclass}{\ensuremath{\mathscr{G}}}
\newcommand{\Gfclass}{\ensuremath{\mathscr{G}}}
\newcommand{\FclassTwo}{\ensuremath{\Fclass'}}
\newcommand{\FclassBar}{\ensuremath{\widebar{\Fclass}}}
\newcommand{\FclassBarUnder}{\ensuremath{\bar{\Fclass}}}

\newcommand{\Xsam}[1]{\ensuremath{X_{#1}}}

\newcommand{\Zf}{\ensuremath{Z}}


\newcommand{\fancysoln}[1]{
\ifthenelse{\equal{\doctype}{WITHSOLS}}
{
\begin{soln}
#1
\end{soln}
}
{
% Do nothing
}
}


%\newcommand{\mobs}{\ensuremath{\numobs}}

\newcommand{\trace}{\ensuremath{\operatorname{trace}}}
\newcommand{\med}{\ensuremath{\operatorname{med}}}

\newcommand{\Plainrep}{\ensuremath{R}}

\newcommand{\CoverNum}{\ensuremath{N}}

\newcommand{\thetaone}{\ensuremath{\theta}}
\newcommand{\thetatwo}{\ensuremath{\widetilde{\theta}}}

\newcommand{\wtil}{\ensuremath{\widetilde{w}}}

\newcommand{\alphatil}{\ensuremath{\widetilde{\alpha}}}
\newcommand{\ntil}{\ensuremath{\widetilde{\numobs}}}
\newcommand{\tseqtil}[1]{\ensuremath{\widetilde{t}_{#1}}} 
\newcommand{\ftil}{\ensuremath{\widetilde{f}}}



\newcommand{\Nat}{\ensuremath{\mathbb{N}}}

\newcommand{\discent}[1]{\ensuremath{H(#1)}}
\newcommand{\pmasspl}[1]{\ensuremath{p_{#1}}}
\newcommand{\pmass}[2]{\ensuremath{p_{#1}(#2)}}
\newcommand{\qerr}{\ensuremath{q_e}}
\newcommand{\discentcond}[2]{\ensuremath{H(#1 \, | \, #2)}}
\newcommand{\binent}[1]{\ensuremath{h(#1)}}
\newcommand{\xhat}{\ensuremath{\widehat{X}}}


\newcommand{\kerrank}{\ensuremath{r}}
\newcommand{\betatil}{\ensuremath{\widetilde{\beta}}}
\newcommand{\gammatil}{\ensuremath{\widetilde{\gamma}}}

\newcommand{\kull}[2]{\ensuremath{D(#1 \, \| \, #2)}}
\newcommand{\kulltwo}[2]{\ensuremath{D_2(#1 \, \| \, #2)}}
\newcommand{\qprob}{\ensuremath{\mathbb{Q}}}


\newcommand{\ugenvec}{\ensuremath{u}}
\newcommand{\vgenvec}{\ensuremath{v}}
\newcommand{\wgenvec}{\ensuremath{w}}

\newcommand{\tpt}{\ensuremath{x}}

\newcommand{\mjwcomment}[1]{\marginpar{#1}}
%\newcommand{\mjwcomment}[1]{\colorbox{red}{\marginpar{#1}}}
\newcommand{\mjwcommentbf}[1]{\marginpar{{\bf{#1}}}}
\newcommand{\mjwcommentred}[1]{\colorbox{red}{#1}}


\newcommand{\MYBIBTIT}{Bibliographic details and background}

% Old form
%\newcommand{\Tspace}{\ensuremath{\mathbb{X}}}
\newcommand{\Tspace}{\ensuremath{\mathcal{X}}}

\newcommand{\Rep}[1]{\ensuremath{\Plainrep_{#1}}}

\newcommand{\xseq}[1]{\ensuremath{x_{#1}}}
\newcommand{\tseq}[1]{\ensuremath{x_{#1}}}
\newcommand{\vseq}[1]{\ensuremath{v_{#1}}}
\newcommand{\useq}[1]{\ensuremath{u_{#1}}}

\newcommand{\VecSpace}{\ensuremath{\mathbb{V}}}

\newcommand{\genin}[3]{\ensuremath{\inprod{#1}{#2}_{#3}}}
\newcommand{\gennorm}[2]{\ensuremath{\|#1\|_{#2}}}


\newcommand{\alphahat}{\alhat}
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
\newcommand{\ppar}{\ensuremath{p}}
\newcommand{\mobs}{\ensuremath{n}}
\newcommand{\Zuni}{\ensuremath{Z}}
\newcommand{\Rad}{\ensuremath{\mathfrak{R}}}
\newcommand{\fstar}{\ensuremath{f^*}}
\newcommand{\gstar}{\ensuremath{{g^*}}}
\newcommand{\radtwo}{\ensuremath{r}}
\newcommand{\polydeg}{\ensuremath{m}}

\newcommand{\goodendex}{\hfill $\clubsuit$}
%\newcommand{\goodendex}{\hfill $\diamondsuit$}
%\newcommand{\goodendex}{\\ $\:$ \hline $\;$ \\}

\newcommand{\order}{\ensuremath{\mathcal{O}}}



\long\def\comment#1{}

%% modify cite command to do \cite[e.g, ]{foo1,foo2} 
\makeatletter
\def\@cite#1#2{[\if@tempswa #2 \fi #1]}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\Sam}{\ensuremath{\mathcal{S}}} 

\newcommand{\ysam}[1]{\ensuremath{y_{#1}}}
\newcommand{\xsam}[1]{\ensuremath{x_{#1}}}
\newcommand{\wsam}[1]{\ensuremath{w_{#1}}}


\newcommand{\Ysam}[1]{\ensuremath{Y_{#1}}}


\newcommand{\capysam}[1]{\ensuremath{Y_{#1}}}
\newcommand{\capxsam}[1]{\ensuremath{X_{#1}}}
\newcommand{\capwsam}[1]{\ensuremath{W_{#1}}}




\newcommand{\Hil}{\ensuremath{\mathbb{H}}}


\newcommand{\fhat}{\ensuremath{\widehat{f}}}
\newcommand{\yhat}{\ensuremath{\widehat{y}}}

%\newcommand{\Xspace}{\ensuremath{\mathbb{X}}}
\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}

%\newcommand{\Yspace}{\ensuremath{\mathbb{Y}}}

\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}

\newcommand{\Ker}{\ensuremath{\mathcal{K}}}
\newcommand{\Kertwo}[2]{\ensuremath{\Ker(#1, \, #2)}}
\newcommand{\KerTwo}[2]{\ensuremath{\Kertwo{#1}{#2}}}
\newcommand{\KerfunPlain}{\ensuremath{\Ker}}
%\newcommand{\hilin}[2]{\ensuremath{\inprod{#1}{#2}_{\Hil}}}

\newcommand{\alhat}{\ensuremath{\widehat{\alpha}}}

\newcommand{\Kerpl}{\ensuremath{\Kmat}}
\newcommand{\KerplPlain}{\ensuremath{K}}
\newcommand{\KerMat}{\ensuremath{\mathbf{K}}}
\newcommand{\Kerpltil}{\ensuremath{\widetilde{\Kerpl}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\HyperSub}{\ensuremath{\widetilde{\Hyper}}}
\newcommand{\rhohamm}{\ensuremath{\rho_{\tiny{H}}}}
\newcommand{\BallHamm}{\ensuremath{\Ball_{\tiny{H}}}}

\newcommand{\epspack}{\ensuremath{\epsilon}}

\newcommand{\kaplow}{\ensuremath{\kappa_\ell}}
\newcommand{\betalas}{\ensuremath{\widehat{\beta}^{\scriptsize{LA}}}}

\newcommand{\Interval}{\ensuremath{\mathcal{I}}}

\newcommand{\Hyper}{\ensuremath{\mathcal{H}}}

%\newcommand{\spindex}{\ensuremath{s}}



\newcommand{\tracer}[2]{\ensuremath{\langle \!\langle {#1}, \; {#2}
\rangle \!\rangle}}


\newcommand{\defn}{\ensuremath{: \, = }}

\newcommand{\GenSset}{\ensuremath{S}}
\newcommand{\GenTheta}{\ensuremath{\Theta}}

\newcommand{\var}{\ensuremath{\operatorname{var}}}

\newcommand{\real}{\ensuremath{\mathbb{R}}}


\newcommand{\CovNum}{\ensuremath{N}}
\newcommand{\PackNum}{\ensuremath{M}}
\newcommand{\PackSet}{\ensuremath{\mathcal{P}}}

\newcommand{\qpar}{\ensuremath{q}}

\newcommand{\pdim}{\ensuremath{p}}
\newcommand{\numobs}{\ensuremath{n}}
\newcommand{\kdim}{\ensuremath{\spindex}}
\newcommand{\spindex}{\ensuremath{s}}


\newcommand{\Sset}{\ensuremath{S}}
\newcommand{\Scomp}{\ensuremath{\Sbar}}
\newcommand{\Sbar}{\ensuremath{{\Sset^c}}}

\newcommand{\mprob}{\ensuremath{\mathbb{P}}}
\newcommand{\GenSet}{\ensuremath{\mathbb{T}}}
%\newcommand{\MetSpace}{\ensuremath{\mathbb{X}}}
\newcommand{\rhomet}{\ensuremath{\rho}}
\newcommand{\SuperCovNum}[3]{\ensuremath{\CovNum(#1 \:; \,  #2, \, #3)}}
\newcommand{\SuperCovLower}[3]{\ensuremath{\CovNum_{#3}(#1 \:; \,  #2)}}
\newcommand{\CovNumTwo}[2]{\ensuremath{\CovNum_2(#1 \:; \,  #2)}}
\newcommand{\PackNumTwo}[2]{\ensuremath{\PackNum_2(#1 \:; \,  #2)}}

\newcommand{\SuperPackNum}[3]{\ensuremath{\PackNum(#1 \:; \,  #2, \, #3)}}
\newcommand{\Ball}{\ensuremath{\mathbb{B}}}
\newcommand{\ddim}{\ensuremath{d}}

\newcommand{\GaussComp}{\ensuremath{\mathcal{G}}}
\newcommand{\GaussCompEmp}{\ensuremath{\mathcal{G}_\numobs}}
\newcommand{\RadComp}{\ensuremath{\mathbf{R}}}

%\newcommand{\MATZERO}{\ensuremath{0}}
\newcommand{\MATZERO}{\ensuremath{\mathbf{0}}}

%\newcommand{\Gvolpl}{\ensuremath{\Gamma_g}}
\newcommand{\Gvolpl}{\ensuremath{\mathcal{G}}}

\newcommand{\RADE}[1]{\ensuremath{\mathcal{R}(#1)}}

\newcommand{\Gvol}[1]{\ensuremath{\Gvolpl(#1)}}
\newcommand{\gentheta}{\ensuremath{\theta}}
\newcommand{\genthetatil}{\ensuremath{{\tilde{\gentheta}}}}
\newcommand{\sgauss}{\ensuremath{w}}
\newcommand{\rpar}{\ensuremath{p}}


\newcommand{\mdim}{\ensuremath{m}}


\newcommand{\mymathbf}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Xmat}{\ensuremath{\mymathbf{X}}}
\newcommand{\Ymat}{\ensuremath{\mymathbf{Y}}}
\newcommand{\Dmat}{\ensuremath{\mymathbf{D}}}
\newcommand{\Zmat}{\ensuremath{\mymathbf{Z}}}
\newcommand{\ZhatMat}{\ensuremath{\widehat{\Zmat}}}
\newcommand{\ZtilMat}{\ensuremath{\mymathbf{\Ztil}}}
\newcommand{\XtilMat}{\ensuremath{\widetilde{\Xmat}}}
\newcommand{\XmatTil}{\XtilMat}
\newcommand{\Mmat}{\ensuremath{\mymathbf{M}}}
\newcommand{\Nmat}{\ensuremath{\mymathbf{N}}}
\newcommand{\Smat}{\ensuremath{\mymathbf{S}}}
\newcommand{\Wmat}{\ensuremath{\mymathbf{W}}}
\newcommand{\Hmat}{\ensuremath{\mymathbf{H}}}
\newcommand{\Amat}{\ensuremath{\mymathbf{A}}}
\newcommand{\Tmat}{\ensuremath{\mymathbf{T}}}
\newcommand{\Lmat}{\ensuremath{\mymathbf{L}}}
\newcommand{\Qmat}{\ensuremath{\mymathbf{Q}}}
\newcommand{\Kmat}{\ensuremath{\mymathbf{K}}}
\newcommand{\Rmat}{\ensuremath{\mymathbf{R}}}
\newcommand{\Pmat}{\ensuremath{\mymathbf{P}}}
\newcommand{\Bmat}{\ensuremath{\mymathbf{B}}}
\newcommand{\Vmat}{\ensuremath{\mymathbf{V}}}
\newcommand{\Umat}{\ensuremath{\mymathbf{U}}}
\newcommand{\UmatHat}{\ensuremath{\widehat{\Umat}}}
\newcommand{\Cmat}{\ensuremath{\mymathbf{C}}}
\newcommand{\Emat}{\ensuremath{\mymathbf{E}}}
\newcommand{\MatVar}{\ensuremath{\mymathbf{V}}}

\newcommand{\ZeroMat}{\mathbf{0}}

%\newcommand{\Qmat}{\ensuremath{Q}}


\newcommand{\svarb}[1]{\ensuremath{\mysingval_{#1}}}
\newcommand{\svarbsq}[1]{\ensuremath{\mysingval^2_{#1}}}
\newcommand{\svarbfour}[1]{\ensuremath{\mysingval^4_{#1}}}
\newcommand{\svmax}{\ensuremath{\mysingval_{\operatorname{max}}}}
\newcommand{\svmin}{\ensuremath{\mysingval_{\operatorname{min}}}}
%\newcommand{\mprob}{\ensuremath{\mathbb{P}}}

\newcommand{\regx}{\ensuremath{x}}
\newcommand{\regw}{\ensuremath{w}}
\newcommand{\regy}{\ensuremath{y}}

\newcommand{\PlainSphere}{\ensuremath{\mathbb{S}}}
\newcommand{\Sphere}[1]{\ensuremath{\PlainSphere^{#1-1}}}
\newcommand{\SphereClose}[1]{\ensuremath{\widebar{\PlainSphere}^{#1-1}}}

\newcommand{\gencon}{\ensuremath{c}}

\newcommand{\uone}{\ensuremath{u}} 
\newcommand{\vone}{\ensuremath{v}}
\newcommand{\utwo}{\ensuremath{\tilde{\uone}}}
\newcommand{\vtwo}{\ensuremath{\tilde{\vone}}}

\newcommand{\SuperSet}{\ensuremath{T}}

%\newcommand{\vup}[1]{\ensuremath{v_{#1}}}
%\newcommand{\uup}[1]{\ensuremath{u_{#1}}}

\newcommand{\vup}[1]{\ensuremath{v^{#1}}}
\newcommand{\uup}[1]{\ensuremath{u^{#1}}}


\newcommand{\ballrad}{\ensuremath{r}}



\newcommand{\ysca}{\ensuremath{y}}
\newcommand{\wsca}{\ensuremath{w}}

\newcommand{\yvec}{\ensuremath{y}}

\newcommand{\xrow}{\ensuremath{x}}
\newcommand{\betastar}{\ensuremath{\beta^*}}


\newcommand{\betahat}{{\ensuremath{{\widehat{\beta}}}}}

\newcommand{\betals}{\ensuremath{\widehat{\beta}^{\;\mathtiny{LS}}}}
\newcommand{\rid}{\operatorname{\mathtiny{RG}}}
\newcommand{\betarid}{\ensuremath{\widehat{\beta}^{\; \rid}}}
\newcommand{\frid}{\ensuremath{f^{\rid}}}


\newcommand{\Loss}{\ensuremath{\LossSing_\numobs}}
\newcommand{\LossSing}{\ensuremath{\mathcal{L}}}
\newcommand{\LossBar}{\ensuremath{\widebar{\LossSing}}}
\newcommand{\LossSingBar}{\ensuremath{\widebar{\LossSing}}}

%\newcommand{\delLike}{\ensuremath{\delta \LossSing_{\tparam}}}
%\newcommand{\delLikeBar}{\ensuremath{\delta \LossSingBar_{\tparam}}}

\newcommand{\delLikeSing}{\ensuremath{\mathcal{E}}}
\newcommand{\delLike}{\ensuremath{\delLikeSing_\numobs}}
\newcommand{\delLikeBar}{\ensuremath{\mathcal{\widebar{E}}}}



\newcommand{\regpar}{\ensuremath{\lambda}}

\newcommand{\CovMat}{\ensuremath{\mathbf{\Sigma}}}
\newcommand{\CovMatPlain}{\ensuremath{\Sigma}}

\newcommand{\ThetaBf}{\ensuremath{\mathbf{\Theta}}}
\newcommand{\ThetaBfTil}{\ensuremath{\widetilde{\ThetaBf}}}

\newcommand{\CovMatStar}{\ensuremath{\CovMat^*}}

\newcommand{\plaincon}{\ensuremath{c}}

\newcommand{\lammin}{\ensuremath{\myeigval_{\operatorname{\tiny{min}}}}}
\newcommand{\lammax}{\ensuremath{\myeigval_{\operatorname{\tiny{max}}}}}

\newcommand{\betaup}[1]{\ensuremath{\beta^{#1}}}
\newcommand{\BetaSet}{\ensuremath{\Theta}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}


% NEW MJW VERSION
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}



\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

\newcommand{\inprodd}[3]{\ensuremath{\langle #1 , \, #2 \rangle_{#3}}}

\newcommand{\covv}[3]{\ensuremath{\cov_{#3}\{#1, \, #2\}}}


%\newcommand{\kull}[2]{\ensuremath{D(#1\; \| \; #2)}}

% IEEE Trans. Info. Theory form of Kullback-Leibler
\newcommand{\kullinf}[2]{\ensuremath{D(#1\, \| \, #2)}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Noise vector
\newcommand{\wvec}{\ensuremath{w}}
\newcommand{\Wvec}{\ensuremath{W}}

% Error vector
\newcommand{\evec}{\ensuremath{e}}

\newcommand{\Exs}{\ensuremath{\mathbb{E}}}


\newcommand{\vol}{\ensuremath{\operatorname{vol}}}


==> neurips_poster/commands.tex <==
% Common commands and definitions

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{latexsym}
\usepackage{verbatim}
% \usepackage{subfigure}
\usepackage{graphicx}
% \usepackage{psfrag}

\input{BookMacros}
\input{AMS_commands}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}

\graphicspath{ {../figures/} }
%\newcommand{\ip}[2]{\left\langle {#1}, {#2} \right\rangle}
% \newcommand{\bdsb}[1]{\boldsymbol{#1}}%%%
% \newcommand{\Pe}{\mathbb{P}_{\mathsf{e}}}
% \newcommand{\Pf}{\mathbb{P}_{F}}
% % \newcommand{\Prob}[1]{\mathsf{Pr}\left({#1}\right)}
% \newcommand{\supp}[1]{\mathsf{supp}\left({#1}\right)}
% \newcommand{\diag}[1]{\mathsf{diag}\left[{#1}\right]}
% \newcommand{\sgn}[1]{\mathsf{sgn}\left[{#1}\right]}
% \newcommand{\lr}[1]{\left(#1\right)}
% \newcommand{\lrc}[1]{\left\{#1\right\}}

% \newcommand{\red}[1]{{\color{red} #1}}
% \newcommand{\blue}[1]{{\color{blue} #1}}
% \newcommand{\magenta}[1]{{\color{magenta} #1}}


% % \floatname{algorithm}{Procedure}
% % \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% % \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \newenvironment{notation}{\noindent {\bf Notation:}}{\hspace*{\fill}\mbox{$\diamond$}}

% \renewcommand{\figurename}{Fig.}

% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{claim}{Claim}

% %\newtheorem{remark}{Remark}
% \newtheorem{result}{Result}
% \newtheorem{property}{Property}
% \newtheorem{assumption}{Assumption}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}
% \newtheorem{condition}{Condition}
% \newtheorem{fact}{Fact}
% % \newtheorem{procedure}{Procedure}
% \newtheorem{question}{Question}
% \newtheorem{problem}{Problem}
% \newtheorem{idea}{Idea}
% \newenvironment{remark}{\textit{Remark:}}


% \newenvironment{densitemize}%    Densely printed itemized list,
% {\begin{list}               %    with flush left bullets.
%     {$\bullet$ \hfill}{
%         \setlength{\leftmargin}{\parindent}
%         \setlength{\parsep}{0.04\baselineskip}
%         \setlength{\itemsep}{0.5\parsep}
%         \setlength{\labelwidth}{\leftmargin}
%         \setlength{\labelsep}{0em}}
%     }
% {\end{list}}

% \providecommand{\eref}[1]{\eqref{eq:#1}}  % call \eqref from amstex
% \providecommand{\cref}[1]{Chapter~\ref{chap:#1}}
% \providecommand{\sref}[1]{Section~\ref{sec:#1}}
% \providecommand{\fref}[1]{Fig.~\ref{fig:#1}}
% \providecommand{\sfref}[1]{Fig.~\ref{subfig:#1})}
% \providecommand{\tref}[1]{Table~\ref{tab:#1}}
% \providecommand{\aref}[1]{Algorithm~\ref{alg:#1}}
% \providecommand{\lref}[1]{Lemma~\ref{lem:#1}}
% \providecommand{\thref}[1]{Theorem~\ref{thm:#1}}

% \providecommand{\R}{\ensuremath{\mathbb{R}}}
% \providecommand{\C}{\ensuremath{\mathbb{C}}}
% \providecommand{\N}{\ensuremath{\mathbb{N}}}
% \renewcommand{\S}{\ensuremath{\mathbb{S}}}
% \providecommand{\Z}{\ensuremath{\mathbb{Z}}}

% % added by Orhan
% \providecommand{\E}[1]{\mathbb{E}\left[#1\right] }
% \providecommand{\Var}[1]{\mathrm{Var}\left[#1\right]}
% \providecommand{\Cov}[1]{\mathrm{Cov}\left[#1\right]}
% \providecommand{\sinc}{\operatorname{sinc}}
% \providecommand{\boxfun}{\operatorname{box}}
% \providecommand{\calN}{\mathcal{N}}
% \providecommand{\calL}{\mathcal{L}} 
% \DeclareMathOperator*{\argmax}{\arg\!\max}
% \DeclareMathOperator*{\argmin}{\arg\!\min}
% %%%%%

% \providecommand{\bfP}{\mathbf{P}}
% \providecommand{\abs}[1]{\left|#1\right|}
% \providecommand{\norm}[1]{\lVert#1\rVert}
% \providecommand{\inprod}[1]{\langle#1\rangle}
% \providecommand{\set}[1]{\left\{#1\right\}}
% \providecommand{\seq}[1]{\left<#1\right>}
% \providecommand{\bydef}{\overset{\text{def}}{=}}
% \providecommand{\diag}{\mathop{\mathrm{diag}}}
% \providecommand{\rank}{\mathop{\mathrm{rank}}}

% \providecommand{\parder}[2]{{\partial{#1} \over \partial{#2}}}
% \providecommand{\parderr}[2]{{\partial^2{#1} \over \partial{#2}^2}}
% \providecommand{\Rint}{\int_{\R}}

% \providecommand{\di}{\ensuremath{~\text{d}}}
% \providecommand{\e}{\ensuremath{\mathrm{e}}}
% \providecommand{\I}{\ensuremath{\mathrm{i}}}
% \providecommand{\epi}[1]{\e^{\I{#1}}}
% \providecommand{\emi}[1]{\e^{-\I{#1}}}


% \renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
% \providecommand{\mat}[1]{\ensuremath{\mathbf{#1}}}

% % \renewcommand{\vec}[1]{\ensuremath{\boldsymbol{#1}}}
% % \providecommand{\mat}[1]{\ensuremath{\boldsymbol{#1}}}

% \providecommand{\wh}[1]{\ensuremath{\widehat{#1}}}
% \providecommand{\wt}[1]{\ensuremath{\widetilde{#1}}}


% % Some calligraphic letters
% \providecommand{\calS}{\mathcal{S}} \providecommand{\calP}{\mathcal{P}}
% \providecommand{\calR}{\mathcal{R}} \providecommand{\calH}{\mathcal{H}}
% \providecommand{\calM}{\mathcal{M}} \providecommand{\calV}{\mathcal{V}}
% \providecommand{\calF}{\mathcal{F}} \providecommand{\calG}{\mathcal{G}}
% \providecommand{\calO}{\mathcal{O}} \providecommand{\calY}{\mathcal{Y}}

% % Common matrices and vectors
% \providecommand{\mA}{\mat{A}} \providecommand{\mB}{\mat{B}}
% \providecommand{\mC}{\mat{C}} \providecommand{\mD}{\mat{D}}
% \providecommand{\mE}{\mat{E}} \providecommand{\mH}{\mat{H}}
% \providecommand{\mI}{\mat{I}} \providecommand{\mJ}{\mat{J}} 
% \providecommand{\mK}{\mat{K}} \providecommand{\mL}{\mat{L}} 
% \providecommand{\mN}{\mat{N}}
% \providecommand{\mM}{\mat{M}} \providecommand{\mP}{\mat{P}} 
% \providecommand{\mQ}{\mat{Q}} \providecommand{\mR}{\mat{R}}
% \providecommand{\mS}{\mat{S}} \providecommand{\mU}{\mat{U}} 
% \providecommand{\mV}{\mat{V}} \providecommand{\mT}{\mat{T}}
% \providecommand{\mW}{\mat{W}} \providecommand{\mSigma}{\mat{\Sigma}}
% \providecommand{\mGm}{\mat{\Gamma}} \providecommand{\mG}{\mat{G}}
% \providecommand{\mPi}{\mat{\Pi}}
% \providecommand{\mX}{\mat{X}} \providecommand{\mY}{\mat{Y}}
% \providecommand{\mZ}{\mat{Z}}


% \providecommand{\va}{\vec{a}} \providecommand{\vb}{\vec{b}}
% \providecommand{\vc}{\vec{c}} \providecommand{\vd}{\vec{d}}
% \providecommand{\ve}{\vec{e}} \providecommand{\vf}{\vec{f}}
% \providecommand{\vE}{\vec{E}} \providecommand{\vF}{\vec{F}}
% \providecommand{\vg}{\vec{g}}
% \providecommand{\vh}{\vec{h}} \providecommand{\vk}{\vec{k}}
% \providecommand{\vm}{\vec{m}} \providecommand{\vn}{\vec{n}} 
% \providecommand{\vl}{\vec{l}} \providecommand{\vp}{\vec{p}}
% \providecommand{\vq}{\vec{q}} \providecommand{\vr}{\vec{r}}
% \providecommand{\vs}{\vec{s}} \providecommand{\vt}{\vec{t}}
% \providecommand{\vu}{\vec{u}} \providecommand{\vw}{\vec{w}}
% \providecommand{\vU}{\vec{U}}
% \providecommand{\vx}{\vec{x}} \providecommand{\vy}{\vec{y}}
% \providecommand{\vz}{\vec{z}} \providecommand{\vi}{\vec{i}}
% \providecommand{\vj}{\vec{j}} \providecommand{\vzero}{\vec{0}}
% \providecommand{\vgm}{\vec{\gamma}} \providecommand{\vv}{\vec{v}}
% \providecommand{\vlambda}{\vec{\lambda}}
% \providecommand{\vmu}{\vec{\mu}}
% \providecommand{\vomg}{\vec{\omega}}
% \providecommand{\vsigma}{\vec{\sigma}}


% % symbols with wide hats
% \providecommand{\whu}{\wh{u}} \providecommand{\whf}{\wh{f}}

% % symbols with wide tildas

% \providecommand{\w}{\omega}

% \providecommand{\conv}{\ast}
% \providecommand{\circonv}[1]{\circledast_{#1}}

% \renewcommand{\div}{\mathop{\mathrm{div}}}
% \providecommand{\grad}{\mathop{\mathrm{grad}}}
% \newcommand{\defn}{\ensuremath{:=}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\gammastar}{\ensuremath{\gamma^*}}
\renewcommand{\Loss}{\ensuremath{\mathcal{L}}}
\newcommand{\Jloss}{\ensuremath{\mathcal{J}}}
\newcommand{\EmpLoss}{\ensuremath{\Loss_\numobs}}
\newcommand{\EmpJloss}{\ensuremath{\Jloss_\numobs}}
\newcommand{\EmpOp}{G_{\numobs}}
\newcommand{\PopOp}{G}

\newcommand{\ffun}{\ensuremath{f}}
%\newcommand{\fhat}{\ensuremath{\widehat{\ffun}}}
%\newcommand{\fstar}{\ensuremath{\ffun^*}}

\newcommand{\fval}{\ensuremath{\theta}}
\newcommand{\fvalhat}{\ensuremath{\widehat{\fval}}}
\newcommand{\fvalstar}{\ensuremath{\fval^*}}
\newcommand{\fvaltil}{\ensuremath{\tilde{\fval}}}
\newcommand{\fvalstarConst}{\fvalstar_{\ConstSet}}
\newcommand{\stsize}{\alpha}

\newcommand{\inprodk}[2]{\langle #1, #2 \rangle_{\Hil}}
\newcommand{\inprodfunc}[2]{\langle #1, #2 \rangle_\numobs}
\newcommand{\enorm}[1]{\| #1 \|_\numobs}
\newcommand{\fnorm}[1]{\|#1\|_{\mathcal{F}}}
\newcommand{\knorm}[1]{\|#1\|_{\Hil}}
\newcommand{\ltwo}[1]{\| #1 \|_2}
\newcommand{\Fspace}{\mathcal{F}}

\newcommand{\fvalit}[1]{\ensuremath{\fval^{#1}}}
\newcommand{\HilNorm}[1]{\ensuremath{\| #1\|_{\Hil}}}
\newcommand{\EmpNorm}[1]{\ensuremath{\|#1\|_{\numobs}}}
\newcommand{\somenorm}[1]{\ensuremath{\|#1\|}}
\newcommand{\EmpInner}[2]{\ensuremath{\inprod{#1}{#2}_\numobs}}
\newcommand{\DelIt}[1]{\ensuremath{\Delta^{#1}}}
\renewcommand{\strongcon}{\ensuremath{m}}
\newcommand{\lipcon}{\ensuremath{M}}
\newcommand{\lipconprime}{\ensuremath{\tilde{\lipcon}}}
\newcommand{\zval}{\ensuremath{z}}
\newcommand{\zvalit}[1]{\ensuremath{\zval^{#1}}}
\newcommand{\zvalstar}{\ensuremath{z^*}}
\newcommand{\zvalstarConst}{\zvalstar_{\ConstSet}}
\newcommand{\zstar}{\ensuremath{z^*}}
\newcommand{\Kmax}{\lambda_{\max}}
% Successive difference
\newcommand{\Sdiff}[1]{\ensuremath{d^{#1}}}
\newcommand{\Hdiff}[1]{\ensuremath{D}^{#1}}

\renewcommand{\Kmat}{\ensuremath{K}}
\newcommand{\KmatSqrt}{\ensuremath{\sqrt{K}}}
\newcommand{\Kdiag}{\Lambda}
\newcommand{\KdiagSqrt}{\Kdiag^{1/2}}
\newcommand{\KdiagUpper}{\Kdiag_1}
\newcommand{\KdiagLower}{\Kdiag_2}
\newcommand{\DelGamUpper}{\Delta_{\gamma,1}}
\newcommand{\DelGam}{\Delta_{\gamma}}
\newcommand{\DelFun}{\Delta_{\fval}}
\newcommand{\Delz}{\Delta_\zval}
\newcommand{\Exp}{\text{exp}}
\newcommand{\ConstSet}{\mathcal{C}}
\newcommand{\RespSet}{\mathcal{Y}}
\newcommand{\secarg}{\ensuremath{\theta}}


\newcommand{\Tele}[1]{\ensuremath{V^{#1}}}
\newcommand{\Radius}{C_{\mathcal{H}}}
\newcommand{\popnorm}[1]{\|#1\|_{L^2(\PP)}}

\newcommand{\hatf}{\widehat{f}}
\newcommand{\GW}{\mathcal{G}_\numobs}
\newcommand{\GWP}{\mathcal{\widebar{G}}_\numobs}
\newcommand{\EGW}{\mathcal{Z}_\numobs}
\newcommand{\EGWS}{\mathcal{\tilde{Z}}_\numobs}
\newcommand{\RadeC}{\widebar{\mathcal{R}}}
\newcommand{\Fstar}{\mathcal{F}^*}

\newcommand{\Eset}[2]{\mathcal{E}(#1,#2)}
% \newcommand{\ltwo}[1]{\|#1\|_2}
\newcommand{\dotprod}{\odot}
\newcommand{\CrudeTerm}{T}

\newcommand{\straightd}{\text{d}}
\newcommand{\Hess}{H}
\newcommand{\E}{\text{e}}
\newcommand{\Gspace}{\mathcal{G}}
\newcommand{\phiLoss}{\phi}
\newcommand{\critquant}{\delta_n}
\newcommand{\popcritquant}{\widebar{\delta}_\numobs}
\newcommand{\Sobolev}{\mathbb{H}}

\newcommand{\sceff}{\gamma}
\newcommand{\scefftil}{\widetilde{\sceff}}
\newcommand{\Short}{S}
\newcommand{\AnnCon}{c_3}
\newcommand{\A}{\mathcal{A}}
\newcommand{\Kspace}{\mathcal{K}}
\newcommand{\SubK}{\Hil_{\numobs}}
\newcommand{\AvgEst}{\bar{\fval}}
\newcommand{\Inprod}{T_\numobs}
\newcommand{\Diam}{D}
\newcommand{\PhiB}{B}
\newcommand{\Kerfunc}{\mathbb{K}}
\newcommand{\KerR}{\mathcal{R}}
\newcommand{\PP}{\mathbb{P}}

\newcommand{\indloss}{\phi}
\newcommand{\phibound}{L}
%\newcommand{\R}{\ensuremath{\mathcal{\rho}}}
\newcommand{\R}{R}
\newcommand{\Rfstar}{\ensuremath{\fstar_\R}}
\newcommand{\Rfvalstar}{\ensuremath{\fvalstar_\R}}

\newcommand{\barspan}{\widebar{\text{span}}}

\newcommand{\conrad}{r_1}
\newcommand{\enormball}{\mathbb{B}_\numobs}
\newcommand{\HilNormball}{\mathbb{B}_{\Hil}}
\newcommand{\HilNormBall}{\HilNormball}
\newcommand{\Hilstar}{\partial \Hil}
\newcommand{\matchquant}{\xi}
\newcommand{\critC}{C_\ell}
\newcommand{\noise}{w}
\newcommand{\fcoeff}{\omega}
\newcommand{\fcoefftil}{\tilde{\fcoeff}}
\newcommand{\evalfunct}{R}
\newcommand{\const}{c}
\newcommand{\sigmaType}{h}
\newcommand{\Rkrr}{R}
\newcommand{\set}{\mathcal{S}}
\newcommand{\dhat}{\widehat{d}}

\DeclareMathOperator*{\argmax}{arg\, max\,}

% For comments and colors
\newcommand{\makepink}[1]{{\color{mypink}{#1}}}
\newcommand{\makered}[1]{{\color{myred}{#1}}}
\newcommand{\makeblue}[1]{{\color{blue}{#1}}}
\newcommand{\mjwred}[1]{\makered{{MJW: $\quad$ #1}}}
\newcommand{\fycomment}[1]{\makeblue{{FY: $\quad$ #1}}}
\newcommand{\yutingcomment}[1]{\makepink{{YW: $\quad$ #1}}}


\renewcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\renewcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\domX}{\mathcal{X}}
\newcommand{\ExsY}{\ensuremath{\Exs_{Y_1^\numobs}}}
\newcommand{\XYDATA}{\ensuremath{\{x_i, Y_i\}_{i=1}^\numobs}}
\newcommand{\fit}[1]{\ensuremath{f^{#1}}}
\newcommand{\step}[1]{\ensuremath{\alpha^{#1}}}
\newcommand{\KerFun}{\ensuremath{\mathbb{K}}}
\renewcommand{\Hil}{\ensuremath{\mathcal{H}}}
\newcommand{\FSEQ}{\ensuremath{\{\fit{t}\}_{t=0}^\infty}}
\renewcommand{\muhat}{\ensuremath{\widehat{\mu}}}
\renewcommand{\d}{\text{d}}
\newcommand{\pseudinv}{\dagger}
\newcommand{\statdim}{d_{\numobs}}

\newcommand{\newnoise}{\epsilon}
\newcommand{\level}{\sigma}
\newcommand{\Avgf}[1]{\bar{f}^{#1}}
\newcommand{\opcrit}{\rho_\numobs}

\newcommand{\mMC}{$m$-$M$-condition}
\newcommand{\PhiBC}{$\phi'$-boundedness}
\newcommand{\red}[1]{\textcolor{red}{#1}}

\newcommand{\HANASET}{\ensuremath{\mathbb{S}}}
%\newcommand{\Event}{\ensuremath{\mathcal{E}}}

\newcommand{\Qfun}{\ensuremath{Q}}
\newcommand{\yback}[1]{\ensuremath{y^{\backslash #1}}}

\newcommand{\EllipseBar}{\ensuremath{\widebar{\Ellipse}}}

\newcommand{\mprobx}{\ensuremath{\mprob_X}}

\newenvironment{hclist}
 {\begin{list}{$\bullet$}
 {\setlength{\topsep}{0in} \setlength{\partopsep}{0in}
  \setlength{\parsep}{0in} \setlength{\itemsep}{\parskip}
  \setlength{\leftmargin}{0.15in} \setlength{\rightmargin}{0.08in}
  \setlength{\listparindent}{0in} \setlength{\labelwidth}{0.08in}
  \setlength{\labelsep}{0.1in} \setlength{\itemindent}{0in}}}
 {\end{list}}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 



